Phase Transitions via Complex Extensions of Markov Chains

We study algebraic properties of partition functions, particularly the location of zeros, through the lens of rapidly mixing Markov chains. The classical Lee-Yang program initiated the study of phase transitions via locating complex zeros of partition functions. Markov chains, besides serving as algorithms, have also been used to model physical processes tending to equilibrium. In many scenarios, rapid mixing of Markov chains coincides with the absence of phase transitions (complex zeros). Prior works have shown that the absence of phase transitions implies rapid mixing of Markov chains. We reveal a converse connection by lifting probabilistic tools for the analysis of Markov chains to study complex zeros of partition functions. Our motivating example is the independence polynomial on $k$-uniform hypergraphs, where the best-known zero-free regime has been significantly lagging behind the regime where we have rapidly mixing Markov chains for the underlying hypergraph independent sets. Specifically, the Glauber dynamics is known to mix rapidly on independent sets in a $k$-uniform hypergraph of maximum degree $\Delta$ provided that $\Delta \lesssim 2^{k/2}$. On the other hand, the best-known zero-freeness around the point $1$ of the independence polynomial on $k$-uniform hypergraphs requires $\Delta \le 5$, the same bound as on a graph. By introducing a complex extension of Markov chains, we lift an existing percolation argument to the complex plane, and show that if $\Delta \lesssim 2^{k/2}$, the Markov chain converges in a complex neighborhood, and the independence polynomial itself does not vanish in the same neighborhood. In the same regime, our result also implies central limit theorems for the size of a uniformly random independent set, and deterministic approximation algorithms for the number of hypergraph independent sets of size $k \le \alpha n$ for some constant $\alpha$.

==> amend.tex <==
\newpage
\section{Decay of percolation}\label{sec:proof}

In this section, we prove the decay of percolation property (\Cref{lemma:diminishing-bad-tree}), which asserts that large bad trees have diminishing contributions. Recall that we use bad trees to keep track of a ``percolation probability'', so this lemma controls the ``decay of percolation''. 

Our approach follows a similar framework to the one used for bounding the contributions of small bad trees (\Cref{lemma:characterization}-(\ref{item:characterization-2}) 
 and \Cref{lemma:modulus-bound-subset}). A key technical distinction here is that, when the bad tree is large, the outcome may no longer be determined solely by the bad component. To address this, we show that in such cases, the information from the bad component, along with the $r_t$ values for the first $n$ timestamps, is sufficient to serve as a certificate of the outcome.

Fix $T\ge n$. Let $I = [-T+1, -T+n]$. Let $\*r_I = (r_t)_{t = -T+1}^{-T+n}\in \{0,\bot\}^I$ denote the first $n$ timestamps of~$\*r$.  We first show a counterpart of \Cref{lemma:characterization}-(\ref{item:characterization-2}) for large bad trees.


\begin{lemma}\label{lemma:outcome-correspondence}
Fix any $T\geq n$ and any event $A\subseteq \{0,1\}^V$. 
Consider the witness graph $G_H^S = \tp{V_H^S, E_H^S}$ constructed using the set of variables $S=\vbl(A)$.
Let $\bm{\rho}=(\rho_t)_{t=-T+1}^{0}\in\{0,\bot\}^T$. 
%be a sequence where each $\rho_t\in \{0,1,\bot\}$. 

Then for any initial configuration $\sigma\in \supp(\mu)$, the occurrence of $A$ at time $0$ is determined by $\cbad(\bm{\rho})$ and $\*\rho_{I}$, i.e.,
\begin{equation}\label{eq:4-11-2-tree-modulus-bound-subset}
% Fix
\mu_{T, \sigma, \*b}^\-{GD}(\sigma_0\in A \mid \+C^\-{bad}(\*r) = \cbad(\*\rho) \land \*r_I = \*\rho_I) \in \{0, 1\}.
\end{equation}


\end{lemma}
\begin{proof}
Let $\BadTS{\*\rho} \defeq \bigcup\limits_{s \in \cbad(\*\rho)} s$.
    Conditioning on $\+C^\-{bad}
    (\*r) = \cbad(\*\rho) \land \*r_I = \*\rho_I$, we know that for all $t\in \BadTS{\*\rho}$ that $t \le -T + n$, it holds that $r_t = \*\rho_{I}(t)$.

    If $t \ge -T + n + 1$ for all $t\in \BadTS{\*\rho}$, then we can determine $\sigma_0$ by $\cbad(\*\rho)$ following the proof of \Cref{lemma:characterization}-(\ref{item:characterization-2}). Otherwise, we claim that, given $\*\rho_I$, we can still deduce the result of the update at each timestamp $t\in \BadTS{\*\rho}$. Then, the lemma directly follows from this claim, as the updates alone can completely determine $\sigma_0$.

We then prove the claim. By \Cref{Alg:complex-GD-decomposed-his}, given some timestamp $t$, 
% let $v=v_{i(t)}$. Note 
$r_t = 0 \text{ or } \bot$ due to the $\*b$-decomposition scheme specified in \eqref{eq:base-measure-his}. If $r_t=0$, then  $\sigma_t(v_{i(t)})$ is updated to $0$ at time $t$; otherwise  $r_t=\bot$, and $\sigma_t(v_{i(t)})$ is updated to $0$ if and only if the following event occurs:
\begin{equation}\label{eq:4-11-his-bad-event}
    \exists e\in \+E \text{ s.t. }v_{i(t)}\in e:  \forall u\in e\setminus \{v_{i(t)}\}, \sigma_t(u)=1,
\end{equation} meaning that the value of all the vertices in $e\setminus \{v_{i(t)}\}$ got updated to $1$ at their last updates. 

Fix a specific $t \in \BadTS{\*\rho}$, 
\begin{itemize}
    \item if $t\geq -T+1+n$, 
 we argue that it suffices to check the event in \eqref{eq:4-11-his-bad-event} for the hyperedges $e$ such that $\ts(e,t)\in \+C^{\-{bad}}(\*\rho)$. We note that when $t\geq -T+1+n$ and $t\in \BadTS{\*\rho}$, an edge $e'$ such that $v_{i(t)}\in e'$ and
$\ts(e',t)\not\in \+C^{\-{bad}}(\*\rho)$  means there exists $t' \in \ts(e',t)$ such that $r_{t'} = 0$, which means $\sigma_t(v_{i(t')}) = \sigma_{t'}(v_{i(t')})=0$.  Therefore, this edge $e'$ does not satisfy \eqref{eq:4-11-his-bad-event} as one of its vertices is already assigned $0$,
\item if $t\le-T+n$,  all events in \eqref{eq:4-11-his-bad-event} can be determined from $\*\rho_I$. 
\end{itemize}
% So we only need the initial configuration and the values of timestamps in $\BadTS{\*\rho}$, $I$ to deduce the result of updates.
Therefore, we can deduce the result of the updates at each $t\in \BadTS{\*\rho}$ in chronological order.

% Because for any edge $e'$ that involves values at $t\not\in \BadTS{\*\rho}$, we have $\ts(e',t)\not\in \+C^{\-{bad}}(\*\rho)$, and by the same argument as above, $e'$ does not satisfy \eqref{eq:his-bad-event}.


\end{proof}

We also have the following lemma that serves as a counterpart of \Cref{lemma:modulus-bound-subset}.
\begin{lemma}\label{lemma:modulus-bound-component-rn}
Fix any $S\subseteq V$ and $T\geq n$. 
Consider the witness graph $G_H^S$, the bad component $\cbad=\cbad(\*r)$, and the bad tree $\+T^{\-{bad}}=\+T^{\-{bad}}(\bm{r})=\=T(\cbad)$ ,
where $\bm{r}=(r_t)_{t=-T+1}^{0}\in\{0,\bot\}^T$ is constructed as in \Cref{Alg:complex-GD-decomposed-his}, following the product measure in~\eqref{eq:base-measure-his}.
Then, for any $\sigma\in \supp(\mu)$, for any $2$-tree $\+T$ in $G^S_H$ containing $\ts(S,0)$, we have
\begin{equation}\label{eq:2-tree-modulus-bound-component-rn}
\sum\limits_{\+C \in \=T^{-1}(\+T)}
\sum\limits_{\*\rho_I \in \{0,\bot\}^I}
\abs{\mu^{\-{GD}}_{T,\sigma,\bm{b}} \tp{\+C^{\-{bad}} = \+C \land \*r_I = \*\rho_I}}\leq \alpha^{|\+T|-1}\cdot M^{4\Delta^2k^4|S| + n}.
\end{equation}
\end{lemma}
\begin{proof}
According to the deterministic process in \Cref{definition:2-tree-construction} for the construction of the $2$-tree $\+T^{\-{bad}}=\=T(\+C^{\-{bad}})$, all $\+C\in \=T^{-1}(\+T^\-{bad})$ must only contain vertices in $G^S_H$ that are within distance $1$ of $\+T^\-{bad}$, and to determine $\cbad$ it is sufficient to check for all vertices in $G_H^S$ that are within distance $2$ of $\+T^\-{bad}$ whether they are in $V^{\-{bad}}$ or not. Therefore, we can bound the left-hand side in \eqref{eq:2-tree-modulus-bound-component-rn} by translating to the following condition on $\bm{r}$:
\begin{enumerate}
   \item for each $s\in \+T\setminus \ts(S,0)$, we have $r_t=\bot$ for all $t\in s$;\label{item:4-11-modulus-bound-1}
   \item $r_t=\bm{\rho}_I(t)$ for each $t\in I$; \label{item:4-11-modulus-bound-2}
   \item $r_t$'s on vertices within distance $2$ of $\+T$ satisfy certain restrictions so that $\cbad\in \=T^{-1}(\+T)$.  \label{item:4-11-modulus-bound-3}
\end{enumerate}

Here, the \Cref{item:4-11-modulus-bound-1} contributes a factor of 
\[
\prod\limits_{t\in s:s\in \+T\setminus \ts(S,0)}\abs{\frac{\lambda_{v_{i(t)}}}{1+\lambda_{v_{i(t)}}}}\leq N^{|\+T|-1},
\]by the definition of $2$-trees that all vertices in $\+T$ contain disjoint timestamps. We can use a simple triangle inequality to bound \Cref{item:4-11-modulus-bound-2}. 
% Let $(G_H^{S})^2 = (V_H^S, (E_H^{S})^2)$ be the square graph of $G_H^S$, where $(E_H^{S})^2 = \{(u,v) \mid  u,v\in V_H^S, 1\le \text{dist}_{G_H^S}(u, v) \le 2 \}$.
By \Cref{lemma:witness-graph-degree-bound}, the degree of $\ts(S,0)$ in $\left(G_H^S\right)^2$ can be upper bounded by $4\Delta^2k^3|S|$, where $\left(G_H^S\right)^2$ is the square graph of $G_H^S$. For vertices other than $\ts(S,0)$, the number of their neighboring vertices in $\left(G_H^S\right)^2$, excluding those already adjacent to $\ts(S,0)$, can be upper bounded by $4\Delta^2k^4$. Therefore, there are at most $4\Delta^2k^4(|\+T|-1)+4\Delta^2k^3|S|$ vertices and at most $4\Delta^2k^5(|\+T|-1)+4\Delta^2k^4|S|$ timestamps included. And each timestamp $t$ contributes at most $\abs{\frac{1}{1 + \lambda_{v_{i(t)}}}} + \abs{\frac{\lambda_{v_{i(t)}}}{1 + \lambda_{v_{i(t)}}}} \le M$ by a triangle inequality. So \Cref{item:4-11-modulus-bound-2,item:4-11-modulus-bound-3} together contribute a factor of at most 
\[M^{4\Delta^2k^5(|\+T|-1)+4\Delta^2k^4|S| + n}.
\]
Summarizing, we have
\begin{align*}
\sum\limits_{\+C \in \=T^{-1}(\+T)}
\sum\limits_{\*\rho_I \in \{0,\bot\}^I}
\abs{\mu^{\-{GD}}_{T,\sigma,\bm{b}} \tp{\+C^{\-{bad}} =\+C \land \*r_I = \*\rho_I}}
&\leq  N^{|\+T|-1}\cdot M^{4\Delta^2k^5(|\+T|-1)+4\Delta^2k^4|S| + n}\\
&\leq \alpha^{|\+T|-1}\cdot M^{4\Delta^2k^4|S|+n}. 
% &\qedhere
\end{align*}
%finishing the proof of the lemma.
\end{proof}

% \begin{}

We are now ready to prove \Cref{lemma:diminishing-bad-tree}.
 \begin{proof}[Proof of \Cref{lemma:diminishing-bad-tree}]
For each $i\geq 1$, let $\+T_i$ denote the set of possible $2$-trees of size $i$ in $G^S_H$ containing $\ts(S,0)$. Recall the definition of the bad component $\cbad=\cbad(\*r)$ in \Cref{definition:bad-vertices-his} and that we use $\=T$ to denote the construction in \Cref{definition:2-tree-construction} such that $\=T(\cbad)=\tbad$.  Then letting $D_1=4\Delta^2k^4$ and $D_2=4\Delta^2k^3|S|$, we have 
% \begin{equation}\label{eq:bad-tree-growth-transform}
\begin{align*}
 &  \lim\limits_{T\to \infty}\abs{\mu^{\-{GD}}_{T,\sigma,\bm{b}}\tp{\sigma_0=\tau\land |\tbad|>T/(2n)-2}}\\
 \le&\lim\limits_{T\to \infty} \sum\limits_{i>T/(2n)-2}\sum\limits_{\+T\in \+T_i}\sum\limits_{\+C\in \=T^{-1}(\+T)} 
 \sum\limits_{\*\rho_I \in \{0,\bot\}^I}
 \abs{\mu^{\-{GD}}_{T,\sigma,\bm{b}}(\sigma_0 = \tau \mid \+C^\-{bad} = \+C \land \*r_I = \*\rho_I)}\\
 &\qquad \cdot \abs{\mu^{\-{GD}}_{T,\sigma,\bm{b}}(\+C^\-{bad} = \+C \land \*r_I = \*\rho_I))}\\
 (\text{by \Cref{lemma:outcome-correspondence}})\quad\le& \lim\limits_{T\to \infty} \sum\limits_{i>T/(2n)-2}\sum\limits_{\+T\in \+T_i}\sum\limits_{\+C\in \=T^{-1}(\+T)} 
 \sum\limits_{\*\rho_I \in \{0,\bot\}^I} \abs{\mu^{\-{GD}}_{T,\sigma,\bm{b}}(\+C^\-{bad} = \+C \land \*r_I = \*\rho_I))} \\ 
 (\text{by \Cref{lemma:modulus-bound-component-rn}}) \quad  \leq &  \lim\limits_{T\to \infty}\sum\limits_{i> T/(2n)-2} \sum\limits_{\+T\in \+T_i} \alpha^{i-1}\cdot M^{4\Delta^2k^4n + n}\\
 (\text{by \Cref{lemma:bad-tree-num-bound}}) \quad  \leq & \lim\limits_{T\to \infty}\sum\limits_{i> T/(2n)-2}  (\mathrm{e}(D_2 + i - 2))^{D_2 - 1} \cdot (\mathrm{e}D_1)^{i-1}\cdot \alpha^{i-1}\cdot M^{4\Delta^2k^4n + n} \\
(\text{by \eqref{eq:bound-alpha}})\quad \le& \lim\limits_{T\to \infty}\sum\limits_{i> T/(2n)-2}  (\mathrm{e}(D_2 + i - 2))^{D_2 - 1}\cdot M^{4\Delta^2k^4n + n} \frac{1}{2^{i-1}}\\
(\text{by taking limit})\quad =&0.
\end{align*}
% \end{equation}

% \begin{equation}\label{eq:bad-tree-growth-transform}
% \begin{aligned}
%  &  \lim\limits_{T\to \infty}\abs{\mu^{\-{GD}}_{T,\sigma,\bm{b}}\tp{\sigma_0=\tau\land |\tbad|>T/(2n)-2}}\\
%  \le&\lim\limits_{T\to \infty} \sum\limits_{i>T/(2n)-2}\sum\limits_{\+T\in \+T_i}\sum\limits_{\+C\in \=T^{-1}(\+T)} \abs{\mu^{\-{GD}}_{T,\sigma,\bm{b}}\tp{\cbad=\+C}\cdot \mu^{\-{GD}}_{T,\sigma,\bm{b}}\tp{\sigma_0=\tau\mid \cbad=\+C}}.
% \end{aligned}
% \end{equation}

% We claim that for any $C$. Let $I = [-T-n, -T-1]$, it holds that,
% \begin{align*}
%  \abs{\mu^{\-{GD}}_{T,\sigma,\bm{b}}\tp{\sigma_0=\tau\mid \cbad=\+C}}&\le
% \sum\limits_{\*\rho_{I} \in \{0,1\}^n}\abs{\mu^{\-{GD}}_{T,\sigma,\bm{b}}\tp{\sigma_0=\tau, \*r_I = \*\rho_I\mid \cbad=\+C}}\\
% &\le M^n.
% \end{align*}

\begin{comment}
 Note that by \Cref{lemma:characterization}-(\ref{item:characterization-2}), for any $\+T\in \+T_i$ with $i>T/(2n)-2$,
 \todo{JL:FIXME, this is incorrect}
 the measure $\mu^{\-{GD}}_{T,\sigma,\bm{b}}(\sigma_0=\tau\mid \cbad=\+C)$ evaluates to either $0$ or $1$ for each $\+C\in \mathbb{T}^{-1}(\+T)$. We then define $\+C^{T,\sigma,\tau}(\+T)$ as the set of bad components $\+C\in \mathbb{T}^{-1}(\+T)$ such that $\mu^{\-{GD}}_{\tau,\sigma,\bm{b}}(\sigma_0=\tau\mid \cbad=\+C)=1$.

     Therefore, letting $D_1=4\Delta^2k^4$ and $D_2=4\Delta^2k^3|S|$, we have
    \begin{align*}
    &\lim\limits_{T\to \infty} \sum\limits_{i>T/(2n)-2}\sum\limits_{\+T\in \+T_i}\sum\limits_{\+C\in \=T^{-1}(\+T)} \abs{\mu^{\-{GD}}_{T,\sigma,\bm{b}}\tp{\cbad=\+C}\cdot \mu^{\-{GD}}_{T,\sigma,\bm{b}}\tp{\sigma_0=\tau\mid \cbad=\+C}}\\
= &\lim\limits_{T\to \infty}\sum\limits_{i> T/(2n)-2} \sum\limits_{\+T\in \+T_i} \abs{ \mu^{\-{GD}}_{T,\sigma,\bm{b}}\tp{\cbad \in \+C^{T,\sigma,\tau}(\+T)}}\\
 (\text{by \Cref{lemma:modulus-bound-subset}}) \quad  \leq &  \lim\limits_{T\to \infty}\sum\limits_{i> T/(2n)-2} \sum\limits_{\+T\in \+T_i} \alpha^{i-1}\cdot M^{4\Delta^2k^4n}\\
 (\text{by \Cref{lemma:bad-tree-num-bound}}) \quad  \leq & \lim\limits_{T\to \infty}\sum\limits_{i> T/(2n)-2}  (\mathrm{e}(D_2 + i - 2))^{D_2 - 1} \cdot (\mathrm{e}D_1)^{i-1}\cdot \alpha^{i-1}\cdot M^{4\Delta^2k^4n} \\
(\text{by \eqref{eq:bound-alpha}})\quad \le& \lim\limits_{T\to \infty}\sum\limits_{i> T/(2n)-2}  (\mathrm{e}(D_2 + i - 2))^{D_2 - 1}\cdot M^{4\Delta^2k^4n} \frac{1}{2^{i-1}}\\
(\text{by taking limit})\quad =&0.
    \end{align*}
    This completes the proof of the lemma after combining with \eqref{eq:bad-tree-growth-transform}.
\end{comment}
 \end{proof}

==> backup_intro.tex <==
The relation between approximate counting and the zero-free region has recently been extensively studied in theoretical computer science. 
The task of approximate counting is to approximate a graph polynomial, also known as the partition function, which originated from Statistical physics. In combinatorics, the partition function is equal to the generating function. For example, the partition function for the hardcore model on graph $G=(V, E)$ is defined as $Z(\lambda) = \sum_{i\ge 0} a_i \lambda^i$ where $a_i$ equals to the number of  size-$i$ independent sets which encompasses the information of the independent sets.
The zero-free region of the partition function is a connected region in the complex plane such that the partition function does not vanish. The zero-free region is an important geometric property of polynomials whose researches date back to the seminal Lee-Yang theorem that proves the zero-free region of the ferromagnetic Ising model \cite{Lee1952StatisticalTO} and the half-plane zero-free region of the Monomer-dimer model  \cite{Heilmann1972TheoryOM}.  The zero-free region can imply many combinatorial properties. For example, zero-free region implies properties about the associating distribution, such as the central limit theorem from zero-free region \cite{Michelen2019CentralLT} and the strongly Rayleigh from the real stability which means that the partition function is zero-free in the upper half complex plane \cite{Borcea2007NegativeDA}. It also relates the log-concavity and the Lorentzian polynomial  \cite{branden2020lorentzian}. 

A direct corollary from the zero-free region of the spin system is the deterministic approximate counting algorithm by the polynomial interpolation method \cite{barvinok2016computing, barvinok2016combinatorics, Liu2017TheIP}. 
The intuition is to view the partition function as a polynomial and then truncate the $\log$-partition function to give a multiplicative approximation of the partition function where the zero-free property is used to ensure the convergence rate of the truncated polynomial \cite{barvinok2016combinatorics}. This method is also refined to give FPTASes in bounded degree graphs in \cite{patel2017deterministic, Liu2017TheIP} by subgraphs counting and insects counting.
This method almost matches many state-of-the-art results. 

Besides the polynomial interpolation method from the zero-free property, there are many powerful methods for approximate counting that do not originate from the zero-free property like Markov Chain Monte Carlo (MCMC), correlation decay and linear programming.  
Among them, MCMC is a powerful tool for designing randomized approximate sampling algorithms. For self-reducible problems, one can derive approximate counting algorithms by approximate sampling algorithms \cite{jerrum1986random}. 
With the development of the spectral independence recently, MCMC achieves near linear time sampling for many problems \cite{chen2021optimal, CFYZ2022,anari2022entropic,chen2023uniqueness, CE22,chen2023strong}. While the correlation decay and the linear programming methods are used to design deterministic algorithms \cite{Moi19,guo2019counting,galanis2019counting, Vishesh21towards, Wang2024ASL}. 

At first glance, these methods are so different. But surprisingly, some results about the relations between zero-freeness and other methods have been done recently.
For the correlation decay method, it can be lifted to the complex plane to prove zero-free regions \cite{peter2019conjecture, Liu2017TheIP, liu2019correlation, Shao2019ContractionAU}. 
% This holds for the cluster expansion method that \cite{Chen2019FastAA,Jenssen2018AlgorithmsF}  . 
Also, the zero-free region under arbitrary pinnings can derive the bound of the aforementioned spectral independence which is a powerful tool to bound the mixing time of MCMC \cite{Alimohammadi2021FractionallyLA, Chen2021SpectralIV}. 

So an open conjecture is that if there is a FPTAS, there is a zero-free region.

% In this paper, we focus on the relation between the rapid mixing of the Markov chain and the zero-free region.
% It is interesting if approximate counting is equal to the zero-free regions. 
% The key to applying the polynomial interpolation method is to establish the zero-free region.
Currently, the zero-free regions are primarily derived from the following methods. Asano contraction originated in ~\cite{Asano1970LeeYangTA} and refined in \cite{Ruelle2008CharacterizationOL, Liu2017TheIP} is a powerful tool to establish the zero-free region \cite{Chen2021SpectralIV, Guo2019ZerosOF}. Each step of Asano contraction contracts a vertex or an edge from the isolated vertices to the whole graph while preserving certain properties of the zero-free region.
For real stability, the operations preserving real stability are characterized in \cite{Borcea2007NegativeDA} which extends the results in \cite{Heilmann1972TheoryOM}.
Cluster expansion utilizes the recursion of the partition function to show that the marginal measures avoid $-1$ ~\cite{galvin2024zeroes, Patel2023ANZ}. The contraction method is to maintain a possible region of the marginal measure avoiding $-1$ such that the partition function does not vanish, the aforementioned correlation decay is a special case of the contraction method that extends the contraction property to the complex plane \cite{Shao2019ContractionAU,liu2019correlation}. 

% A common belief is that tools for designing approximate counting algorithms can also be adapted to prove zero-free region. 

% Compared to other algorithm design tools, zero-free regions are harder to establish because of the intrinsic complexity of dynamics in complex settings.

% And the common methods to derive zero-free regions are 

In this paper, we explore the relation between MCMC and zero-free regions. We show that we can lift the information percolation method which is originally designed to analyze the mixing time to the complex plane to prove zero-free regions.

Information percolation is first designed to analyze the cut-off phenomenon of the mixing time \cite{lubetzky2015exposition, lubetzky2016information}. The intuition of this method is that we can classify transitions as oblivious transitions and normal transitions. 
For oblivious transitions, the configuration is updated by a coin flip. For normal transitions, the configuration is updated through a measure defined by its neighbors' configurations. So for normal transitions, one needs to trace back to compute the neighbors' configurations to complete the transition. If the oblivious transitions are ``many enough'' then one can determine the configuration at time $n$ without tracing back to the starting time $1$, so that one can bound the mixing time. This kind of analysis successfully applies to problems in local lemma regime and also extends to the discrete Markov chains known as the systematic scan Glauber dynamics \cite{Vishesh21sampling,qiu2022perfect, HSW21,feng2023towards}.

\subsection{Our contributions}
We prove the Lee-yang zero-free region and the Fisher zero-free region for hypergraph independent set polynomials by lifting existing MCMC algorithms to the complex plane, which implies FPTASes by the polynomial interpolation method matching the lower bound in \cite{NPH}. We also provide an approximate counting method by enumerating. We show that the systematic scan Glauber dynamics converges in the same regime which to the best of our knowledge is the first result for the convergence of the complex dynamics.

\subsubsection{Zero-free region for hypergraph independence polynomial}
Since Sokal conjectured the zero-free region of independence polynomial in \cite{Sokal2000APL}, there are many results about it. Scott and Sokal showed a zero-free disk centred at the origin whose radius matches the Shearer's bound by a similar proof of the celebrated Lov\'asz local lemma \cite{Scott2003TheRL}. Peters and Regts finally proved a zero-free strip near the $[0, \lambda_c(\Delta))$ interval by lifting the correlation decay to the complex plane which proves Sokal's conjecture \cite{peter2019conjecture}. Later the location of complex roots is refined in \cite{Bencs2022OnCR}.

But for hypergraph independence polynomial, the existing zero-free region is far from the regime that we have FPTASes. For the general case, it is proved that there is a zero-free disk centred around the origin \cite{galvin2024zeroes},  essentially matching Shearer's bound for independence polynomials on graphs. They also conjectured a larger zero-free disk for linear hypergraphs but this was subsequently disproved by \cite{Zhang2023ANO}.

==> convergence.tex <==

% \begin{comment}
% \label{section:convergence}
% In this section, we show that 
% if the decay of bad tree (\Cref{definition:framework-bad-tree-decay}), zero-one law of the outcome (\Cref{definition:framework-zero-one-law-outcome}) and finiteness of bad trees (\Cref{definition:framework-finiteness-bad-trees}) hold, 
% under the conditions in \Cref{theorem:zero-freeness-his-lee-yang} or \Cref{theorem:zero-freeness-his-fisher}
% , the corresponding complex systematic scan Glauber dynamics converges. 

% \begin{theorem}[restatement of \Cref{theorem:convergence-area-complex-mcmc}]
% \label{theorem:restatement-convergence-area-complex-mcmc}
%  Suppose the conditions of \Cref{theorem:zero-freeness-his-lee-yang} or the conditions of \Cref{theorem:zero-freeness-his-fisher}, the corresponding complex systematic scan Glauber dynamics converges. Furthermore, $\forall \tau^* \in \{0,1\}^{\abs{V}}$ it holds that,
%  \[
%  \forall \tau  \in \-{supp}(\mu), \lim\limits_{T \to \infty} \abs{\mu^\-{GD}_{T, \tau}(\sigma_0 = \tau^*) - \mu(\tau^*)} = 0,
%  \]
%  which means that it converges to the stationary measure.
% \end{theorem}
\yxtodo{This outline will be changed after wcy finishing changing the section 3.3}
In this section, we prove \Cref{theorem:convergence-lee-yang} and \Cref{lemma:convergence-reduced-lee-yang}.
By the framework (\Cref{subsection:decomposition-schemes}), it suffices to check the condition of \Cref{lemma:framework-convergence-lemma}. We first give an abstract outline of how we check this. 

Recall \Cref{definition:bad-vertices-his}, we will work on $G_H^V$.
% Let stopping patterns be $\+P^* = \{(r_1, r_2, \dots, r_{p-1}) \mid p\le k, r_1, r_2, \dots, r_{p-1} \in \{0, \bot\}, \exists 1\le j \le p-1, r_j = 0\}$.  we collect some useful properties for the degree of $G_H^V$ and witness $2$-trees on it.

\begin{lemma}
\label{lemma:maximum-degree-witness-graph}
Let $H=(V, \+E)$ be a hypergraph  with maximum degree $\Delta$ and maximum edge size $k$.
In graph $G_H^V$, $\-{deg}(\ts(V, 0)) \le 2\abs{\+E} \Delta k^2$ and $\forall e \in V_H^V, e \neq \ts(V, 0)$, $\-{deg}(e) \le 2 \Delta k^2$.
\end{lemma}
\begin{proof}
    Recall \Cref{lemma:witness-graph-degree-bound}, $\-{deg}(\ts(V, 0)) \le \sum_{e \in \+E} \deg(\ts(e, 0)) \le 2 \abs{\+E} \Delta k^2$. For other vertices, the degree can only increase $1$ because we only add one vertex $\ts(V, 0)$.
\end{proof}


\begin{lemma}[construction of a maximal 2-tree in a connected graph with one large-degree vertex]
\label{lemma:2-tree-construction-one-large-degree}
Let $G = (V, E)$ be a connected graph. Let $v \in V$, $\text{deg}(v) = D$ and $\forall u \neq v, \text{deg}(u) \le d$. The algorithm in \Cref{definition:2-tree-construction} returns a 2-tree $\+T$ of $G$ containing $u$ such that $\abs{\+T} \ge \lfloor (\abs{V} - (D+1))/(d+1) \rfloor $.
\end{lemma}

\begin{proof}
    The algorithm is equal to removing $N^+(v)$ and then running the algorithm in \Cref{definition:2-tree-construction} on each connected component of the new graph.
\end{proof}

We will use the decomposition scheme to prove the following lemma. We defer its proof to the end of this section.

\begin{lemma}[decay of witness $2$-trees]
\label{lemma:convergence-decay-witness-2-tree}
Let $H=(V, \+E)$ be a hypergraph with maximum degree $\Delta$ and maximum edge size $k$. Fix $T \ge \abs{V}$. For a graphical model on $H$ with stationary measure $\mu$ and $q=2$, the $T$ step systematic scan Glauber dynamics is well-defined. Let $\+P^*$ be stopping patterns with respect to the dynamics. For a given witness $2$-tree $T^\-{wit}$, if there is $\*b \in \=C^{V_H^V}$, the stationary measure $\mu$ is decomposed by $\*b$ with parameters $(\ell^\-{pad}, \ell)$ and $\forall v \in V, b_v(1)=0$, let $A = \left(\ell^\-{pad}\right)^{-1} \ell^{4 \abs{\+E}^2 \Delta^2 k^5}$, then it holds,
    \[
    \sum\limits_{\substack{C: \=T(C)=T^\-{wit} \\ \tau \in \{0,1\}^C}} \abs{\mu_\infty^\-{GD}(\+T^\-{wit}=T^\-{wit}, \+C^\-{wit}=C, \sigma(C) = \tau)} \le A \left(\ell^\-{pad}\right)^{k\abs{T^\-{wit}}} \ell^{4 \Delta^2 k^5 \abs{T^\-{wit}}}.
    \]
\end{lemma}


Finally, we check that 
\[
\lim_{T\to \infty} A \sum\limits_{i \ge T/\abs{V}-1} \abs{\+T_i^\-{wit}} \left( \left(\ell^\-{pad}\right)^k \ell^{4 \Delta^2 k^5} \right)^i \to 0.
\]

We use next two lemmas to bound $\abs{\+T^\-{wit}_i}$.


% Now we bound the 2-tree in $G_H^*$ containing $\ts(V,0)$. 
\begin{corollary}
\label{corollary:2-tree-bound-extended-witness-graph}
Let $H=(V, \+E)$ be a hypergraph with maximum degree $\Delta$ and maximum edge size $k$.
The number of $2$-trees in $G_H^V$ of size $i \ge 2$ containing $\ts(V, 0)$ is at most
\[\binom{4 \abs{\+E}^2 \Delta^2 k^4 + i - 2}{4 \abs{\+E}^2 \Delta^2 k^4-1} (4 \mathrm{e} \Delta^2 k^4)^{i - 1}.\]
\end{corollary}
\begin{proof}
    % We first include the following lemma 
    Consider the graph $G_H^{V^2} = (V_H^V, E_H^{V^2})$ such that $(u, v) \in E_H^{V^2}$ if and only if $1\le\-{d}(u,v) \le 2$ in graph $G_H^V$. 
    Because $\ts(V, 0)$ must be in $2$-trees.
    Let $N(\ts(V,0))$ be the neighbors of $\ts(V,0)$ in $G_H^V$.
    We can remove $N(\ts(V,0))$ from $G_H^{V^2}$ to form a new graph $G_H^{\top} = G_H^{V^2}[V_H^V \backslash N(\ts(V, 0)) ]=(V_H^{\top}, E_H^{\top})$.  Any $2$-tree containing $\ts(V,0)$ in $G_H^V$ is a subtree containing $\ts(V, 0)$ in $G_H^{\top}$. It suffices to bound the number of subtrees containing $\ts(V, 0)$ in $G_H^{\top}$.
    % \yxtodo{Give a general lemma here.}
    
    By \Cref{lemma:witness-graph-degree-bound}, for the graph $G_H^{\top}$, $\-{deg}(\ts(V, 0)) \le 4 \abs{\+E}^2 \Delta^2 k^4$ and $\forall u \in V_H^\top, u \neq \ts(V, 0)$, $\-{deg}(u) \le 4\Delta^2 k^4$. By \Cref{lemma:subtree-bound-large-degree}, the number of subtrees containing $\ts(V,0)$ in $G_H^\top$ of size $i\ge 2$ is bounded by 
    \[\binom{4 \abs{\+E}^2 \Delta^2 k^4 + i - 2}{4 \abs{\+E}^2 \Delta^2 k^4-1} (4 \mathrm{e} \Delta^2 k^4)^{i - 1}.\]
\end{proof}

\subsection{Dynamics on Lee-Yang zeros}
% Now we establish the decomposition scheme  (\Cref{definition:decomposition-scheme}).
% \yxtodo{Need to establish the decay of witness 2 trees.}
% For the systematic scan Glauber dynamics on Lee-Yang zeros, we first establish the decomposition scheme, we set the lower bound measure $\mu^\-{ly, LB}$ as,

% \[\mu^\-{ly, LB}_v(0)=\frac{1}{1+\lambda_v}, \quad \mu^\-{ly, LB}_v(1)=0, \quad \mu^\-{ly, LB}_v(\bot) = \frac{\lambda_v}{1+\lambda_v}.\]

% By \Cref{lemma:his-ly-bound-l-l-pad}, we know have bounds for the maximum padding total norm $\ell^\-{ly, pad}$ and the maximum total norm $\ell^\-{ly}$,
% \[
% \ell^\-{ly, pad}\le \left(2\mathrm{e}\Delta k^2\right)^{-2/k}, \quad \ell^\-{ly} \le \frac{1 + \varepsilon}{1 - \varepsilon}.
% \]

\begin{comment}
For the systematic scan Glauber dynamics on Fisher zeros, we set the lower bound measure $\ell^\-{fs, LB}$ as,

\[
\mu^\-{fs, LB}_v(0)=\frac{1}{2}, \quad \mu^\-{fs, LB}_v(1)=0,\quad \mu^\-{fs, LB}_v(\bot) = \frac{1}{2}.
\]

We have the next lemma to bound $\ell^\-{fs, pad}$ and $\ell^\-{fs}$.

\yxtodo{This lemma is under construction.}
\begin{lemma}[bounds on $\ell^\-{fs, pad}$ and $\ell^\-{fs}$]
\label{lemma:convergence-bound-fs-l-l-pad}
    Suppose the condition of \Cref{theorem:convergence-fisher}, it holds that,
    \[
    \ell^\-{fs, pad} \le \frac{1}{2} + 6 \varepsilon,\quad \ell^\-{fs} \le 1 + 6 \varepsilon.
    \]
\end{lemma}
\begin{proof}[Proof of \Cref{lemma:convergence-bound-fs-l-l-pad}]
    We first analyze the transition measure. Given $v$ and $\sigma_{V \backslash \{v\}}$, let $\tilde{E}(v, \sigma_{V \backslash \{v\}}) = \{e \mid \forall u, v \in e, u\neq v, \sigma_u = 1\}$.
    \[
    \mu^{\sigma_{V \backslash \{v\}}}_v(0) = \frac{1}{1 + \prod_{e\in \tilde{E}(v, \sigma_{V \backslash \{v\}})} \beta_e },\quad \mu^{\sigma_{V \backslash \{v\}}}_v(1)=\frac{\prod_{e\in \tilde{E}(v, \sigma_{V \backslash \{v\}})} \beta_e}{1 + \prod_{e\in \tilde{E}(v, \sigma_{V \backslash \{v\}})} \beta_e}.
    \]
    So, 
    \[
    \ell^\-{fs, pad} = \max_{v, \sigma_{V \backslash \{v\}}} \left( \abs{\frac{1}{1 + \prod_{e\in \tilde{E}(v, \sigma_{V \backslash \{v\}})} \beta_e }-\frac{1}{2}} + \abs{\frac{\prod_{e\in \tilde{E}(v, \sigma_{V \backslash \{v\}})} \beta_e}{1 + \prod_{e\in \tilde{E}(v, \sigma_{V \backslash \{v\}})} \beta_e}} \right).
    \]
    Let $v$ and $\sigma_{V \backslash \{v\}}$ be the parameters that maximize $\ell^\-{fs, pad}$. Let $\+R = \prod_{e \in \tilde{E}(v, \sigma_{V \backslash \{v\}})}\beta_e$. So
    \[
    \ell^\-{fs, pad} = \abs{\frac{1}{1+\+R}-\frac{1}{2}} + \abs{\frac{\+R}{1 + \+R}} = \abs{\frac{1 - \+R}{2(1 + \+R)}} + \abs{\frac{\+R}{1 + \+R}} = \frac{\abs{1 - \+R} + 2\abs{\+R}}{\abs{2(1 + \+R)}}.
    \]
    Next, we show that 
    \[
    \+R \in \{(x, y) \mid -2\varepsilon \le x \le 1 + 2 \Delta \varepsilon, \abs{y} \le 2\varepsilon \}.
    \]
    
    For the real part of $\+R$, $\`R(\+R) = \`R(\prod_{e \in \tilde{E}(v, \sigma_{V \backslash \{v\}})} \beta_e) \le (1 + \varepsilon)^{\Delta} \le \exp(\varepsilon \Delta) \le 1 + 2 \Delta \varepsilon$. $\`R(\+R) \ge -\varepsilon (1 + \varepsilon)^{\Delta - 1} \ge -\varepsilon \exp(\varepsilon(\Delta-1)) \ge -2 \varepsilon$.

    For the imaginary part of $\+R$,$\abs{\`I(\+R)} \le 2\varepsilon(1 + \varepsilon)^{\Delta -1} \le 4 \varepsilon$.

    Let $\+R^*$ be the nearest point in $[0, 1 + 2 \Delta \epsilon]$ to $\+R$.

    \[
    \ell^\-{fs, pad} \le \frac{\abs{1-\+R^*} + 4\varepsilon + 2 \+R^* + 8\varepsilon}{2(1 + \+R^* - 4 \varepsilon)}.
    \]
    When $\+R^* > 1$, 
    \[
    \ell^\-{fs, pad} \le \frac{2 \Delta \varepsilon + 4\varepsilon + 2 \+R^* + 8\varepsilon}{2(1 + \+R^* - 4 \varepsilon)}=
    \]
\end{proof}
\end{comment}



% Now it is ready to prove \Cref{theorem:convergence-lee-yang}.
\begin{proof}[Proof of \Cref{theorem:convergence-lee-yang}]
For the systematic scan Glauber dynamics on Lee-Yang zeros, we set the $\*b$ in \Cref{definition:decomposition-scheme} as,

\[b_v(0)=\frac{1}{1+\lambda_v}, \quad b_v(1)=0, \quad b_v(\bot) = \frac{\lambda_v}{1+\lambda_v}.\]

By \Cref{lemma:his-ly-bound-l-l-pad}, we know have bounds for the maximum padding total norm $\ell^\-{pad}$ and the maximum total norm $\ell^\-{ly}$,
\[
\ell^\-{pad}\le \left(2\mathrm{e}\Delta k^2\right)^{-2}, \quad \ell \le \frac{1 + \varepsilon}{1 - \varepsilon}.
\]

By \Cref{lemma:convergence-decay-witness-2-tree}, it holds that,
\[
\sum\limits_{\substack{C: \=T(C)=T^\-{wit} \\ \tau \in \{0,1\}^C}} \abs{\mu_\infty^\-{GD}(\+T^\-{wit}=T^\-{wit}, \+C^\-{wit}=C, \sigma(C) = \tau)} \le A \left(\ell^\-{pad}\right)^{\abs{T^\-{wit}}} \ell^{4 \Delta^2 k^5 \abs{T^\-{wit}}}.
\]

By \Cref{corollary:2-tree-bound-extended-witness-graph}, it holds that,
\[
\abs{\+T^\-{wit}_i} \le \binom{4 \abs{\+E}^2 \Delta^2 k^4 + i - 2}{4 \abs{\+E}^2 \Delta^2 k^4-1} \left(4 \mathrm{e} \Delta^2 k^4\right)^{i - 1}.
\]
Finally,
\begin{align*}
&A \sum\limits_{i \ge T/\abs{V}-1} \abs{\+T_i^\-{wit}} \left( \ell^\-{pad} \ell^{4 \Delta^2 k^5} \right)^i\\
    (\text{by \Cref{lemma:his-lee-yang-bad-tree-decay}})\quad \le&
A
\sum\limits_{i\ge T/\abs{V} - 1}
\abs{\+T_i^\-{wit}}
\left( 8 \mathrm{e} \Delta^2 k^4 \right)^{-i}
\\
(\text{by \Cref{corollary:2-tree-bound-extended-witness-graph}})\quad\le&
A
\sum\limits_{i\ge T/\abs{V} - 1}
\binom{4 \abs{\+E}^2 \Delta^2 k^4 + i - 2}{4 \abs{\+E}^2 \Delta^2 k^4 - 1} \left(4 \mathrm{e} \Delta^2 k^4 \right)^{i - 1}
\left( 8 \mathrm{e} \Delta^2 k^4 \right)^{-i}
\\
\le&
A
\sum\limits_{i\ge T/\abs{V} - 1}
\binom{4 \abs{\+E}^2 \Delta^2 k^4 + i - 2}{4 \abs{\+E}^2 \Delta^2 k^4 - 1} 2^{-i}
\\
(\text{when $T$ is sufficiently large})\le&
A
\sum\limits_{i\ge T/\abs{V} - 1}
\left(4 \abs{\+E}^2 \Delta^2 k^4 + i - 2\right)^{4 \abs{\+E}^2 \Delta^2 k^4}
2^{-i},
\end{align*}
whose limit is $0$ as $T \to \infty$. So by the \Cref{lemma:framework-convergence-lemma}, the associating systematic scan Glauber dynamics is convergent.

Also by \Cref{theorem:zero-freeness-his-lee-yang}, we know that in the same regime, the partition function is non-zero, so the stationary measure is well-defined and the associating systematic scan Glauber dynamics converges to the stationary measure.
\end{proof}

% Now we give the proof of \Cref{lemma:convergence-marginal-bad-tree-decay}. The proof almost follows that of \Cref{lemma:framework-marginal-lower-bound-to-bad-tree-decay}.

\subsection{Dynamics on Fisher zeros}

Under the condition of \Cref{theorem:zero-freeness-his-fisher}, we prove the next lemma.

\begin{lemma}
\label{lemma:convergence-reduced-lee-yang}
Let $H=(V, \+E)$ be a $k$-uniform hypergraph with maximum degree $\Delta$. Let $\varepsilon = \varepsilon_{k, \Delta}$ and $\+D_\varepsilon$ be as defined in \Cref{theorem:zero-freeness-his-fisher}. For any $\*\beta \in \+D_\varepsilon^{\+E}$, let $(H^*=(V^*, \+E^*), \*\lambda) = \+M(H, \*\beta)$ where $\+M$ is defined in \Cref{lemma:reduction-lee-yang-fisher}. Then $Z^\-{ly}_H(\*\lambda)$ is non-zero and the associated systematic scan Glauber dynamics converges to the stationary measure.
    % Suppose the condition of \Cref{theorem:zero-freeness-his-fisher}, let $\+G^\-{fs} = (H=(V, \+E), 1^{\abs{V}}, \*\beta)$ be the hypergraph independent set model on Fisher zeros. Let $\+G^\-{ly} = \+M(\+G^\-{fs}) = (H^*=(V^*, \+E^*), \*\lambda, 1^{\abs{\+E^*}})$ be the model on Lee-Yang zeros after the reduction in \Cref{lemma:reduction-lee-yang-fisher}, then the systematic scan Glauber dynamics of $\+G^\-{ly}$ converges to its stationary measure.
\end{lemma}
\begin{proof}
we set the $\*b^*$ (\Cref{definition:decomposition-scheme}):

\[
b^*_v(0)=\frac{1}{1+\lambda_v}, \quad b^*_v(1)=0,\quad b^*_v(\bot)=\frac{\lambda_v}{1+\lambda_v}.
\]

By \Cref{lemma:reduced-lee-yang-bound-l-pad-l}, we know that
    \[\ell^\-{*, pad} \le (1+2\varepsilon) \left(\frac{1}{2}\right)^k,\quad \ell^\-{*} \le 1 + 4\varepsilon.\]

By \Cref{lemma:convergence-decay-witness-2-tree} and \Cref{observation:reduced-lee-yang}, let $A = \left(\ell^{*,\-{pad}}\right)^{-1} \ell^{4 \abs{\+E}^2 \Delta^2 (k+1)^5}$ it holds that,

\[
\sum\limits_{\substack{C: \=T(C)=T^\-{wit} \\ \tau \in \{0,1\}^C}} \abs{\mu_\infty^\-{GD}(\+T^\-{wit}=T^\-{wit}, \+C^\-{wit}=C^\-{wit}, \sigma(C) = \tau)} \le A \left(\ell^\-{*, pad}\right)^{\abs{T^\-{wit}}} \left(\ell^\-{*}\right)^{4 \Delta^2 (k+1)^5 \abs{T^\-{wit}}}.
\]

By \Cref{corollary:2-tree-bound-extended-witness-graph} and \Cref{observation:reduced-lee-yang}, it holds that,
\[
\abs{\+T^\-{wit}_i} \le \binom{4 \abs{\+E^*}^2 \Delta^2 (k+1)^4 + i - 2}{4 \abs{\+E^*}^2 \Delta^2 (k+1)^4-1} \left(4 \mathrm{e} \Delta^2 (k+1)^4\right)^{i - 1}.
\]

Finally,
\begin{align*}
&A \sum\limits_{i \ge T/\abs{V}-1} \abs{\+T_i^\-{wit}} \left( \ell^\-{pad} \ell^{4 \Delta^2 (k+1)^5} \right)^i\\
    (\text{by \Cref{lemma:reduced-lee-yang-bad-tree-decay}})\quad \le&
A
\sum\limits_{i\ge T/\abs{V} - 1}
\abs{\+T_i^\-{wit}}
\left( 4 \Delta^2 (k+1)^4 \right)^{-i}
\\
\le&
A
\sum\limits_{i\ge T/\abs{V} - 1}
\binom{4 \abs{\+E}^2 \Delta^2 (k+1)^4 + i - 2}{4 \abs{\+E}^2 \Delta^2 (k+1)^4 - 1} \left(4 \mathrm{e} \Delta^2 (k+1)^4\right)^{i - 1}
\left( 8 \Delta^2 (k+1)^4 \right)^{-i}
\\
\le&
A
\sum\limits_{i\ge T/\abs{V} - 1}
\binom{4 \abs{\+E}^2 \Delta^2 (k+1)^4 + i - 2}{8 \abs{\+E}^2 \Delta^2 (k+1)^4 - 1} 2^{-i}
\\
(\text{when $T$ is sufficiently large})\le&
A
\sum\limits_{i\ge T/\abs{V} - 1}
\left(4 \abs{\+E}^2 \Delta^2 (k+1)^4 + i - 2\right)^{8 \abs{\+E}^2 \Delta^2 (k+1)^4}
2^{-i},
\end{align*}
whose limit is $0$ as $T \to \infty$. So by the \Cref{lemma:framework-convergence-lemma}, the associating systematic scan Glauber dynamics is convergent.
Also by \Cref{theorem:zero-freeness-his-fisher} and \Cref{lemma:reduction-lee-yang-fisher}, we know that in the same regime, partition function is non-zero, so the stationary measure is well-defined, so the associating systematic scan Glauber dynamics converges to the staionary measure.
\end{proof}

% \begin{proof}[Proof of \Cref{theorem:convergence-fisher}]
% For the systematic scan Glauber dynamics on Lee-Yang zeros, we first establish the decomposition scheme, we set the lower bound measure $\mu^\-{fs, LB}$ as,
% \[
% \mu^{\-{fs, LB}}(0) = \frac{1}{2}, \quad \mu^{\-{fs, LB}}(1) = 0, \quad \mu^{\-{fs, LB}}(\bot) = \frac{1}{2}.
% \]
% By \Cref{lemma:his-fisher-bound-fs-l-l-pad}, we know that 
% \[
%     \ell^\-{fs, pad} \le \frac{1}{2} + 6 \Delta \varepsilon,\quad \ell^\-{fs} \le 1 + 6 \Delta \varepsilon.
% \]
% % Now it is ready to prove \Cref{theorem:convergence-fisher}.

% By \Cref{lemma:convergence-decay-witness-2-tree}, it holds that,
% \[
% \sum\limits_{\substack{C: \=T(C)=T^\-{wit} \\ \tau \in \{0,1\}^C}} \abs{\mu_\infty^\-{GD}(\+T^\-{wit}=T^\-{wit}, \+C^\-{wit}=C^\-{wit}, \sigma(C) = \tau)} \le A \left(\ell^\-{fs, pad}\right)^{k\abs{T^\-{wit}}} \left(\ell^\-{fs}\right)^{4 \Delta^2 k^5 \abs{T^\-{wit}}}.
% \]

% By \Cref{corollary:2-tree-bound-extended-witness-graph}, it holds that,
% \[
% \abs{\+T^\-{wit}_i} \le \binom{4 \abs{\+E}^2 \Delta^2 k^4 + i - 2}{4 \abs{\+E}^2 \Delta^2 k^4-1} (4 \mathrm{e} \Delta^2 k^4)^{i - 1}.
% \]
% Finally,
% \begin{align*}
% &A \sum\limits_{i \ge T/\abs{V}-1} \abs{\+T_i^\-{wit}} \left( \left(\ell^\-{pad}\right)^k \ell^{4 \Delta^2 k^5} \right)^i\\
%     (\text{by \Cref{lemma:his-fisher-bad-tree-decay}})\quad \le&
% A
% \sum\limits_{i\ge T/\abs{V} - 1}
% \abs{\+T_i^\-{wit}}
% \left( 4 \Delta^2 k^4 \right)^{-i}
% \\
% (\text{by \Cref{corollary:2-tree-bound-extended-witness-graph}})\quad\le&
% A
% \sum\limits_{i\ge T/\abs{V} - 1}
% \binom{4 \abs{\+E}^2 \Delta^2 k^4 + i - 2}{4 \abs{\+E}^2 \Delta^2 k^4 - 1} (4 \mathrm{e} \Delta^2 k^4)^{i - 1}
% \left( 4 \Delta^2 k^4 \right)^{-i}
% \\
% \le&
% A
% \sum\limits_{i\ge T/\abs{V} - 1}
% \binom{4 \abs{\+E}^2 \Delta^2 k^4 + i - 2}{4 \abs{\+E}^2 \Delta^2 k^4 - 1} 2^{-i}
% \\
% (\text{when $T$ is sufficiently large})\le&
% A
% \sum\limits_{i\ge T/\abs{V} - 1}
% \left(\frac{4 \abs{\+E}^2 \Delta^2 k^4 + i - 2}{4 \abs{\+E}^2 \Delta^2 k^4 - 1}\right)^{4 \abs{\+E}^2 \Delta^2 k^4}
% 2^{-i},
% \end{align*}
% whose limit is $0$ as $T \to \infty$. So by the \Cref{lemma:framework-convergence-lemma}, the associating systematic scan Glauber dynamics is convergent.
% Also by \Cref{theorem:zero-freeness-his-fisher}, we know that in the same regime, partition function is non-zero, so the stationary measure is well-defined, so the associating systematic scan Glauber dynamics converges to the staionary measure.
% \end{proof}
\subsection{Omitted proofs}
% In this subsection, we now get the omitted proof of \Cref{lemma:convergence-decay-witness-2-tree}.

% Given $\+T^\-{wit} = T^\-{wit}$, let $U = T^\-{wit} \cup N^2(T)$, $T^* = T^\-{wit} \backslash \{\ts(V, 0)\}$. Note $U$ contains all vertices for all possible witness components and their neighbors due to \Cref{definition:stationary-start} and \Cref{definition:framework-witness-component-2-trees}.

% % We sort the timestamps in $U$ forming a sequence $\-{TP} = (t_1, t_2, \dots, t_m)$ such that $t_1 < t_2 < \dots < t_m$.
% Recall the decomposed systematics scan Glauber dynamics (\Cref{Alg:complex-GD-decomposed}), each timestamp $t$ is associated with $r_t$ and $c_t$. 
% % We define the vector form of $r$'s and $c$'s as $\vec{r} = (r_{t_1},r_{t_2}, \dots, r_{t_m})$, $\vec{c} = (c_{t_1}, c_{t_2}, \dots, c_{t_m})$.
% Let $X \subseteq V_H^V$, we define two functions $\*r^X:X \to \{0, \bot\}$ and $\*c^X: X \to \{0, 1\}$. For $X \subseteq Y \subseteq V_H^V$ We denote $\text{ex}(\*r^X, Y)$ be the set of all possible function $\*r^Y$ such that $\forall t \in X, r^X(t)=r^Y(t)$ and $\text{ex}(\*c^X, Y)$ similarly. Let $Y \subseteq X$, we also define $\text{res}(\*r^X, Y)$ be the function $\*r^Y$ such that $\forall t \in Y, r^X(t) = r^Y(t)$, we define $\text{res}(\*c^X, Y)$ similarly. We write $\*r$ instead of $\*r^X$ when its domain is clear from the context.

% Note if $\*c^C$ is fixed, the configuration on $C$ is fixed.
% We abuse the notation a little, let $\mu^{\*r, \*c, \bot}_{v_{i(t_i)}}(c({t_i}))$ be the measure condition on $\*r, \*c$ except $r_{t_i}$ and $c_{t_i}$ as \Cref{definition:decomposition-scheme}.  
% We say $t \in T$ if $\exists v \in T \text{ s.t. } t \in v$ and $t \in C$ if $\exists v \in C \text{ s.t. } t\in v$.

% % Define 
% % \[ \Omega_T = \{(\vec{r}, \vec{c}) \mid (\vec{r}, \vec{c}) \in \{0, \bot\}^{U} \times \{0, 1\}^U, \forall t_i \in T, r_{i}=\bot \}. \]
% % % We claim that in our applications we set $\mu$
% % be the set containing all possible $(\vec{r},\vec{c})$'s on $U$, note this set is finite due to the size limit of witness component given the witness $2$-tree. 
% Define $\Omega_T$ be the set of all functions $\*r^U$ such that for timestamps in $T^*$, $r=\bot$, i.e.,
% \[ \Omega_T = \left\{\*r^U \mid \forall t_i \in T^*, r(t_i)=\bot \right\}, \]
% % be the set containing all possible $(\*r,\*c)$'s on $U$, note this set is finite due to the size limit of witness component given the witness $2$-tree.

% For $T^*$, let 
% \[A = \prod_{t\in T^*} \left(\max\limits_{\*r^U, \*c^U} \left(\abs{\mu^{\*r, \*c, \bot}_{v_{i(t)}}(0)} + \abs{\mu^{\*r, \*c, \bot}_{v_{i(t)}}(1)}\right) \abs{b_{v_{i(t)}}(\bot)}  \right) = \prod_{t\in T^*} \ell^\-{pad}_{v_{i(t)}},\]
% \[
% B(U) = 
% A
% \prod_{t\in U \backslash T^*} \left( \abs{b_{v_{i(t)}}(0)} + \max\limits_{\*r^U, \*c^U} \left(\abs{\mu^{\*r, \*c, \bot}_{v_{i(t)}}(0)} + \abs{\mu^{\*r, \*c, \bot}_{v_{i(t)}}(1)}\right) \abs{b_{v_{i(t)}}(\bot)} \right) = A \prod_{t \in U \backslash T^*} \ell_{v_{i(t)}}.
% \]

% By the assumpstion in \Cref{lemma:bad-tree-decay}, $B(U) \le \left(\ell^\-{pad}\right)^{\abs{T^*}} \ell^{k\abs{U \backslash T^*}}$. We define
% \[
% B_{\*r^{U}}(U) = A \prod_{t\in U \backslash T^*} \left( \abs{b_{v_{i(t)}}(0)} \=I[r(t)=0] + \max\limits_{\substack{\*r' \in \text{ex}(\*r, V_H^V) \\  \*c^{V_H^V}}} \left(\abs{\mu^{\*r', \*c, \bot}_{v_{i(t)}}(0)} + \abs{\mu^{\*r', \*c, \bot}_{v_{i(t)}}(1)}\right) \abs{b_{v_{i(t)}}(\bot)} \=I[r(t)=\bot] \right),
% \]

% It holds that $B(U) \ge \sum_{\*r \in \Omega_T} B_{\*r}(U)$.

% \begin{lemma}
% \label{lemma:witness-tree-decay-fix-r}
% Given a witness $2$-tree $T^\-{wit}$, a witness component $C$ and a function $\*r'{^{N^{+}(C)}}$, suppose the conditions in \Cref{lemma:convergence-decay-witness-2-tree}, it holds that,
% \[\sum\limits_{\tau \in \{0,1\}^{\abs{C}}}\abs{\mu_T^\-{GD}(\+T^\-{wit} = T^\-{wit}, \+C^\-{wit}=C, \sigma_C = \tau, \*r')} \le \sum\limits_{\*r \in \text{ex}(\*r', U)} B_{\*r'}(U).\]
% \end{lemma}
% % \begin{proof}
% \begin{proof}
% Given a witness $2$-tree $T^\-{wit}$, a witness component $C$, configuration on it $\tau \in \{0,1\}^C$ and a function $\*r'{^{N^{+}(C)}}$. We can upper bound 
% \[\abs{\mu_T^\-{GD}(\+T^\-{wit} = T^\-{wit}, \+C^\-{wit}=C, \sigma_C = \tau, \*r')},\]
% by the following procedure:
% \yxtodo{under construction}
% \begin{enumerate}
%     \item enumerate all timestamps in $N^+(C)$ by an arbitrary order, let $\*c^C$ satisfying $\forall t \in C$, $c(t) = \tau_t$;
%     \item for a timestamp $t$, let $v = v_{t}$,
%     \begin{itemize}
%         % \item if $i$ is in $T^\-{bad}$, it contributes at most $\abs{\mu^\-{LB}_{v}(\bot)} \max_{\tau' \in \{0,1\}^{V\backslash v}}\abs{\mu_v^{\tau'}(\tau_v)}$.
%         \item if $t$ is in $\ts(V, 0)$, it contributes at most $\abs{b_{v}(0)}\=I(r_t=0) + \abs{\mu_v^{\*r', \*c, \bot}(\tau_t)}\=I(r_t = \bot)$
%         \item if $t$ is in $C$ and $t \notin \ts(V, 0)$, it contributes at most $\abs{b_{v}(\bot) \mu_v^{\*r', \*c, \bot}(\tau_t) } $.
%         \item if $t$ is in the neighbor of $C$, it contributes at most $\abs{b_v(r(t))}$.
%     \end{itemize}
% \end{enumerate}

% Then, we take the enumeration of $\tau$ into consideration,
% for all $t$'s are in $N(C)$, their contributes are at most $\prod_{t\in N(C)} \abs{b_{v_{i(t)}}(r(t))} $.
% For all $t$'s are in $\ts(V, 0)$, they contribute at most 
% \[F \defeq \prod_{t \in \ts(V,0)}\left(\abs{b_{v_{i(t)}}(0)} + \max_{\*c^{C}} \left(\abs{\mu_{v_{i(t)}}^{\*r', \*c, \bot}(0)} + \abs{\mu_{v_{i(t)}}^{\*r', \*c, \bot}(1)}\right) \cdot \abs{b_{v_{i(t)}}(\bot)}\right),\]

% and we denote this quantity by $F$.

% For timestamps that are in $C \backslash \ts(V,0)$, their contributions are at most 
% % $\max_{\*c^{C}} \left(\abs{\mu_v^{\*r', \*c, \bot}(0)} + \abs{\mu_v^{\*r', \*c, \bot}(1)}\right) \cdot \abs{b_v(\bot)}$. 

% \[J \defeq \prod_{t \in C\backslash \ts(V,0)} \left(\max_{\*c^{C}} \left(\abs{\mu_{v_{i(t)}}^{\*r', \*c, \bot}(0)} + \abs{\mu_{v_{i(t)}}^{\*r', \*c, \bot}(1)}\right) \cdot \abs{b_{v_{i(t)}}(\bot)}\right),\]
% and we denote this quantity by $J$.

% So 
% \[\sum\limits_{\tau \in \{0,1\}^{\abs{C}}}\abs{\mu_T^\-{GD}(\+T^\-{bad} = T, \+C^\-{bad}=C, \sigma_C = \tau, \*r')} \le A \cdot F \cdot J \cdot \prod\limits_{t\in N(C)}\abs{b_{v_{i(t)}}(r'(t))}. \]
% % is bounded by 
% % \[A \cdot F \cdot J \cdot \prod\limits_{t\in N(C)}\abs{b_{v_{i(t)}}(r'(t))} .\]
% % \[A \prod\limits_{t \in C \backslash T} \left(\left(\abs{\mu^{\*r, \*c, \bot}_{v_{i(t)}}(0)} + \abs{\mu^{\*r, \*c, \bot}_{v_{i(t)}}(1)}\right) \abs{b_{v_{i(t)}}(\bot)} \right) \prod\limits_{t\in N(C)}\abs{b_{v_{i(t)}}(r'(t))} .\]

% Let 
% \[
% E \defeq A \cdot F \cdot J.
% \]

% It holds that,
% \begin{align*}
% \sum\limits_{\*r \in \text{ex}(\*r', U)} B_{\*r'}(U) &= E 
% \prod\limits_{\substack{t\in N(C) \\ r'(t)=0}}\abs{b_{v_{i(t)}}(0)}
% \left(\prod\limits_{\substack{t\in N(C) \\ r'(t)=\bot}}\abs{b_{v_{i(t)}}(\bot)}\left( \max_{\*c^{V_H^S}} \left(\abs{\mu_{v_{i(t)}}^{\*r', \*c, \bot}(0)} + \abs{\mu_{v_{i(t)}}^{\*r', \*c, \bot}(1)}\right) \right)\right)
% \prod_{t \in U \backslash N^+(C)} \ell_{v_{i(t)}} \\
% &\ge E 
% \prod\limits_{\substack{t\in N(C) \\ r'(t)=0}}\abs{b_{v_{i(t)}}(0)}
% \left(\prod\limits_{\substack{t\in N(C) \\ r'(t)=\bot}}\abs{b_{v_{i(t)}}(\bot)}\left( \max_{\*c^{V_H^S}} \left(\abs{\mu_{v_{i(t)}}^{\*r', \*c, \bot}(0)} + \abs{\mu_{v_{i(t)}}^{\*r', \*c, \bot}(1)}\right) \right)\right)
% \\
% &\ge E 
% \prod\limits_{\substack{t\in N(C) \\ r'(t)=0}}\abs{b_{v_{i(t)}}(0)}
% \left(\prod\limits_{\substack{t\in N(C) \\ r'(t)=\bot}}\abs{b_{v_{i(t)}}(\bot)}\right) \\
% &\ge 
% \sum\limits_{\tau \in \{0,1\}^{\abs{C}}}\abs{\mu_T^\-{GD}(\+T^\-{bad} = T, \+C^\-{bad}=C, \sigma_C = \tau, \*r')}
% \end{align*}
% The first inequality is due to $\ell_v \ge 1$, the second inequality is due to the triangle inequality.
% % \[
% % \sum\limits_{\*r \in \text{ex}(\*r', U)} B_{\*r'}(U) = E 
% % \prod\limits_{\substack{t\in N(C) \\ r'(t)=0}}\abs{b_{v_{i(t)}}(0)}
% % \prod\limits_{\substack{t\in N(C) \\ r'(t)=\bot}}\abs{b_{v_{i(t)}}(\bot)\left( \max_{\*c^{V_H^S}} \left(\abs{\mu_{v_{i(t)}}^{\*r', \*c, \bot}(0)} + \abs{\mu_{v_{i(t)}}^{\*r', \*c, \bot}(1)}\right) \right)}
% % \prod_{t \in U \backslash N^+(C)} \ell_{v_{i(t)}}.
% % \]

% \end{proof}

% % Now let $R_i = \{ (\text{res}(\*r^U, \{t_1, t_2, \dots, t_i\}, \text{res}(\*c^U, \{t_1, t_2, \dots, t_i\}) \mid (\*r^U, \*c^U) \in \Omega_T\}$ be the set containing all possible $r$'s and $\tau$'s of the first $i$ timestamps in the order of $\-{TP}$.
% % We give following useful functions:

% % \[f(\*r, \*c, t) = \abs{b_{v_{i(t)}}(0)}\cdot \=I[r_t = 0] + \max\limits_{\substack{
% % \*r' \in \text{ex}(\*r, V_H^S) \\
% % \*c' \in \text{ex}(\*c, V_H^S)
% % }}\abs{\mu_{v_{i(t)}}^{\bot, \*r', \*c'}(c_{t}) b_{v_{i(t)}}(\bot)} \cdot \=I[r_t = \bot], \]

% % $f$ indicates the maximal norm of all possible transitions for timestamp $t_j$ under $\*r$ and $\*c$.

% % For $S\subseteq U$, let 
% % \[
% % F(\*r, \*c, S) = \prod\limits_{t_j \in S}f(\*r, \*c, t_j).
% % \]

% % \[
% % g(\*r, t) = \abs{b_{v_{i(t)}}(0)} \cdot \=I[r_t = 0] + \abs{b_{v_{i(t)}}(\bot)} \cdot \=I[r_t = \bot],
% % \]

% % $g$ indicates the maximal norm of possible ``coin flip'' transitions using only $r$'s.

% % For $S\subseteq U$, let 
% % \[
% % G(\*r, S) = \prod\limits_{t_j \in S}g(\*r, t_j).
% % \]

% % % Now let $R_i = \{\{(r_1,\tau_{1}), (r_2,\tau_2), \dots, (r_i,\tau_i)\} \mid (\vec{r}, \vec{\tau}) \in \Omega_T\}$ be the set containing all possible $r$'s and $\tau$'s of the first $i$ timestamps in the order of $\-{TP}$.

% % % We give following useful functions:

% % % \[f(\vec{r}, \vec{c}, j) = \abs{\mu^\-{LB}_{v_{i(t_j)}}(0)}\cdot \=I[r_j = 0] + \max\limits_{
% % % \substack{\vec{r}'\in\{0, \bot\}^{\abs{V_S^V}}, \vec{r}'_{U}=\vec{r} \\
% % % \vec{c}'\in\{0, 1\}^{\abs{V_S^V}}, \vec{c}'_{U}=\vec{c}
% % % }}\abs{\mu_{v_{i(t_j)}}^{\-{pad}, \vec{r}', \vec{c}'}(c_j) \mu_{v_{i(t_j)}}^\-{LB}(\bot)} \cdot \=I[r_j = \bot], \]

% % % $f$ indicates the maximal norm of all possible transitions for timestamp $t_j$ under $\vec{r}$ and $\vec{c}$.

% % % For $S\subseteq U$, let 
% % % \[
% % % F(\vec{r}, \vec{c}, S) = \prod\limits_{t_j \in S}f(\vec{r}, \vec{c}, j).
% % % \]

% % % \[
% % % g(\vec{r}, j) = \abs{\mu_{v_{i(t_j)}}^\-{LB}(0)} \cdot \=I[r_j = 0] + \abs{\mu_{v_{i(t_j)}}^\-{LB}(\bot)} \cdot \=I[r_j = \bot],
% % % \]

% % % $g$ indicates the maximal norm of possible ``coin flip'' transitions using only $r$'s.

% % % For $S\subseteq U$, let 
% % % \[
% % % G(\vec{r}, S) = \prod\limits_{t_j \in S}G(\vec{r}, j).
% % % \]

% % Set 

% % \[
% % A_i = \sum\limits_{(\*r,\*c) \in R_i} \prod\limits_{j \le i} f(\*r, \*c, t_j).
% % \]


% % We give following two lemmas to establish decay of witness $2$-trees.

% % \begin{lemma}
% % \label{lemma:decay-witness-2-tree-am-upper-bound}
% % Suppose the assumptions in \Cref{lemma:convergence-decay-witness-2-tree}, it holds that,

% %     \[
% %     A_m \le  \left(\ell^\-{pad}\right)^{\abs{T^*}}\ell^{k \abs{N^2(T)} + \abs{V}}.
% %     \]
% % \end{lemma}
% % \begin{proof}

% % We now show that $A_m \le \left( \ell^\-{pad} \right)^{\abs{T^*}} \ell^{k \abs{N^2(T)} + \abs{V}}$ by the induction on $m$. Let $\-{wit}(i)$ be the number of timestamps $t_j$ that $j \le i$ and belong to $T^*$, i.e. $\-{wit}(i) = \abs{\{ t_j \mid t_j \in T^*, j \le i \}}$. Specifically, we prove


% % \[\forall 1\le i \le m,\quad A_i \le \ell^{i-\-{wit}(i)} \prod\limits_{\substack{j\le i \\ t_j\in T^*}}\ell^\-{pad}_{t_j}.\]


% % For the base case, we set $A_0 = 1$.
% % For the induction step, assume it holds for $i < p$. For $i = p$, let $t=t_i$, $v=v_{i(t)}$, we use the additive principle and the multiplicative principle to bound $A_i$,
% % \begin{itemize}
% %     \item if $t \in T^*$,  we know that $r(t) = \bot$. By the additive principle and the multiplicative principle it contributes at most $ \max_{\*r^{V_H^V}, \*c^{V_H^V}} \left( \abs{b_v(\bot) \mu_v^{\bot, \*r, \*c}(0)} + \abs{b_v(\bot) \mu_v^{\bot, \*r, \*c}(1) }\right) \le \ell^\-{pad}$. So 
% %     \[A_p \le A_{p-1} \ell^\-{pad}_v \le \ell^{p-\-{wit}(p)} \prod\limits_{\substack{j\le i \\ t_j\in T^*}}\ell^\-{pad}_{t_j}.\]
% %     \item otherwise, by the additive principle and the multiplicative principle it contributes at most $\abs{b(0)} + \max_{\*r^{V_H^V}, \*c^{V_H^V}} \left( \abs{b_v(\bot) \mu_v^{\bot, \*r, \*c}(0)} + \abs{b_v(\bot) \mu_v^{\bot, \*r, \*c}(1) }\right) \le \ell$.
% %      So
% %     \[A_p \le A_{p-1} \ell \le \ell^{p-\-{wit}(p)} \prod\limits_{\substack{j\le i \\ t_j\in T^*}}\ell^\-{pad}_{t_j}.\]
% % \end{itemize}

% % So, it holds that,

% % \[
% % A_m \le \ell^{k \abs{N^2(T)}} \prod\limits_{t \in T}\ell_t^\-{pad} \le \left(\ell^\-{pad}\right)^{\abs{T^*}}\ell^{k \abs{N^2(T)} + \abs{V}}.
% % \]
% % \end{proof}

% % \begin{lemma}
% % \label{lemma:decay-witness-2-tree-upper-bounded-by-am}
% % Suppose assumptions in \Cref{lemma:convergence-decay-witness-2-tree}, it holds that,
% % \begin{align}\label{eq:am}
% % \sum\limits_{
% % \substack{
% % C: \=T(C) = T \\
% %  \tau \in \{0,1\}^{\abs{C}}
% % }}
% % \abs{\mu^\-{GD}_\infty \left( \+T^\-{wit} = T^\-{wit}, \+C^\-{wit} = C, \sigma_C = \tau_C \right)}
% % \le A_m.
% % \end{align}
% % \end{lemma}

% % \begin{proof}
    
% % Fix a bad component $C$, a configuration $\tau\in\{0,1\}^{\abs{C}}$ on $C$ and a function $\*r^U$. Let $\Omega_C^{\tau, \*r}$ be all possible $(\*r'^U, \*c'^U)$'s satisfying $\+C^\-{wit} = C$, $\*c'(C) = \tau$ and $\*r'(N^+(C))=\*r(N^+(C))$, i.e.,

% % \[
% % \Omega_C^{\tau, \vec{r}} = \left\{(\*r', \*c') \mid (\*r', \*c')\in \Omega_T, \*c'(C) = \tau, \*r'=\text{res}(\*r, N^+(C)), \mu_T^\-{GD}(\+C^\-{wit}=C \mid \*r') = 1 \right\}.
% % \]

% % Let 
% % \[
% % A_{C}^{\tau, \*r} = \sum\limits_{(\*r',\*c') \in \Omega_C^{\tau, \*r}} F(\*r', \*c', U) = F(\*r, \*c', C)\sum\limits_{(\*r',\*c') \in \Omega_C^{\tau, \*r}} F(\*r', \*c', U \backslash C).\]

% % The second equality is due to we fixed the $r$'s and $c$'s on $C$. Let $\*c'(C) = \tau$ and

% % \[
% % \+A_{C}^{\tau, \*r} = F(\*r, \*c', C) \cdot  G(\*r, N(C)).
% % % \abs{\mu_T^\-{GD}(\+T^\-{wit}=T^\-{wit}, \+C^\-{wit}=C, \sigma_C=\tau, \vec{r})}.
% % \]

% % We show that in order to prove \Cref{eq:am1}, it suffices to prove for any witness component $C$, a configuration $\tau\in\{0,1\}^{\abs{C}}$ on $C$ and a vector $\*r^U \in \Omega_T$, it holds that $\+A_{C}^{\tau, \*r} \le A_{C}^{\tau, \*r}$.


% % Given witness component $C$, configuration on it $\tau \in \{0,1\}^C$ and a function $\*r'{^{N^{+}(C)}}$ containing only $r$'s in $N^+(C)$. We can upper bound 
% % \[\abs{\mu_T^\-{GD}(\+T^\-{wit} = T^\-{wit}, \+C^\-{wit}=C, \sigma_C = \tau, \*r')},\]
% % by the following procedure:
% % \begin{enumerate}
% %     \item enumerate all timestamps in the order of $\-{TP}$, let $\*c^C$ satisfying $\forall t \in C$, $c_t = \tau_t$;
% %     \item for the $i$-th timestamps, let $t=t_i$, $v = v_{i(t)}$ and ,
% %     \begin{itemize}
% %         % \item if $i$ is in $T^\-{bad}$, it contributes at most $\abs{\mu^\-{LB}_{v}(\bot)} \max_{\tau' \in \{0,1\}^{V\backslash v}}\abs{\mu_v^{\tau'}(\tau_v)}$.
% %         \item if $t$ is in $C$, it contributes at most $\abs{b_v(\bot) \mu_v^{\bot, \*r, \*c}(\tau_v) } $.
% %         \item if $t$ is in the neighbor of $C$, it contributes at most $\abs{b_v(r_t)}$.
% %     \end{itemize}
% % \end{enumerate}


% % So it holds by the triangle inequality,


% % \[\sum\limits_{
% % \substack{
% % C: \=T(C) = T \\
% %  \tau \in \{0,1\}^{\abs{C}}
% % }}
% % \abs{\mu^\-{GD}_T \left( \+T^\-{wit} = T^\-{wit}, \+C^\-{wit} = C, \sigma_C = \tau_C \right)} 
% % \le
% % \sum\limits_{\substack{C:\=T(C)=T\\ \tau \in \{0,1\}^{\abs{C}} \\ {\*r}^{N^{+}(C)} }} \+A_C^{\tau, \*r},
% % \]



% % and it holds by the definition of $A_C^{\tau, \*r}$ and $A_m$,
% % \[
% % \sum\limits_{\substack{C:\=T(C)=T^\-{wit}\\ \tau \in \{0,1\}^{\abs{C}} \\ {\*r}^{N^{+}(C)} }} A_C^{\tau, \*r} = A_m.
% % \]



% % % For a possible witness component $C$, define $\Omega_C$ be all possible $(\vec{r}, \vec{c})$ satisfying that $\+C^\-{wit} = C$, i.e.,
% % % \[
% % % \Omega_C =  \{(\vec{r}, \vec{c}) \mid (\vec{r}, \vec{c}) \in \Omega_T, \mu_\infty^\-{GD}(\+C^\-{wit}=C \mid \vec{r}) = 1 \}.
% % % \]

% % % Note for two distinct witness components $C_1, C_2$, $\Omega_{C_1} \cap \Omega_{C_2} = \emptyset$.

% % % Let
% % % \[
% % % A^{C}_{\tau} = \sum\limits_{\substack{(\vec{r},\vec{c}) \in \Omega_C \\ \forall t_i \in C, c_i = \tau_{t_i}}} \prod\limits_{j \le m} \left( \abs{\mu^\-{LB}_{v_{i(t_j)}}(0)}\cdot \=I[r_j = 0] + \abs{\mu_{v_{i(t_j)}}^{\-{pad}, \vec{r}, \vec{c}}(c_j) \mu_{v_{i(t_j)}}^\-{LB}(\bot)} \cdot \=I[r_j = \bot] \right),
% % % \]



% % % \[
% % % \+A^{C}_{\tau}=
% % % \abs{\mu^\-{GD}_\infty \left( \+T^\-{wit} = T^\-{wit}, \+C^\-{wit} = C, \sigma_C = \tau \right)}.
% % % \]

% % % It suffices to show that for any witness component $C$ and any $\tau \in \{0,1\}^{\abs{C}}$, $\+A^C_\tau \le A^C_\tau$.

% % % Recall the aforementioned procedure to bound $\mu_\infty^\-{GD}\left( \+T^\-{bad} = T, \+C^\-{bad} = C, \sigma_C = \tau \right)$ given $r$'s on $N^+(C)$. We can now bound $\+A_\tau^C$ by enumerating $r$'s on $N^+(C)$. We define $\vec{r}' \in \{0, \bot\}^{\abs{U}}$ but we only use $\vec{r}'_{N^+(C)}$ and $\+A^{C, \vec{r}'} = \abs{\mu^\-{GD}_\infty\left( \+T^\-{wit} = T^\-{wit}, \+C^\-{wit} = C, \sigma_C = \tau, \vec{r}'_{N^+(C)} \right)}$, by the aforementioned procedure, it can be upper bounded by,
% % % \begin{align*}
% % %     \+A^{C, \vec{r}'}_\tau &\le \prod\limits_{t \in C}\left( \abs{\mu_{v_{i(t)}}^\-{LB}(0)} \cdot \=I[r_t = 0] + \abs{\mu_{v_{i(t)}}^\-{LB}(\bot)\mu_{v_{i(t)}}^{\-{pad}, \tau, \vec{r}'}(c_t)} \cdot \=I[r_t = \bot] \right) 
% % %     \\&\qquad \cdot \prod\limits_{t \in N(C)} \left( \abs{\mu_{v_{i(t)}}^\-{LB}(0)} \cdot \=I[r_t = 0] + \abs{\mu_{v_{i(t)}}^\-{LB}(\bot)} \cdot \=I[r_t = \bot] \right),
% % % \end{align*}

% % % It can be seen that we put a value on each $t \in N^+(C)$ and then product them together. Now we consider $A^{C, \vec{r}'}_{\tau}$ which is defined as $A^{C}_{\tau}$ restricted $\vec{r}_{N^+(C)} = \vec{r}'_{N^+(C)}$.

% % % We also define 
% % % \[
% % % A^{C, \vec{r}'}_{\tau} = \sum\limits_{\substack{(\vec{r},\vec{c}) \in \Omega_C \\ \forall t_i \in C, c_i = \tau_{t_i} \\ \forall t_i \in N^+(C), r_i = r'_i}} \prod\limits_{j \le m} \left( \abs{\mu^\-{LB}_{v_{i(t_j)}}(0)}\cdot \=I[r_j = 0] + \abs{\mu_{v_{i(t_j)}}^{\-{pad}, \vec{r}, \vec{c}}(c_j) \mu_{v_{i(t_j)}}^\-{LB}(\bot)} \cdot \=I[r_j = \bot] \right),
% % % \]

% % % In order to prove $\+A_\tau^C \le A_\tau^C$ it suffices to prove for any $\vec{r}' \in \{0, \bot\}^{\abs{U}}$, it holds that $\+A^{C, \vec{r}'}_\tau \le A^{C, \vec{r}'}_{\tau}$. Note because we fix the $r$'s and $c$'s on $N^+(C)$, but for $A^{C, \vec{r}'}_\tau$, it enumerate $c$'s on $N(C)$ and $r$'s, $c$'s for $U \backslash N^+(C)$. So it holds that,
% % % \[
% % % \frac{A^{C, \vec{r}'}_{\tau}}{\+A^{C, \vec{r}'}_\tau} = 
% % % \]

% % % a similar following procedure:

% % % \begin{enumerate}
% % % \item enumerate all timestamps in the order of TP;
% % % \item for the $i$-th timestamps, $t=t_i$, $v=v_{i(t)}$.
% % %     \begin{enumerate}
% % %     \item if $t$ is in $\ts(V, 0)$, it contributes $\abs{\mu_v^\-{LB}(0)} + \abs{\mu_v^\-{LB}(\bot) \mu_v^{\-{pad}, \tau}(0)}$ or $\abs{\mu_v^\-{LB}(\bot) \mu_v^{\-{pad}, \tau}(1) }$ depending on $\tau_v$.
        
% % %     \item if  $t \in C \backslash \{\ts(V, 0)\}$, we know $r_t = \bot$, so its contribution is at most $\abs{\mu_{v}^{\-{pad}, \tau, \vec{r}}(\tau_{v}) \mu_{v}^\-{LB}(\bot)}$ which is the same as $\abs{\mu_{v}^{\-{pad}, \vec{r}, \vec{c}}(\tau_{v}) \mu_{v}^\-{LB}(\bot)}$ where we set $\forall t_j \in C, c_{j} = \tau_{t_k}$.
        
% % %     \item if $t$ is in neighbors of $C$, it contributes at most $\abs{\mu_v^\-{LB}(0)} + \abs{\mu_v^\-{LB}(\bot)}$.
    
% % %     \end{enumerate}
% % % \end{enumerate}

% % % For type (a) timestamps, because in $A_{\tau}^C$, we enumerate all possible $r$'s of the timestamps, so the contributions for $A_{\tau}^C$ are the same as those for $\+A_{\tau}^C$.
% % % For type (b) timestamps, the contributions for $\+A_\tau^C $ are also the same as those for $ A_\tau^C$. 
% % % For type (c) timestamps, in $\+A_\tau^C$, it contributes at most $\left(\abs{\mu_v^\-{LB}(0)} + \abs{\mu_v^\-{LB}(\bot)}\right)^{\abs{N(C)}}$. In $A_\tau^C$, it enumerates all possible $r$'s outside of $C$ by the additive principle and the multiplicative principle, it contributes at least $\left(\abs{\mu_v^\-{LB}(0)} + \abs{\mu_v^\-{LB}(\bot)}\right)^{\abs{U}-\abs{C}}$. Note $U$ contains all possible bad components' neighbors. So $\+A_\tau^C \le A_\tau^C$.

% % Now we prove that $\+A_C^{\tau, \*r} \le A_C^{\tau, \*r}$.

% % \begin{align*}
% %     \frac{A_C^{\tau, \*r}}{\+A_C^{\tau, \*r}} &= \frac{\sum\limits_{(\*r',\*c') \in \Omega_C^{\tau, \*r}} F(\*r', \*c', U \backslash C)}{G(\*r, N(C))}.
% % \end{align*}

% % % Note that
% % % \[
% % % \sum\limits_{(\*r',\*c') \in \Omega_C^{\tau, \*r}} F(\*r', \*c', U \backslash C) 
% % % =
% % % \sum\limits_{(\*r',\*c') \in \Omega_C^{\tau, \*r}} 
% % % F(\*r', \*c', N(C)) 
% % % F(\*r', \*c', U \backslash N^+(C)).
% % % \]

% % % We show that for any $X \neq \emptyset$ and $X \subseteq U \backslash C$, pick $t_j \in X$ it holds that,

% % Let $X \subseteq U \backslash N^+(C)$, 
% % \[
% % \Omega_{T, X} = \{(\*r, \*c) \mid (\*r', \*c') \in \Omega_T, \*r = \text{res}(\*r', C \cup X), \*c = \text{res}(\*c', C \cup X) \}.
% % \]
% % \[
% % \Omega_{C, X}^{\tau, \*r} = \{ (\text{res}(\*r', C \cup X), \text{res}(\*c', C \cup X)) \mid (\*r', \*c') \in \Omega_{C}^{\tau, \*r}. \}
% % \]

% % We show that for any $X \neq \emptyset$ and $X \subseteq U \backslash N^+(C)$, pick $t_j \in X$ such that,

% % \[
% % \sum\limits_{(\*r',\*c') \in \Omega_{C, X \cup N^+(C)}^{\tau, \*r}} 
% % F(\*r', \*c', N(C)) 
% % F(\*r', \*c', X)
% % \ge 
% % \sum\limits_{(\*r',\*c') \in \Omega_{C, X \cup N^+(C) \backslash \{t_j\}}^{\tau, \*r}} 
% % F(\*r', \*c', N(C)) 
% % F(\*r', \*c', X \backslash \{t_j\}).
% % \]
% % % \yxtodo{bugs and not clear here.}
% % \begin{align*}
% % &\sum\limits_{(\*r',\*c') \in \Omega_{C, X \cup N^+(C)}^{\tau, \*r}} 
% % F(\*r', \*c', N(C)) 
% % F(\*r', \*c', X) \\
% % =&\sum\limits_{(\*r',\*c') \in \Omega_{C, X \cup N^+(C) \backslash \{t_j\}}^{\tau, \*r}} 
% % F(\*r', \*c', N(C)) 
% % F(\*r', \*c', X \backslash \{t_j\}) \left( \sum\limits_{\substack{ 
% % \*r^* \in \text{ex}(\*r', N^+(C) \cup X)
% % \\ 
% % \*c^* \in  \text{ex}(\*c', N^+(C) \cup X)
% % }}  f(\*r^*, \*c^*, t_j) \right) \\
% % (\text{by Triangle inequality})\quad \ge& \sum\limits_{(\*r',\*c') \in \Omega_{C, X \cup N^+(C) \backslash \{t_j\}}^{\tau, \*r}} 
% % F(\*r', \*c', N(C)) 
% % F(\*r', \*c', X \backslash \{t_j\})
% % \end{align*}

% % So it holds that,
% % \[
% % \sum\limits_{(\*r',\*c') \in \Omega_C^{\tau, \*r}} F(\*r', \*c', U \backslash C) \ge \sum\limits_{(\*r',\*c') \in \Omega_{C, \emptyset}^{\tau, \*r}} 
% % F(\*r', \*c', N(C)).
% % \]

% % Next we show that for any $X \subseteq N(C)$, pick $t_j \in X$, it holds that,
% % \[
% % \sum\limits_{(\*r',\*c') \in \Omega_{C, C \cup X}^{\tau, \*r}} 
% % F(\*r', \*c', X)\ge 
% % G(\*r, t_j)\cdot \sum\limits_{(\*r',\*c') \in \Omega_{C, C \cup X \backslash \{t_j\}}^{\tau, \*r}} 
% % F(\*r', \*c', X\backslash\{t_j\}).
% % \]

% % \begin{align*}
% %     &\sum\limits_{(\*r',\*c') \in \Omega_{C, C \cup X}^{\tau, \*r}} 
% % F(\*r', \*c', X) \\
% % &=\sum\limits_{(\*r',\*c') \in \Omega_{C, C \cup X \backslash \{t_j\}}^{\tau, \*r}} 
% % F(\*r', \*c', X) \left( \sum\limits_{\substack{ \*r^*: \*r^* \in \text{ex}(\*r', C \cup X ) \\ \*c^*: \*c^* \in \text{ex}(\*c', C \cup X) }}  f(\*r^*, \*c^*, t_j) \right) \\
% % (\text{by Triangle inequality})\quad &\ge G(\*r, t_j)\cdot \sum\limits_{(\*r',\*c') \in \Omega_{C, C \cup X \backslash \{t_j\}}^{\tau, \*r}} 
% % F(\*r', \*c', X\backslash\{t_j\}).
% % \end{align*}

% % So $\+A_C^{\tau, \*r} \le A_C^{\tau, \*r}$ which implies the lemma.
% % \end{proof}
% %     Fix a witness component $C$, a configuration $\tau\in\{0,1\}^{\abs{C}}$ on $C$ and a vector $\vec{r} \in \{0,\bot\}^{\abs{U}}$. Let $\Omega_C^{\tau, \vec{r}}$ be all possible $(\vec{r}', \vec{c}')$'s satisfying $\+C^\-{wit} = C$, $\vec{c}'_{C} = \tau$ and $\vec{r}'_{N^+(C)}=\vec{r}_{N^+(C)}$, i.e.,

% % \[
% % \Omega_C^{\tau, \vec{r}} = \left\{(\vec{r}', \vec{c}') \mid (\vec{r}', \vec{c}')\in \Omega, \vec{c}'_{C} = \tau, \vec{r}'_{N^+(C)}=\vec{r}_{N^+(C)}, \mu_T^\-{GD}(\+C^\-{wit}=C \mid \vec{r}') = 1 \right\}.
% % \]

% % Let 
% % \[
% % A_{C}^{\tau, \vec{r}} = \sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} F(\vec{r}, \vec{c}, U) = F(\vec{r}, \vec{c}', C)\sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} F(\vec{r}', \vec{c}', U \backslash C),\quad \vec{c}'_{C} = \tau.\]

% % The second equality is due to we fixed the $r$'s and $c$'s on $C$.

% % \[
% % \+A_{C}^{\tau, \vec{r}} = F(\vec{r}, \vec{c}', C) \cdot  G(\vec{r}, N(C)),\quad \vec{c}'_{C} = \tau.
% % % \abs{\mu_T^\-{GD}(\+T^\-{wit}=T^\-{wit}, \+C^\-{wit}=C, \sigma_C=\tau, \vec{r})}.
% % \]

% % We show that in order to prove \Cref{eq:am}, it suffices to prove for any witness component $C$, a configuration $\tau\in\{0,1\}^{\abs{C}}$ on $C$ and a vector $\vec{r} \in \{0,\bot\}^{\abs{U}}$, it holds that $\+A_{C}^{\tau, \vec{r}} \le A_{C}^{\tau, \vec{r}}$.


% % Given witness component $C$, configuration on it $\tau \in \{0,1\}^C$ and a vector $\vec{r}'$ containing only $r$'s in $N^+(C)$. We can upper bound 
% % \[\abs{\mu_\infty^\-{GD}(\+T^\-{wit} = T^\-{wit}, \+C^\-{wit}=C, \sigma_C = \tau, \vec{r}')},\]
% % by the following procedure:
% % \begin{enumerate}
% %     \item enumerate all timestamps in the order of $\-{TP}$;
% %     \item for the $i$-th timestamps, let $t=t_i$, $v = v_{i(t)}$ and ,
% %     \begin{itemize}
% %         % \item if $i$ is in $T^\-{bad}$, it contributes at most $\abs{\mu^\-{LB}_{v}(\bot)} \max_{\tau' \in \{0,1\}^{V\backslash v}}\abs{\mu_v^{\tau'}(\tau_v)}$.
% %         \item if $t$ is in $C$, it contributes at most $\abs{\mu^\-{LB}_{v}(\bot) \mu_v^{\-{pad}, \vec{r}, \vec{c}}(\tau_v) } $.
% %         \item if $t$ is in $N(C)$, it contributes at most $\abs{\mu^\-{LB}_v(r_t)}$.
% %     \end{itemize}
% % \end{enumerate}


% % So it holds by the triangle inequality,


% % \[\sum\limits_{
% % \substack{
% % C: \=T(C) = T \\
% %  \tau \in \{0,1\}^{\abs{C}}
% % }}
% % \abs{\mu^\-{GD}_\infty \left( \+T^\-{wit} = T^\-{wit}, \+C^\-{wit} = C, \sigma_C = \tau_C \right)} 
% % \le
% % \sum\limits_{\substack{C:\=T(C)=T^\-{wit}\\ \tau \in \{0,1\}^{\abs{C}} \\ \vec{r} \in \{0,\bot\}^{N^+(C)} }} \+A_C^{\tau, \vec{r}},
% % \]



% % and 
% % \[
% % \sum\limits_{\substack{C:\=T(C)=T^\-{wit}\\ \tau \in \{0,1\}^{\abs{C}} \\ \vec{r} \in \{0,\bot\}^{N^+(C)} }} A_C^{\tau, \vec{r}} = A_m.
% % \]



% % % For a possible witness component $C$, define $\Omega_C$ be all possible $(\vec{r}, \vec{c})$ satisfying that $\+C^\-{wit} = C$, i.e.,
% % % \[
% % % \Omega_C =  \{(\vec{r}, \vec{c}) \mid (\vec{r}, \vec{c}) \in \Omega_T, \mu_\infty^\-{GD}(\+C^\-{wit}=C \mid \vec{r}) = 1 \}.
% % % \]

% % % Note for two distinct witness components $C_1, C_2$, $\Omega_{C_1} \cap \Omega_{C_2} = \emptyset$.

% % % Let
% % % \[
% % % A^{C}_{\tau} = \sum\limits_{\substack{(\vec{r},\vec{c}) \in \Omega_C \\ \forall t_i \in C, c_i = \tau_{t_i}}} \prod\limits_{j \le m} \left( \abs{\mu^\-{LB}_{v_{i(t_j)}}(0)}\cdot \=I[r_j = 0] + \abs{\mu_{v_{i(t_j)}}^{\-{pad}, \vec{r}, \vec{c}}(c_j) \mu_{v_{i(t_j)}}^\-{LB}(\bot)} \cdot \=I[r_j = \bot] \right),
% % % \]



% % % \[
% % % \+A^{C}_{\tau}=
% % % \abs{\mu^\-{GD}_\infty \left( \+T^\-{wit} = T^\-{wit}, \+C^\-{wit} = C, \sigma_C = \tau \right)}.
% % % \]

% % % It suffices to show that for any witness component $C$ and any $\tau \in \{0,1\}^{\abs{C}}$, $\+A^C_\tau \le A^C_\tau$.

% % % Recall the aforementioned procedure to bound $\mu_\infty^\-{GD}\left( \+T^\-{bad} = T, \+C^\-{bad} = C, \sigma_C = \tau \right)$ given $r$'s on $N^+(C)$. We can now bound $\+A_\tau^C$ by enumerating $r$'s on $N^+(C)$. We define $\vec{r}' \in \{0, \bot\}^{\abs{U}}$ but we only use $\vec{r}'_{N^+(C)}$ and $\+A^{C, \vec{r}'} = \abs{\mu^\-{GD}_\infty\left( \+T^\-{wit} = T^\-{wit}, \+C^\-{wit} = C, \sigma_C = \tau, \vec{r}'_{N^+(C)} \right)}$, by the aforementioned procedure, it can be upper bounded by,
% % % \begin{align*}
% % %     \+A^{C, \vec{r}'}_\tau &\le \prod\limits_{t \in C}\left( \abs{\mu_{v_{i(t)}}^\-{LB}(0)} \cdot \=I[r_t = 0] + \abs{\mu_{v_{i(t)}}^\-{LB}(\bot)\mu_{v_{i(t)}}^{\-{pad}, \tau, \vec{r}'}(c_t)} \cdot \=I[r_t = \bot] \right) 
% % %     \\&\qquad \cdot \prod\limits_{t \in N(C)} \left( \abs{\mu_{v_{i(t)}}^\-{LB}(0)} \cdot \=I[r_t = 0] + \abs{\mu_{v_{i(t)}}^\-{LB}(\bot)} \cdot \=I[r_t = \bot] \right),
% % % \end{align*}

% % % It can be seen that we put a value on each $t \in N^+(C)$ and then product them together. Now we consider $A^{C, \vec{r}'}_{\tau}$ which is defined as $A^{C}_{\tau}$ restricted $\vec{r}_{N^+(C)} = \vec{r}'_{N^+(C)}$.

% % % We also define 
% % % \[
% % % A^{C, \vec{r}'}_{\tau} = \sum\limits_{\substack{(\vec{r},\vec{c}) \in \Omega_C \\ \forall t_i \in C, c_i = \tau_{t_i} \\ \forall t_i \in N^+(C), r_i = r'_i}} \prod\limits_{j \le m} \left( \abs{\mu^\-{LB}_{v_{i(t_j)}}(0)}\cdot \=I[r_j = 0] + \abs{\mu_{v_{i(t_j)}}^{\-{pad}, \vec{r}, \vec{c}}(c_j) \mu_{v_{i(t_j)}}^\-{LB}(\bot)} \cdot \=I[r_j = \bot] \right),
% % % \]

% % % In order to prove $\+A_\tau^C \le A_\tau^C$ it suffices to prove for any $\vec{r}' \in \{0, \bot\}^{\abs{U}}$, it holds that $\+A^{C, \vec{r}'}_\tau \le A^{C, \vec{r}'}_{\tau}$. Note because we fix the $r$'s and $c$'s on $N^+(C)$, but for $A^{C, \vec{r}'}_\tau$, it enumerate $c$'s on $N(C)$ and $r$'s, $c$'s for $U \backslash N^+(C)$. So it holds that,
% % % \[
% % % \frac{A^{C, \vec{r}'}_{\tau}}{\+A^{C, \vec{r}'}_\tau} = 
% % % \]

% % % a similar following procedure:

% % % \begin{enumerate}
% % % \item enumerate all timestamps in the order of TP;
% % % \item for the $i$-th timestamps, $t=t_i$, $v=v_{i(t)}$.
% % %     \begin{enumerate}
% % %     \item if $t$ is in $\ts(V, 0)$, it contributes $\abs{\mu_v^\-{LB}(0)} + \abs{\mu_v^\-{LB}(\bot) \mu_v^{\-{pad}, \tau}(0)}$ or $\abs{\mu_v^\-{LB}(\bot) \mu_v^{\-{pad}, \tau}(1) }$ depending on $\tau_v$.
        
% % %     \item if  $t \in C \backslash \{\ts(V, 0)\}$, we know $r_t = \bot$, so its contribution is at most $\abs{\mu_{v}^{\-{pad}, \tau, \vec{r}}(\tau_{v}) \mu_{v}^\-{LB}(\bot)}$ which is the same as $\abs{\mu_{v}^{\-{pad}, \vec{r}, \vec{c}}(\tau_{v}) \mu_{v}^\-{LB}(\bot)}$ where we set $\forall t_j \in C, c_{j} = \tau_{t_k}$.
        
% % %     \item if $t$ is in neighbors of $C$, it contributes at most $\abs{\mu_v^\-{LB}(0)} + \abs{\mu_v^\-{LB}(\bot)}$.
    
% % %     \end{enumerate}
% % % \end{enumerate}

% % % For type (a) timestamps, because in $A_{\tau}^C$, we enumerate all possible $r$'s of the timestamps, so the contributions for $A_{\tau}^C$ are the same as those for $\+A_{\tau}^C$.
% % % For type (b) timestamps, the contributions for $\+A_\tau^C $ are also the same as those for $ A_\tau^C$. 
% % % For type (c) timestamps, in $\+A_\tau^C$, it contributes at most $\left(\abs{\mu_v^\-{LB}(0)} + \abs{\mu_v^\-{LB}(\bot)}\right)^{\abs{N(C)}}$. In $A_\tau^C$, it enumerates all possible $r$'s outside of $C$ by the additive principle and the multiplicative principle, it contributes at least $\left(\abs{\mu_v^\-{LB}(0)} + \abs{\mu_v^\-{LB}(\bot)}\right)^{\abs{U}-\abs{C}}$. Note $U$ contains all possible bad components' neighbors. So $\+A_\tau^C \le A_\tau^C$.

% % Now we prove that $\+A_C^{\tau, \vec{r}} \le A_C^{\tau, \vec{r}}$.

% % \begin{align*}
% %     \frac{A_C^{\tau, \vec{r}}}{\+A_C^{\tau, \vec{r}}} &= \frac{\sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} F(\vec{r}', \vec{c}', U \backslash C)}{G(\vec{r}, N(C))}.
% % \end{align*}

% % Let $X = U \backslash N^+(C)$.
% % \[
% % \sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} F(\vec{r}', \vec{c}', U \backslash C) 
% % =
% % \sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} 
% % F(\vec{r}', \vec{c}', N(C)) 
% % F(\vec{r}', \vec{c}', X)
% % \]

% % \yxtodo{bugs and not clear here.}

% % We show that for any $X \neq \emptyset$ and $X \subseteq U \backslash N^+(C)$, pick $t_j \in X$ it holds that,
% % \[
% % \sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} 
% % F(\vec{r}', \vec{c}', N(C)) 
% % F(\vec{r}', \vec{c}', X)
% % \ge 
% % \sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} 
% % F(\vec{r}', \vec{c}', N(C)) 
% % F(\vec{r}', \vec{c}', X \backslash \{t_j\}).
% % \]

% % \begin{align*}
% % &\sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} 
% % F(\vec{r}', \vec{c}', N(C)) 
% % F(\vec{r}', \vec{c}', X) \\
% % =& \sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} 
% % F(\vec{r}', \vec{c}', N(C)) 
% % F(\vec{r}', \vec{c}', X\backslash\{t_j\}) \left( \sum\limits_{\substack{ \vec{r}^*: \vec{r}^*_{U \backslash t_j } = \vec{r}'_{U \backslash t_j } \\ \vec{c}^*: \vec{c}^*_{U \backslash t_j } = \vec{c}'_{U \backslash t_j } }}  f(\vec{r}^*, \vec{c}^*, j) \right) \\
% % (\text{by triangle inequality})\quad \ge& \sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} 
% % F(\vec{r}', \vec{c}', N(C)) 
% % F(\vec{r}', \vec{c}', X \backslash \{t_j\}).
% % \end{align*}

% % So it holds that,
% % \[
% % \sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} F(\vec{r}', \vec{c}', U \backslash C) \ge \sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} 
% % F(\vec{r}', \vec{c}', N(C)).
% % \]

% % We show that for any $X \subseteq N(C)$, pick $t_j \in X$, it holds that,
% % \[
% % \sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} 
% % F(\vec{r}', \vec{c}', X)\ge 
% % G(\vec{r}, j)\cdot \sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} 
% % F(\vec{r}', \vec{c}', X\backslash\{t_j\}).
% % \]

% % \begin{align*}
% %     &\sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} 
% % F(\vec{r}', \vec{c}', X) \\
% % &=\sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} 
% % F(\vec{r}', \vec{c}', X \backslash \{t_j\}) \left( \sum\limits_{\substack{ \vec{r}^*: \vec{r}^*_{U \backslash t_j } = \vec{r}'_{U \backslash t_j } \\ \vec{c}^*: \vec{c}^*_{U \backslash t_j } = \vec{c}'_{U \backslash t_j } }}  f(\vec{r}^*, \vec{c}^*, j) \right) \\
% % (\text{by triangle inequality})\quad &\ge G(\vec{r}, j)\cdot \sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} 
% % F(\vec{r}', \vec{c}', X\backslash\{t_j\}).
% % \end{align*}

% % So $\+A_C^{\tau, \vec{r}} \le A_C^{\tau, \vec{r}}$, which implies the lemma.
% % \end{proof}
% For a given witness component $C$, define $\+B_C$ be a set of $\*r^{N^+(C)}$ such that $C$ is exactly the witness component from $\*r^{N^+(C)}$.
% \[
% \+B_C = \{ \*r^{N^+(C)} \mid \mu_T^\-{GD}(\+C^\-{bad} = C \mid \*r^{N^+(C)}) \neq 0 \}.
% \]

% \begin{lemma}
% \label{lemma:witness-2-tree-disjoint-extension}
%     For a witness $2$-tree $T^\-{wit}$ and two different witness component $C_1$ and $C_2$, $\forall, \*r \in \+B_{C_1}, \*r' \in \+B_{C_2}$, it holds that,
%     \[
%     \text{ex}(\*r, U) \cap \text{ex}(\*r', U) = \emptyset.
%     \]
% \end{lemma}
% \begin{proof}
%     Assume $\text{ex}(\*r, U) \cap \text{ex}(\*r', U) \neq \emptyset$, pick $\*r^* \in \text{ex}(\*r, U) \cap \text{ex}(\*r', U)$. Thus we can construct two different bad components given $\*r^*$, which reaches a contradiction.
% \end{proof}
\yxtodo{This proof is deleted, we can use the proof in sec 4.4}
Now we are ready to prove \Cref{lemma:convergence-decay-witness-2-tree}.
\begin{proof}[Proof of \Cref{lemma:convergence-decay-witness-2-tree}]
\begin{align*}
\sum\limits_{
\substack{
C: \=T(C) = T \\
 \tau \in \{0,1\}^{\abs{C}}
}}
\abs{\mu^\-{GD}_T \left( \+T^\-{wit} = T^\-{wit}, \+C^\-{wit} = C, \sigma_C = \tau_C \right)}
\le&
\sum\limits_{
\substack{
C: \=T(C) = T \\
 \tau \in \{0,1\}^{\abs{C}} \\
 \*r' \in \+B(C)
}}
\abs{\mu^\-{GD}_T \left( \+T^\-{wit} = T^\-{wit}, \+C^\-{wit} = C, \sigma_C = \tau_C, \*r' \right)} \\
\le&
\sum\limits_{\*r \in \text{ex}(\*r', U)} B_{\*r'}(U) \\
\le&
\sum\limits_{\*r \in \Omega_T} B_{\*r}(U) \\
\le&
B(u) \\
\le&
\left(\ell^\-{pad}\right)^{\abs{T^*}} \ell^{k\abs{U\backslash T^*}},
\end{align*}
the first inequality is due to \Cref{lemma:witness-tree-decay-fix-r} and the second inequality is due to \Cref{lemma:witness-2-tree-disjoint-extension}.

% So it holds that,
% \[
% \sum\limits_{
% \substack{
% C: \=T(C) = T \\
%  \tau \in \{0,1\}^{\abs{C}}
% }}
% \abs{\mu^\-{GD}_\infty \left( \+T^\-{wit} = T^\-{wit}, \+C^\-{wit} = C, \sigma_C = \tau_C \right)}
% \le A_m
% \le \left( \ell^\-{pad} \right)^{\abs{T^*}} \ell^{k \abs{N^2(T^\-{wit})} + \abs{V}},
% \]
% the first inequality is due to \Cref{lemma:decay-witness-2-tree-upper-bounded-by-am}, the second inequality is due to \Cref{lemma:decay-witness-2-tree-am-upper-bound}

Now we bound $\abs{N^2(T^\-{wit})}$ on $G_H^*$. By \Cref{lemma:maximum-degree-witness-graph} the degree of  $\ts(V, 0)$ is at most $2 \abs{\+E} \Delta k^2$ and the maximum degree of $G_H^*$ is at most $2 \abs{\+E} \Delta k^2$. 
So $N^2(\ts(V, 0)) \le 4 \abs{\+E}^2 \Delta^2 k^4$. 
For any vertex $v$ in $T^\-{wit}$ and $v \neq \ts(V, 0)$, $u \in N(v)$, it suffices to only consider the contributions from $u \notin N(\ts(V,0))$. It contributes at most $4\Delta^2 k^4$ for any $v$ due to \Cref{lemma:2-tree-construction-one-large-degree}.
% we know their distance is at least $2$ due to \Cref{lemma:2-tree-construction-one-large-degree}. We know for any vertex $v \neq \ts(V, 0)$, the degree of it is at most $2 \Delta k^2$. 
% So $N^2(\{v\}) \le 4\Delta^2 k^4$ for $v \in T^\-{wit}$ and $v \neq \ts(V, 0)$. 
So it holds that

\[
\abs{N^2(T^\-{wit})} \le 4 \abs{\+E}^2 \Delta^2 k^4 + 4\Delta^2 k^4\left(\abs{T^\-{wit}}-1\right).
\]
\end{proof}
    % Given $\+T^\-{wit} = T^\-{wit}$, let $U = T^\-{wit} \cup N^2(T)$, $T^* = T^\-{wit} \backslash \{\ts(V, 0)\}$. 
% Let $T^* = T \backslash \{\ts(S, 0)\}$, we will treat $\ts(S, 0)$ differently from other vertices in $T$ because for $t \in \ts(S, 0)$, $r_t$ may not be $\bot$. 
% Note $U$ contains all vertices for all possible bad components and their neighbors due to \Cref{definition:stationary-start} and \Cref{definition:framework-witness-component-2-trees}. 

% We generate a timestamps tuple \text{TP} by the following procedure.
% \begin{enumerate}
%     \item arrange timestamps in $T^*$ by the lexicographical order. Then append them into $\text{TP}$. Set $B = \abs{\text{TP}}$, $B$ is the number of timestamps in $T^*$.
%     \item arrange vertices in $U\backslash T^*$ by the lexicographic order. For a vertex $v$, enumerate all timestamps in it by the chronological order, if $t$ is not in $\text{TP}$, then append $t$ into $\text{TP}$.
% \end{enumerate}
% Let $\text{TP} = (t_1, t_2, \dots, t_m)$. Note the timestamps in $\text{TP}$ are disjoint: all timestamps in $T^*$ are disjoint and step (2) maintains the disjointness.

% Recall the definition of the decomposed systematics scan Glauber dynamics (\Cref{definition:decomposed-systematic-scan-glauber-dynamics}), each time $t$ is associated with $r_t$ and $c_t$. We define the vector form of $r$'s and $c$'s as $\vec{r} = (r_{t_1},r_{t_2}, \dots, r_{t_m})$, $\vec{c} = (c_{t_1}, c_{t_2}, \dots, c_{t_m})$.
% Note if $\vec{c}$ is fixed, the configuration on $C$ is fixed.


% We sort the timestamps in $U$ forming a sequence $\-{TP} = (t_1, t_2, \dots, t_m)$ such that $t_1 < t_2 < \dots < t_m$.
% Recall the definition of the decomposed systematics scan Glauber dynamics (\Cref{definition:decomposed-systematic-scan-glauber-dynamics}), each timestamp $t$ is associated with $r_t$ and $c_t$. We define the vector form of $r$'s and $c$'s as $\vec{r} = (r_{t_1},r_{t_2}, \dots, r_{t_m})$, $\vec{c} = (c_{t_1}, c_{t_2}, \dots, c_{t_m})$.
% Note if $\vec{c}$ is fixed, the configuration on $C$ is fixed.
% We abuse the notation a little, let $\mu^{\-{pad}, \vec{r}, \vec{c}}_{v_{i(t_i)}}(c_{t_i})$ be the padding measure condition on $\vec{r}, \vec{c}$ except $r_{t_i}$ and $c_{t_i}$ as \Cref{definition:decomposition-scheme}.  
% We say $t \in T$ if $\exists v \in T \text{ s.t. } t \in v$ and $t \in C$ if $\exists v \in C \text{ s.t. } t\in v$.

% This procedure forms a product formula to upper bound $\abs{\mu_\infty^\-{GD}(\+T^\-{wit} = T^\-{wit}, \+C^\-{wit}=C, \sigma_C = \tau, \vec{r}')}$.


% Define 
% \[ \Omega_T = \{(\vec{r}, \vec{c}) \mid (\vec{r}, \vec{c}) \in \{0, \bot\}^{U} \times \{0, 1\}^U, \forall t_i \in T, r_{i}=\bot \}. \]
% % We claim that in our applications we set $\mu$
% be the set containing all possible $(\vec{r},\vec{c})$'s on $U$, note this set is finite due to the size limit of witness component given the witness $2$-tree. 
% % We abuse the notation a little, let $\mu^{\-{pad}, \vec{r}, \vec{c}}_{v_{i(t_i)}}(c_{t_i})$ be the padding measure condition on $\vec{r}, \vec{c}$ except $r_{t_i}$ and $c_{t_i}$ as \Cref{definition:decomposition-scheme}.  
% % We say $t \in T$ if $\exists v \in T, t \in v$.

% % Given $\+C^\-{wit} = C, \vec{r}, \vec{c}$, we can calculate $\abs{\mu_\infty^\-{GD}\left( \+T^\-{wit} = T^\-{wit}, \+C^\-{bad} = C, \vec{r}, \vec{c} \right)}$ via the following procedure.

% % \begin{enumerate}
% %     \item We enumerate all timestamps in $C$ by their orders in $\-{TP}$;
% %     \item For the $i$-th timestamps, let $v = v_{i(t_i)}$,
% %     \begin{itemize}
% %         \item if $r_{t_i} = \bot$, it contributes $\abs{\mu^\-{LB}_{v}(\bot)} \cdot \abs{\mu^{\-{pad}, \vec{r}, \vec{c}}_{v}(c_{t_i})}$.
% %         \item otherwise, it contributes $\abs{\mu^\-{LB}_{v}(c_{t_i})}$.
% %     \end{itemize}
% % \end{enumerate}

% Now let $R_i = \{\{(r_1,\tau_{1}), (r_2,\tau_2), \dots, (r_i,\tau_i)\} \mid (\vec{r}, \vec{\tau}) \in \Omega_T\}$ be the set containing all possible $r$'s and $\tau$'s of the first $i$ timestamps in the order of $\-{TP}$.

% We give following useful functions:

% \[f(\vec{r}, \vec{c}, j) = \abs{\mu^\-{LB}_{v_{i(t_j)}}(0)}\cdot \=I[r_j = 0] + \max\limits_{
% \substack{\vec{r}'\in\{0, \bot\}^{\abs{V_S^V}}, \vec{r}'_{U}=\vec{r} \\
% \vec{c}'\in\{0, 1\}^{\abs{V_S^V}}, \vec{c}'_{U}=\vec{c}
% }}\abs{\mu_{v_{i(t_j)}}^{\-{pad}, \vec{r}', \vec{c}'}(c_j) \mu_{v_{i(t_j)}}^\-{LB}(\bot)} \cdot \=I[r_j = \bot], \]

% $f$ indicates the maximal norm of all possible transitions for timestamp $t_j$ under $\vec{r}$ and $\vec{c}$.

% For $S\subseteq U$, let 
% \[
% F(\vec{r}, \vec{c}, S) = \prod\limits_{t_j \in S}f(\vec{r}, \vec{c}, j).
% \]

% \[
% g(\vec{r}, j) = \abs{\mu_{v_{i(t_j)}}^\-{LB}(0)} \cdot \=I[r_j = 0] + \abs{\mu_{v_{i(t_j)}}^\-{LB}(\bot)} \cdot \=I[r_j = \bot],
% \]

% $g$ indicates the maximal norm of possible ``coin flip'' transitions using only $r$'s.

% For $S\subseteq U$, let 
% \[
% G(\vec{r}, S) = \prod\limits_{t_j \in S}G(\vec{r}, j).
% \]

% Set 

% \[
% A_i = \sum\limits_{(\vec{r},\vec{c}) \in R_i} \prod\limits_{j \le i} f(\vec{r}, \vec{c}, j).
% \]

% By the aforementioned procedure, it holds that,

% \[
% \sum\limits_{
% \substack{
% C: \=T(C) = T \\
% (\vec{r},\vec{c}) \in \Omega_T
% }}
% \abs{\mu^\-{GD}_\infty \left( \+T^\-{wit} = T^\-{wit}, \+C^\-{wit} = C, \vec{r}, \vec{c} \right)}
% \le A_m.
% \]

% We now show that $A_m \le \left( \ell^\-{pad} \right)^{\abs{T^*}} \ell^{k \abs{N^2(T)} + \abs{V}}$ by the induction on $m$. Let $b(i)$ be the number of timestamps that are smaller than $t_i$ and belong to $T^*$, i.e. $b(i) = \abs{\{ t \mid t \in T^*, t \le t_i \}}$. Specifically, we prove


% \[\forall 1\le i \le m,\quad A_i \le \ell^{i-b(i)} \prod\limits_{\substack{t\le t_i \\ t\in T^*}}\ell^\-{pad}_t.\]


% For the base case, we set $A_0 = 1$.
% For the induction step, assume it holds for $i < p$. For $i = p$, let $t=t_i$, $v=v_{i(t)}$, we use the additive principle and the multiplicative principle to bound $A_i$,
% \begin{itemize}
%     \item if $t \in T^*$,  we know that $r_{t} = \bot$. By the additive principle and the multiplicative principle it contributes at most $ \max_{\vec{r}, \vec{c}} \left( \abs{\mu^\-{LB}_v(\bot) \mu_v^{\-{pad}, \vec{r}, \vec{c}}(0)} + \abs{\mu^\-{LB}_v(\bot) \mu_v^{\-{pad}, \vec{r}, \vec{c}}(1) }\right) \le \ell^\-{pad}$. So 
%     \[A_p \le A_{p-1} \ell^\-{pad}_v \le \ell^{p-b(p)} \prod\limits_{\substack{u\le t \\ u\in T^*}}\ell^\-{pad}_u.\]
%     \item otherwise, by the additive principle and the multiplicative principle it contributes at most $\abs{\mu_v^\-{LB}(0)} + \max_{\vec{r}, \vec{c}} \left( \abs{\mu^\-{LB}_v(\bot) \mu_v^{\-{pad}, \vec{r}, \vec{c}}(0)} + \abs{\mu^\-{LB}_v(\bot) \mu_v^{\-{pad}, \vec{r}, \vec{c}}(1) }\right) \le \ell$.
%     % if we fix a bad component, there are $2$ possible cases:
%     % \begin{itemize}
%     %     % \item if $t_i \in \ts(S, 0)$, it contributes at most $\ell$;
%     %     \item if $t_i \notin T$ and $t_i$ is not in the bad component nor is neighbors, it contributes $1 \le \ell$;
%     %     \item If $t_i \notin T$ and $t_i$ is in the bad component or its neighbors, it contributes at most $\ell$.
%     % \end{itemize}
%      So
%     \[A_p \le A_{p-1} \ell \le \ell^{p-b(p)} \prod\limits_{\substack{u\le t \\ u\in T^*}}\ell^\-{pad}_u.\]
% \end{itemize}

% % We show that 
% % $A_m \le \left( \ell^\-{pad} \right)^{\abs{T^*}} \ell^{k \abs{N^2(T)} + \abs{V}}$ by induction. Specifically, we prove 

% % \[A_{B} \le \left( \ell^\-{pad} \right)^{\abs{T^*}},\qquad \forall i \ge B,\quad A_i \le \left( \ell^\-{pad} \right)^{\abs{T^*}} \ell^{i-B}. \]

% % \[A_i \le \left( \ell^\-{pad} \right)^{\abs{\{t_j \mid t_j \in T^*, j\le p \}}} \ell^{i - \abs{\{t_j \mid t_j \in T^*, j\le p \}}}.\]
% % Base case: for $A_{B}$, we know that for all timestamp $t_1, t_2, \dots, t_{B}$, their $r$'s are $\bot$ due to the definition of witness $2$-trees. Each vertices in $T^*$ contributes at most $\ell^\-{pad}$ due to the definition of $\ell^\-{pad}$ and the aforementioned process. So it holds that $A_{B} \le \left( \ell^\-{pad} \right)^{\abs{T^*}}$.

% % Induction step: assume for $i=p-1$, $i\ge B$, it holds that $A_i \le \left( \ell^\-{pad} \right)^{\abs{T}} \ell^{i-B}$. For $i=p$, let $t=t_i$, $v=v_{i(t)}$, for the $r_t$ and $c_t$ there are $3$ cases: $(\bot, 1)$, $(\bot, 0)$, $(0, 0)$. So it contributes at most $\ell$ due to the definition of $\ell$ and the aforementioned process. So $A_p = A_{p-1} \ell \le \left( \ell^\-{pad} \right)^{\abs{T}} \ell^{p-B} $


% % For the base case, we set $A_0 = 1$.
% % Assume it holds for $i < p$, for $i = p$,
% % \begin{itemize}
% %     \item if $t_i \in T^*$. We know $r_{t_i}=\bot$, due to the stopping patterns and $\forall v \in V, \mu^\-{ly, LB}_v(1)=0$. So it contributes at most $\ell^\-{pad}$ in all possible bad components. So 
% %     \[A_p \le A_{p-1} \ell^\-{pad} \le \left( \ell^\-{pad} \right)^{\abs{\{t_j \mid t_j \in T^*, j\le p \}}} \ell^{i - \abs{\{t_j \mid t_j \in T^*, j\le p \}}}.\]
% %     \item otherwise, if we fix a bad component, there are $3$ possible cases:
% %     \begin{itemize}
% %         \item if $t_i \in \ts(V, 0)$, it contributes at most $\ell$;
% %         \item if $t_i \notin T^\-{wit}$ and $t_i$ is not in the bad component nor is neighbors, it contributes $1 \le \ell$;
% %         \item If $t_i \notin T^\-{wit}$ and $t_i$ is in the bad component or its neighbors, it contributes at most $\ell$.
% %     \end{itemize}
% %      So
% %     \[A_p \le A_{p-1} \ell \le \left( \ell^\-{pad} \right)^{\abs{\{t_j \mid t_j \in T^*, j\le p \}}} \ell^{i - \abs{\{t_j \mid t_j \in T^*, j\le p \}}}.\]
% % \end{itemize}

% So, it holds that,

% \[
% A_m \le \ell^{k \abs{N^2(T)}} \prod\limits_{v \in T}\ell_v^\-{pad} \le \left(\ell^\-{pad}\right)^{\abs{T^*}}\ell^{k \abs{N^2(T)} + \abs{V}}.
% \]


% Now we show that 
% \begin{align}\label{eq:am}
% \sum\limits_{
% \substack{
% C: \=T(C) = T \\
%  \tau \in \{0,1\}^{\abs{C}}
% }}
% \abs{\mu^\-{GD}_\infty \left( \+T^\-{wit} = T^\-{wit}, \+C^\-{wit} = C, \sigma_C = \tau_C \right)}
% \le A_m.
% \end{align}

% Fix a witness component $C$, a configuration $\tau\in\{0,1\}^{\abs{C}}$ on $C$ and a vector $\vec{r} \in \{0,\bot\}^{\abs{U}}$. Let $\Omega_C^{\tau, \vec{r}}$ be all possible $(\vec{r}', \vec{c}')$'s satisfying $\+C^\-{wit} = C$, $\vec{c}'_{C} = \tau$ and $\vec{r}'_{N^+(C)}=\vec{r}_{N^+(C)}$, i.e.,

% \[
% \Omega_C^{\tau, \vec{r}} = \left\{(\vec{r}', \vec{c}') \mid (\vec{r}', \vec{c}')\in \Omega, \vec{c}'_{C} = \tau, \vec{r}'_{N^+(C)}=\vec{r}_{N^+(C)}, \mu_T^\-{GD}(\+C^\-{wit}=C \mid \vec{r}') = 1 \right\}.
% \]

% Let 
% \[
% A_{C}^{\tau, \vec{r}} = \sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} F(\vec{r}, \vec{c}, U) = F(\vec{r}, \vec{c}', C)\sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} F(\vec{r}', \vec{c}', U \backslash C),\quad \vec{c}'_{C} = \tau.\]

% The second equality is due to we fixed the $r$'s and $c$'s on $C$.

% \[
% \+A_{C}^{\tau, \vec{r}} = F(\vec{r}, \vec{c}', C) \cdot  G(\vec{r}, N(C)),\quad \vec{c}'_{C} = \tau.
% % \abs{\mu_T^\-{GD}(\+T^\-{wit}=T^\-{wit}, \+C^\-{wit}=C, \sigma_C=\tau, \vec{r})}.
% \]

% We show that in order to prove \Cref{eq:am}, it suffices to prove for any witness component $C$, a configuration $\tau\in\{0,1\}^{\abs{C}}$ on $C$ and a vector $\vec{r} \in \{0,\bot\}^{\abs{U}}$, it holds that $\+A_{C}^{\tau, \vec{r}} \le A_{C}^{\tau, \vec{r}}$.


% Given witness component $C$, configuration on it $\tau \in \{0,1\}^C$ and a vector $\vec{r}'$ containing only $r$'s in $N^+(C)$. We can upper bound 
% \[\abs{\mu_\infty^\-{GD}(\+T^\-{wit} = T^\-{wit}, \+C^\-{wit}=C, \sigma_C = \tau, \vec{r}')},\]
% by the following procedure:
% \begin{enumerate}
%     \item enumerate all timestamps in the order of $\-{TP}$;
%     \item for the $i$-th timestamps, let $t=t_i$, $v = v_{i(t)}$ and ,
%     \begin{itemize}
%         % \item if $i$ is in $T^\-{bad}$, it contributes at most $\abs{\mu^\-{LB}_{v}(\bot)} \max_{\tau' \in \{0,1\}^{V\backslash v}}\abs{\mu_v^{\tau'}(\tau_v)}$.
%         \item if $t$ is in $C$, it contributes at most $\abs{\mu^\-{LB}_{v}(\bot) \mu_v^{\-{pad}, \vec{r}, \vec{c}}(\tau_v) } $.
%         \item if $t$ is in $N(C)$, it contributes at most $\abs{\mu^\-{LB}_v(r_t)}$.
%     \end{itemize}
% \end{enumerate}


% So it holds by the triangle inequality,


% \[\sum\limits_{
% \substack{
% C: \=T(C) = T \\
%  \tau \in \{0,1\}^{\abs{C}}
% }}
% \abs{\mu^\-{GD}_\infty \left( \+T^\-{wit} = T^\-{wit}, \+C^\-{wit} = C, \sigma_C = \tau_C \right)} 
% \le
% \sum\limits_{\substack{C:\=T(C)=T^\-{wit}\\ \tau \in \{0,1\}^{\abs{C}} \\ \vec{r} \in \{0,\bot\}^{N^+(C)} }} \+A_C^{\tau, \vec{r}},
% \]



% and 
% \[
% \sum\limits_{\substack{C:\=T(C)=T^\-{wit}\\ \tau \in \{0,1\}^{\abs{C}} \\ \vec{r} \in \{0,\bot\}^{N^+(C)} }} A_C^{\tau, \vec{r}} = A_m.
% \]



% % For a possible witness component $C$, define $\Omega_C$ be all possible $(\vec{r}, \vec{c})$ satisfying that $\+C^\-{wit} = C$, i.e.,
% % \[
% % \Omega_C =  \{(\vec{r}, \vec{c}) \mid (\vec{r}, \vec{c}) \in \Omega_T, \mu_\infty^\-{GD}(\+C^\-{wit}=C \mid \vec{r}) = 1 \}.
% % \]

% % Note for two distinct witness components $C_1, C_2$, $\Omega_{C_1} \cap \Omega_{C_2} = \emptyset$.

% % Let
% % \[
% % A^{C}_{\tau} = \sum\limits_{\substack{(\vec{r},\vec{c}) \in \Omega_C \\ \forall t_i \in C, c_i = \tau_{t_i}}} \prod\limits_{j \le m} \left( \abs{\mu^\-{LB}_{v_{i(t_j)}}(0)}\cdot \=I[r_j = 0] + \abs{\mu_{v_{i(t_j)}}^{\-{pad}, \vec{r}, \vec{c}}(c_j) \mu_{v_{i(t_j)}}^\-{LB}(\bot)} \cdot \=I[r_j = \bot] \right),
% % \]



% % \[
% % \+A^{C}_{\tau}=
% % \abs{\mu^\-{GD}_\infty \left( \+T^\-{wit} = T^\-{wit}, \+C^\-{wit} = C, \sigma_C = \tau \right)}.
% % \]

% % It suffices to show that for any witness component $C$ and any $\tau \in \{0,1\}^{\abs{C}}$, $\+A^C_\tau \le A^C_\tau$.

% % Recall the aforementioned procedure to bound $\mu_\infty^\-{GD}\left( \+T^\-{bad} = T, \+C^\-{bad} = C, \sigma_C = \tau \right)$ given $r$'s on $N^+(C)$. We can now bound $\+A_\tau^C$ by enumerating $r$'s on $N^+(C)$. We define $\vec{r}' \in \{0, \bot\}^{\abs{U}}$ but we only use $\vec{r}'_{N^+(C)}$ and $\+A^{C, \vec{r}'} = \abs{\mu^\-{GD}_\infty\left( \+T^\-{wit} = T^\-{wit}, \+C^\-{wit} = C, \sigma_C = \tau, \vec{r}'_{N^+(C)} \right)}$, by the aforementioned procedure, it can be upper bounded by,
% % \begin{align*}
% %     \+A^{C, \vec{r}'}_\tau &\le \prod\limits_{t \in C}\left( \abs{\mu_{v_{i(t)}}^\-{LB}(0)} \cdot \=I[r_t = 0] + \abs{\mu_{v_{i(t)}}^\-{LB}(\bot)\mu_{v_{i(t)}}^{\-{pad}, \tau, \vec{r}'}(c_t)} \cdot \=I[r_t = \bot] \right) 
% %     \\&\qquad \cdot \prod\limits_{t \in N(C)} \left( \abs{\mu_{v_{i(t)}}^\-{LB}(0)} \cdot \=I[r_t = 0] + \abs{\mu_{v_{i(t)}}^\-{LB}(\bot)} \cdot \=I[r_t = \bot] \right),
% % \end{align*}

% % It can be seen that we put a value on each $t \in N^+(C)$ and then product them together. Now we consider $A^{C, \vec{r}'}_{\tau}$ which is defined as $A^{C}_{\tau}$ restricted $\vec{r}_{N^+(C)} = \vec{r}'_{N^+(C)}$.

% % We also define 
% % \[
% % A^{C, \vec{r}'}_{\tau} = \sum\limits_{\substack{(\vec{r},\vec{c}) \in \Omega_C \\ \forall t_i \in C, c_i = \tau_{t_i} \\ \forall t_i \in N^+(C), r_i = r'_i}} \prod\limits_{j \le m} \left( \abs{\mu^\-{LB}_{v_{i(t_j)}}(0)}\cdot \=I[r_j = 0] + \abs{\mu_{v_{i(t_j)}}^{\-{pad}, \vec{r}, \vec{c}}(c_j) \mu_{v_{i(t_j)}}^\-{LB}(\bot)} \cdot \=I[r_j = \bot] \right),
% % \]

% % In order to prove $\+A_\tau^C \le A_\tau^C$ it suffices to prove for any $\vec{r}' \in \{0, \bot\}^{\abs{U}}$, it holds that $\+A^{C, \vec{r}'}_\tau \le A^{C, \vec{r}'}_{\tau}$. Note because we fix the $r$'s and $c$'s on $N^+(C)$, but for $A^{C, \vec{r}'}_\tau$, it enumerate $c$'s on $N(C)$ and $r$'s, $c$'s for $U \backslash N^+(C)$. So it holds that,
% % \[
% % \frac{A^{C, \vec{r}'}_{\tau}}{\+A^{C, \vec{r}'}_\tau} = 
% % \]

% % a similar following procedure:

% % \begin{enumerate}
% % \item enumerate all timestamps in the order of TP;
% % \item for the $i$-th timestamps, $t=t_i$, $v=v_{i(t)}$.
% %     \begin{enumerate}
% %     \item if $t$ is in $\ts(V, 0)$, it contributes $\abs{\mu_v^\-{LB}(0)} + \abs{\mu_v^\-{LB}(\bot) \mu_v^{\-{pad}, \tau}(0)}$ or $\abs{\mu_v^\-{LB}(\bot) \mu_v^{\-{pad}, \tau}(1) }$ depending on $\tau_v$.
        
% %     \item if  $t \in C \backslash \{\ts(V, 0)\}$, we know $r_t = \bot$, so its contribution is at most $\abs{\mu_{v}^{\-{pad}, \tau, \vec{r}}(\tau_{v}) \mu_{v}^\-{LB}(\bot)}$ which is the same as $\abs{\mu_{v}^{\-{pad}, \vec{r}, \vec{c}}(\tau_{v}) \mu_{v}^\-{LB}(\bot)}$ where we set $\forall t_j \in C, c_{j} = \tau_{t_k}$.
        
% %     \item if $t$ is in neighbors of $C$, it contributes at most $\abs{\mu_v^\-{LB}(0)} + \abs{\mu_v^\-{LB}(\bot)}$.
    
% %     \end{enumerate}
% % \end{enumerate}

% % For type (a) timestamps, because in $A_{\tau}^C$, we enumerate all possible $r$'s of the timestamps, so the contributions for $A_{\tau}^C$ are the same as those for $\+A_{\tau}^C$.
% % For type (b) timestamps, the contributions for $\+A_\tau^C $ are also the same as those for $ A_\tau^C$. 
% % For type (c) timestamps, in $\+A_\tau^C$, it contributes at most $\left(\abs{\mu_v^\-{LB}(0)} + \abs{\mu_v^\-{LB}(\bot)}\right)^{\abs{N(C)}}$. In $A_\tau^C$, it enumerates all possible $r$'s outside of $C$ by the additive principle and the multiplicative principle, it contributes at least $\left(\abs{\mu_v^\-{LB}(0)} + \abs{\mu_v^\-{LB}(\bot)}\right)^{\abs{U}-\abs{C}}$. Note $U$ contains all possible bad components' neighbors. So $\+A_\tau^C \le A_\tau^C$.

% Now we prove that $\+A_C^{\tau, \vec{r}} \le A_C^{\tau, \vec{r}}$.

% \begin{align*}
%     \frac{A_C^{\tau, \vec{r}}}{\+A_C^{\tau, \vec{r}}} &= \frac{\sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} F(\vec{r}', \vec{c}', U \backslash C)}{G(\vec{r}, N(C))}.
% \end{align*}

% Let $X = U \backslash N^+(C)$.
% \[
% \sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} F(\vec{r}', \vec{c}', U \backslash C) 
% =
% \sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} 
% F(\vec{r}', \vec{c}', N(C)) 
% F(\vec{r}', \vec{c}', X)
% \]

% \yxtodo{bugs and not clear here.}

% We show that for any $X \neq \emptyset$ and $X \subseteq U \backslash N^+(C)$, pick $t_j \in X$ it holds that,
% \[
% \sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} 
% F(\vec{r}', \vec{c}', N(C)) 
% F(\vec{r}', \vec{c}', X)
% \ge 
% \sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} 
% F(\vec{r}', \vec{c}', N(C)) 
% F(\vec{r}', \vec{c}', X \backslash \{t_j\}).
% \]

% \begin{align*}
% &\sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} 
% F(\vec{r}', \vec{c}', N(C)) 
% F(\vec{r}', \vec{c}', X) \\
% =& \sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} 
% F(\vec{r}', \vec{c}', N(C)) 
% F(\vec{r}', \vec{c}', X\backslash\{t_j\}) \left( \sum\limits_{\substack{ \vec{r}^*: \vec{r}^*_{U \backslash t_j } = \vec{r}'_{U \backslash t_j } \\ \vec{c}^*: \vec{c}^*_{U \backslash t_j } = \vec{c}'_{U \backslash t_j } }}  f(\vec{r}^*, \vec{c}^*, j) \right) \\
% (\text{by triangle inequality})\quad \ge& \sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} 
% F(\vec{r}', \vec{c}', N(C)) 
% F(\vec{r}', \vec{c}', X \backslash \{t_j\}).
% \end{align*}

% So it holds that,
% \[
% \sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} F(\vec{r}', \vec{c}', U \backslash C) \ge \sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} 
% F(\vec{r}', \vec{c}', N(C)).
% \]

% We show that for any $X \subseteq N(C)$, pick $t_j \in X$, it holds that,
% \[
% \sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} 
% F(\vec{r}', \vec{c}', X)\ge 
% G(\vec{r}, j)\cdot \sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} 
% F(\vec{r}', \vec{c}', X\backslash\{t_j\}).
% \]

% \begin{align*}
%     &\sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} 
% F(\vec{r}', \vec{c}', X) \\
% &=\sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} 
% F(\vec{r}', \vec{c}', X \backslash \{t_j\}) \left( \sum\limits_{\substack{ \vec{r}^*: \vec{r}^*_{U \backslash t_j } = \vec{r}'_{U \backslash t_j } \\ \vec{c}^*: \vec{c}^*_{U \backslash t_j } = \vec{c}'_{U \backslash t_j } }}  f(\vec{r}^*, \vec{c}^*, j) \right) \\
% (\text{by triangle inequality})\quad &\ge G(\vec{r}, j)\cdot \sum\limits_{(\vec{r}',\vec{c}') \in \Omega_C^{\tau, \vec{r}}} 
% F(\vec{r}', \vec{c}', X\backslash\{t_j\}).
% \end{align*}

% So $\+A_C^{\tau, \vec{r}} \le A_C^{\tau, \vec{r}}$.
% So it holds that,

% \[
% \sum\limits_{
% \substack{
% C: \=T(C) = T \\
%  \tau \in \{0,1\}^{\abs{C}}
% }}
% \abs{\mu^\-{GD}_\infty \left( \+T^\-{wit} = T^\-{wit}, \+C^\-{wit} = C, \sigma_C = \tau_C \right)}
% \le A_m
% \le \left( \ell^\-{pad} \right)^{\abs{T^*}} \ell^{k \abs{N^2(T^\-{wit})} + \abs{V}}.
% % \le \left( \ell^\-{pad} \right)^{\abs{T^*}} \ell^{k \Delta\left(G_H^S\right)^2 \abs{T}}.
% \]


% % So it holds that,

% % \[
% % \sum\limits_{
% % \substack{
% % C: \=T(C) = T \\
% % (\vec{r},\vec{c}) \in \Omega_T
% % }}
% % \abs{\mu^\-{GD}_\infty \left( \+T^\-{wit} = T^\-{wit}, \+C^\-{wit} = C, \vec{r}, \vec{c} \right)}
% % \le \left( \ell^\-{pad} \right)^{\abs{T^*}} \ell^{m - k \abs{T^*}}
% % \le \left( \ell^\-{pad} \right)^{\abs{T^\-{wit}}-1} \ell^{k \abs{N^2(T^\-{wit})} + \abs{V}}.
% % \]
% % Also let $\vec{c} = (\tau_{t_1}, \tau_{t_2}, \dots, \tau_{t_m})$. By triangle inequality, 
% % \[
% % \abs{\mu^\-{GD}_\infty\left( \+T^\-{bad}=T^\-{wit}, \+C^\-{bad}=C, \sigma(C) = \tau \right)} 
% % \le
% % \sum\limits_{\vec{r} \in \{0,1\}^C}
% % \abs{\mu^\-{GD}_\infty \left( \+T^\-{bad}=T^\-{wit}, \+C^\-{bad}=C, \vec{r}, \vec{c}  \right)}.
% % \]

% Now we bound $\abs{N^2(T^\-{wit})}$ on $G_H^*$. By \Cref{lemma:maximum-degree-witness-graph} the degree of  $\ts(V, 0)$ is at most $2 \abs{\+E} \Delta k^2$ and the maximum degree of $G_H^*$ is at most $2 \abs{\+E} \Delta k^2$. So $N^2(\{\ts(V, 0)\}) \le 4 \abs{\+E}^2 \Delta^2 k^4$. For any vertex $v$ in $T^\-{wit}$ and $v \neq \ts(V, 0)$, we know their distance is at least $2$ due to \Cref{lemma:2-tree-construction-one-large-degree}. We know for any vertex $v \neq \ts(V, 0)$, the degree of it is at most $2 \Delta k^2$. So $N^2(\{v\}) \le 4\Delta^2 k^4$ for $v \in T^\-{wit}$ and $v \neq \ts(V, 0)$. So it holds that

% \[
% \abs{N^2(T^\-{wit})} \le 4 \abs{\+E}^2 \Delta^2 k^4 + 4\Delta^2 k^4\left(\abs{T^\-{wit}}-1\right).
% \]
% \end{proof}

% \begin{comment}
% We can not use the framework (\Cref{subsection:framework-marginal-ratio}) directly, because we need to study the measure on $V$ in order to study the convergence problem.
% So we define the extended witness graph (\Cref{definition:extend-witness-graph}) and associating properties on it. These definitions and lemmas are similar to those in \Cref{subsection:framework-marginal-ratio}.
% Our strategy is that we will categorize all bad components into $2$ types, 
% \begin{enumerate}
%     \item bad component and its neighbors do not overlap the starting states,
%     \item bad component and its neighbors overlap the starting states.
% \end{enumerate}
% We show the contributions of the first type are the same for different starting states. For the second type, we define the decay of bad trees on the extended witness graph to show that their contributions tend to $0$ as $T \to \infty$.

% We abuse the notation a little in this section that we write $T^\-{bad}$ to indicate the bad tree while $-T$ to indicate the initial time of the complex systematic scan Glauber dynamics.

% The main technical issue here is that we will study the marginal measure on $\ts(V, 0)$ whose degree may be very large. 


% \subsection{Extended witness graph and $2$-tree on it} \label{subsection:extended-witness-graph}
% There are some differences between the extended witness graph (\Cref{definition:extend-witness-graph}) and the witness graph (\Cref{definition:witness-graph-indset}):

% \begin{enumerate}
%     \item We will add $\ts(V, 0)$ instead of $\ts(S, 0)$ ($S \subseteq V$ and $\abs{S} = k$) to form the extended witness graph.
%     \item $\ts(V, 0)$ is included in the bad component and bad tree manually.
% \end{enumerate}


% \begin{definition}[Extended witness graph]
% \label{definition:extend-witness-graph}
%     For a hypergraph $H = (V, \+E)$, the \emph{extended witness graph} $G_H^* = (V_H^*, E_H^*)$ is a graph with vertex set 
%     \[
%     V_H^* = \{ \ts(e, t) \mid e \in \+E, t \in \=Z_{\le 0} \} \cup \{\ts(V, 0)\}.
%     \]

%     and there is an undirected edge between $x, y \in V_H^*$ in $G_H^*$ if and only if $x \neq y$ and $x \cap y \neq \emptyset$.
% \end{definition}

% We describe the following algorithm to construct the $2$-tree on an extended witness graph.

% \begin{lemma}[Construction of a maximal 2-tree in a connected graph with one large-degree vertex]
% \label{lemma:2-tree-construction-one-large-degree}
% Let $G = (V, E)$ be a connected graph. Let $v \in V$, $\text{deg}(v) = D$ and $\forall u \neq v, \text{deg}(u) \le d$. We can deterministically construct a 2-tree $\+T$ of $G$ containing $u$ such that $\abs{\+T} \ge \lfloor (\abs{V} - (D+1))/(d+1) \rfloor $ as follows:

% \begin{itemize}
%     \item order the vertices except $v$ in $V$ in lexicography order. Start with $\+T=\{v\}$ and $U = V \backslash N^+(v)$, where $N^+(u) \defeq N(u) \cup \{u\}$ and $N(u) \defeq \{a \in V \mid (a, u) \in E\}$. 
%     \item repeat until $U = \emptyset$: let $a$ be the vertex in $U$ with the smallest distance to $\+T$, with ties broken by the order on $V$ except $v$. Set $\+T \gets \+T \cup \{a\}$ and $U \gets U \backslash N^+(a)$;
% \end{itemize}
    
% \end{lemma}

% \begin{proof}
%     This algorithm is equal to removing $N^+(v)$ and then running the algorithm in \Cref{definition:2-tree-construction} on each connected component of the new graph.
% \end{proof}

% For vertices in the extended witness graph with all timestamps is $\bot$, we also define the extended bad vertices, bad component and bad tree on them.

% \begin{definition}[Bad vertices, bad component, bad tree on the extended witness graph]
% \label{definition:bad-vertices-components-trees-extended-witness-graph}
%     Fix $T \ge n$. We define the following quantities related to the $T$-step systematic scan Glauber dynamics (\Cref{definition:complex-MCMC}) and the corresponding extended witness graph (\Cref{definition:extend-witness-graph}).
%     \begin{itemize}
%         \item let the set of \emph{bad vertices} in $G_H^*$ be the set containing $\ts(V, 0)$ and  vertices such that all $r_t$ evaluates to $\bot$ for every timestamp $t$ included, i.e.,
%         \[
%         V^{*, \-{bad}} := \{v \in V_H^*: \forall t \in v, r_t = \bot\} \cup \{\ts(V, 0)\};
%         \]
%         \item let $G_H^*[V^{*, \-{bad}}]$ be the subgraph of  $G_H^*$ induced by $V^{*, \-{bad}}$;
%         \item let the \emph{bad component}  $\+C^\-{bad} \subset V^{*, \-{bad}}$ be the maximal set vertices in $V^{*, \-{bad}}$ containing $\ts(V, 0)$ that is connected in $G_H^*[V^{*, \-{bad}}]$. 
%         \item let the \emph{bad tree} $\+T^\-{bad} \subseteq V^{*, \-{bad}}$ be the $2$-tree of the induced subgraph $G_H^*[C^\-{bad}]$ containing $\ts(V, 0)$ constructed \Cref{lemma:2-tree-construction-one-large-degree}. Let $\=T^\-{bad}$ be a function that $\=T^\-{bad}(\+C^\-{bad}) = \+T^\-{bad}$.
%     \end{itemize}
% \end{definition}

% Then we analyse the degree on the extended witness graph.

% \begin{lemma}
% \label{lemma:maximum-degree-extended-witness-graph}
% In graph $G_H^*$, $\-{deg}(\ts(V, 0)) \le 2\abs{\+E} \Delta k^2$ and $\forall e \in V_H^*, e \neq \ts(V, 0)$, $\-{deg}(e) \le 2 \Delta k^2$.
% \end{lemma}

% \begin{proof}
%     Recall \Cref{lemma:witness-graph-degree-bound}, $\-{deg}(\ts(V, 0)) \le \sum_{e \in \+E} \deg(\ts(e, 0)) \le 2 \abs{\+E} \Delta k^2$. For other vertices, the degree can only increase $1$ because we only add one vertex $\ts(V, 0)$.
% \end{proof}

% We also introduce the following lemma to bound the number of $2$-trees on graph $G_H^*$ rooted at $\ts(V, 0)$.

% \begin{lemma}
%     \label{lemma:subtree-bound-large-degree}
%     Let $G=(V, E)$ be a graph, let $v\in V$ $\mathrm{deg}(v) \le D$ and $\forall u \neq v, \mathrm{deg}(u) \le d$. The number of subtrees of $G$ with $i\ge 2$ nodes containing $v$ is at most $\binom{D + i - 2}{D - 1} (\mathrm{e} d)^{i - 1}$ .
% \end{lemma}
% \begin{proof}
%     Recall \Cref{lemma:bound-subtree}, let $f(x) = \sum_{i=0}^{\infty} ( \mathrm{e} d x)^i = \frac{1}{1 - \mathrm{e} d }$. It holds that for a graph with maximum degree $\Delta$, the number of $i\ge 2$ nodes containing a fixed vertex is upper bounded by $\left[x^i\right] f(x)$.
%     By the multiplicative principle, the number of subtrees in $G$ with $i \ge 2$ nodes containing $v$ is bounded by $\left[x^i\right]\left(1 + xf(x)^{D}\right)$.

%     \begin{align*}
%         &\left[x^i\right]\left(1 + x \cdot f(x)^{D}\right)
%         \\
%         =&\left[x^i\right]\left(1 + x \cdot \left(\frac{1}{1 - \mathrm{e} d }\right)^{D}\right)
%         \\
%         =&\left[x^{i-1}\right] \left(\frac{1}{1 - \mathrm{e} d }\right)^{D}
%         \\
%         (\text{by Newton's binomial theorem})\quad=& \binom{D + i - 2}{D - 1} (\mathrm{e} d)^{i - 1}.
%     \end{align*}
% \end{proof}

% Now we bound the 2-tree in $G_H^*$ containing $\ts(V,0)$. 
% \begin{corollary}
% \label{corollary:2-tree-bound-extended-witness-graph}
% The number of $2$-trees in $G_H^*$ of size $i \ge 2$ containing $\ts(V, 0)$ is at most 
% \[\binom{4 \abs{\+E}^2 \Delta^2 k^4 + i - 2}{4 \abs{\+E}^2 \Delta^2 k^4-1} (4 \mathrm{e} \Delta^2 k^4)^{i - 1}.\]
% \end{corollary}
% \begin{proof}
%     % We first include the following lemma 
%     Consider the graph $G_H^{*^2} = (V_H^*, E_H^{*^2})$ such that $(u, v) \in E_H^{*^2}$ if and only if $1\le\-{d}(u,v) \le 2$ in graph $G_H^*$. 
%     Because $\ts(V, 0)$ must be in $2$-tree due to the \Cref{lemma:2-tree-construction-one-large-degree}. We can remove $N(\ts(V, 0))$ to form a new graph $G_H^{\top} = G_H^{*^2}[V_H^* \backslash N(\ts(V, 0)) ]=(V_H^{\top}, E_H^{\top})$.  Any $2$-tree containing $\ts(V,0)$ in $G_H^*$ is a subtree containing $\ts(V, 0)$ in $G_H^{\top}$. It suffices to bound the number of subtrees containing $\ts(V, 0)$ in $G_H^{\top}$.
%     % \yxtodo{Give a general lemma here.}
    
%     In graph $G_H^{\top}$, $\-{deg}(\ts(V, 0)) \le 4 \abs{\+E}^2 \Delta^2 k^4$ and $\forall u \in V_H^*, u \neq \ts(V, 0)$, $\-{deg}(u) \le 4\Delta^2 k^4$. By \Cref{lemma:subtree-bound-large-degree}, the number of subtrees containing $\ts(V,0)$ in $G_H^\top$ is bounded by $\binom{4 \abs{\+E}^2 \Delta^2 k^4 + i - 2}{4 \abs{\+E}^2 \Delta^2 k^4-1} (4 \mathrm{e} \Delta^2 k^4)^{i - 1}$.
% \end{proof}

% \subsection{Adapted framework for the extended witness graph} \label{subsection:convergence-adapted-framework}
% In this subsection, we define the decay of bad trees and the zero-one law of outcomes on the extended witness tree. The definition is slightly different from those in \Cref{subsection:framework-marginal-ratio} due to the $\ts(V, 0)$.

% \begin{definition}[decay of bad trees on the extended witness graph]
% \label{definition:convergence-bad-tree-decay}
% We say the bad trees decay with decay rate $(a, b)$, $a < 1, b \ge 1$, if for any bad tree $T^\-{bad}$, let $N^2(T) = \{u | u \in V_H^S, 1\le \-{dist}(u, T) \le 2\}$, the following equation holds,
% \[
% \sum_{\substack{C: \=T(C) = T^\-{bad} \\ \tau \in \{0,1\}^C}} \left| \mu^\-{GD}_\infty\left(\+T^\-{bad}=T^\-{bad},\+C^\-{bad}= C,\sigma(C) = \tau\right) \right| 
% % \le a^{k \abs{T^*}} b^{\abs{S} + k \abs{N^2(T)}}
% \le a^{k (\abs{T^\-{bad}}-1)} b^{k \abs{N^2(T)} + \abs{V}}.
% \]
% \end{definition}

% Similar to \Cref{lemma:framework-marginal-lower-bound-to-bad-tree-decay}, we introduce the next lemma to establish the decay of bad trees on the extended witness graph through marginal lower bound. We defer the proof to the end of this subsection.

% \begin{lemma}\label{lemma:convergence-marginal-bad-tree-decay}
%     If the stationary measure $\mu$ is $(\ell^\-{pad}, \ell)$-marginally lower bounded, the decay of bad trees on the extended witness graph with decay rate $(\ell^\-{pad}, \ell)$ holds.
% \end{lemma}

% \begin{lemma}[Zero-one law of outcomes]
% \label{lemma:convergence-zero-one-law-outcome}
%   For any bad component $C$ and configuration $\tau$ on $C$, we say the zero-one law of outcomes holds if for any configuration $\tau^* \in \{0,1\}^{\ts(V, 0)}$ on $\ts(V, 0)$, the following equation holds, 
% \[
% \mu^{\-{GD}}_{\infty}\left(\sigma(\ts(V,0)) = \tau^* \mid \+C^{\-{bad}}=C, \sigma(C) = \tau\right) = 0 \text{ or }1.
% \]
% \end{lemma}
% \begin{proof}
%     It holds that $\ts(V, 0) \in C$ due to the construction of bad components in \Cref{definition:extend-witness-graph}. So it holds that $\sigma(\ts(V, 0)) = \tau(\ts(V, 0))$.
% \end{proof}

% Now we give the proof of \Cref{lemma:convergence-marginal-bad-tree-decay}. The proof almost follows that of \Cref{lemma:framework-marginal-lower-bound-to-bad-tree-decay}.
% \begin{proof}[Proof of \Cref{lemma:convergence-marginal-bad-tree-decay}]
%     Given $\+T^\-{bad} = T^\-{bad}$.
%     Let $U = T \cup N^2(T)$, $T^* = T \backslash \{\ts(V, 0)\}$. 
% % Let $T^* = T \backslash \{\ts(S, 0)\}$, we will treat $\ts(S, 0)$ differently from other vertices in $T$ because for $t \in \ts(S, 0)$, $r_t$ may not be $\bot$. 
% Note $N^2(T)$ contains all vertices for all possible bad components and their neighbors except $T$ itself due to \Cref{definition:stationary-start} and \Cref{definition:bad-vertices-components-trees-extended-witness-graph}. 
% We sort the timestamps in $U$ forming a sequence $\-{TP} = (t_1, t_2, \dots, t_m)$ such that $t_1 < t_2 < \dots < t_m$.

% Recall the definition of the decomposed systematics scan Glauber dynamics (\Cref{definition:decomposed-systematic-scan-glauber-dynamics}), each time $t$ is associated with $r_t$ and $c_t$. We define the vector form of $r$'s and $c$'s as $\vec{r} = (r_{t_1},r_{t_2}, \dots, r_{t_m})$, $\vec{c} = (c_{t_1}, c_{t_2}, \dots, c_{t_m})$.Note if $\vec{c}$ is fixed, the configuration on $C$ is fixed.

% Define 
% \[\Omega_T = \{(\vec{r}, \vec{c}) \mid (\vec{r}, \vec{c}) \in ([q] \cup \{\bot\})^{U} \times [q]^U\, \mu_\infty^\-{GD}(\vec{r}, \vec{c} \ mid \+T^\-{bad} = T )\},\]
% be the set containing all possible $(\vec{r},\vec{c})$'s on $U$, note this set is finite due to the size limit of bad component given the bad tree. 
% We abuse the notation a little, let $\mu^{\-{pad}, \vec{r}, \vec{c}}_{v_{i(t)}}(c_{t_i})$ be the padding measure condition on $\vec{r}, \vec{c}$ except $r_{t_i}$ and $c_{t_i}$ as \Cref{definition:decomposition-scheme}.  
% We say $t \in T$ if $\exists v \in T, t \in v$.

% Given $\+C^\-{bad} = C, \vec{r}, \vec{c}$, we can calculate $\abs{\mu_\infty^\-{GD}\left( \+T^\-{bad} = T, \+C^\-{bad} = C, \vec{r}, \vec{c} \right)}$ via the following procedure.

% \begin{enumerate}
%     \item We enumerate all timestamps in $C$ by their orders in $\-{TP}$;
%     \item For the $i$-th timestamps, let $v = v_{i(t_i)}$,
%     \begin{itemize}
%         \item if $r_{t_i} = \bot$, it contributes $\abs{\mu^\-{LB}_{v}(\bot)} \cdot \abs{\mu^{\-{pad}, \vec{r}, \vec{c}}_{v}(c_{t_i})}$.
%         \item otherwise, it contributes $\abs{\mu^\-{LB}_{v}(c_{t_i})}$.
%     \end{itemize}
% \end{enumerate}

% Now let $R_i = \{\{(r_1,\tau_{1}), (r_2,\tau_2), \dots, (r_i,\tau_i)\} \mid (\vec{r}, \vec{\tau}) \in \Omega_T\}$ be the set containing all possible $r$'s and $\tau$'s of the first $i$ timestamps in the order of $\-{TP}$.

% Set 
% \[
% A_i = \sum\limits_{(\vec{r},\vec{\tau}) \in R_i} \prod\limits_{j \le i} \left( \sum\limits_{a=1}^q \mu^\-{LB}_{v_{i(t_j)}}(a)\cdot \=I[r_j = a] + \ell^\-{pad} \cdot \=I[r_j = \bot] \right).
% \]

% By the aforementioned procedure, it holds that,

% \[
% \sum\limits_{
% \substack{
% C: \=T(C) = T \\
% (\vec{r},\vec{c}) \in \Omega_T
% }}
% \abs{\mu^\-{GD}_\infty \left( \+T^\-{bad} = T, \+C^\-{bad} = C, \vec{r}, \vec{c} \right)}
% \le A_m.
% \]

% We show that $A_m \le \left( \ell^\-{pad} \right)^{ k \abs{T^*}} \ell^{k \abs{N^2(T)} + \abs{V}}$ by induction. Specifically, we prove 

% \[A_i \le \left( \ell^\-{pad} \right)^{\abs{\{t_j \mid t_j \in T^*, j\le p \}}} \ell^{i - \abs{\{t_j \mid t_j \in T^*, j\le p \}}}.\]

% For the base case, we set $A_0 = 1$.
% Assume it holds for $i < p$, for $i = p$,
% \begin{itemize}
%     \item if $t_i \in T^*$, it contributes at most $\ell^\-{pad}$ in all possible bad components. So 
%     \[A_p \le A_{p-1} \ell^\-{pad} \le \left( \ell^\-{pad} \right)^{\abs{\{t_j \mid t_j \in T^*, j\le p \}}} \ell^{i - \abs{\{t_j \mid t_j \in T^*, j\le p \}}}.\]
%     \item otherwise, if we fix a bad component, there are $3$ possible cases:
%     \begin{itemize}
%         \item if $t_i \in \ts(V, 0)$, it contributes at most $\ell$;
%         \item if $t_i \notin T$ and $t_i$ is not in the bad component nor is neighbors, it contributes $1 \le \ell$;
%         \item If $t_i \notin T$ and $t_i$ is in the bad component or its neighbors, it contributes at most $\ell$.
%     \end{itemize}
%      So
%     \[A_p \le A_{p-1} \ell \le \left( \ell^\-{pad} \right)^{\abs{\{t_j \mid t_j \in T^*, j\le p \}}} \ell^{i - \abs{\{t_j \mid t_j \in T^*, j\le p \}}}.\]
% \end{itemize}

% So it holds that,

% \[
% \sum\limits_{
% \substack{
% C: \=T(C) = T \\
% (\vec{r},\vec{c}) \in \Omega_T
% }}
% \abs{\mu^\-{GD}_\infty \left( \+T^\-{bad} = T, \+C^\-{bad} = C, \vec{r}, \vec{c} \right)}
% \le \left( \ell^\-{pad} \right)^{k \abs{T^*}} \ell^{m - k \abs{T^*}}
% \le \left( \ell^\-{pad} \right)^{k(\abs{T}-1)} \ell^{k \abs{N^2(T)} + \abs{V}}.
% \]
% Also let $\vec{c} = (\tau_{t_1}, \tau_{t_2}, \dots, \tau_{t_m})$. By triangle inequality, 
% \[
% \abs{\mu^\-{GD}_\infty\left( \+T^\-{bad}=T, \+C^\-{bad}=C, \sigma(C) = \tau \right)} 
% \le
% \sum\limits_{\vec{r} \in \{0,1\}^C}
% \abs{\mu^\-{GD}_\infty \left( \+T^\-{bad}=T, \+C^\-{bad}=C, \vec{r}, \vec{c}  \right)}.
% \]

% So this lemma holds.
% \end{proof}

% % We still follow the framework defined in \Cref{subsection:framework-marginal-ratio} with some extra lemmas to handle the one potential large-degree vertex.
% % \yxtodo{Create a new subsection for the extended witness graph. And state the zero-one law of the outcome explicitly. (In the former definition in section 2, |S|=k)}
% % We will show a variant of bad tree decay (\Cref{definition:framework-bad-tree-decay}) and outcome bound (\Cref{definition:framework-zero-one-law-outcome}). 

% \subsection{Proof of the convergence}

% We will prove that under the following lemma which implies that under the same conditions of \Cref{theorem:zero-freeness-his-lee-yang} the \Cref{theorem:zero-freeness-his-fisher}, the systematic scan Glauber dynamics converges to the stationary measure agnostic of the starting state.

% \begin{lemma}\label{lemma:convergence-lemma}
% For any $k$-uniform hypergraph $H = (V, \+E)$ with maximum degree $\Delta$, if the partition function $Z$ is non-zero, the stationary measure $\mu$ is $(\ell^\-{pad}, \ell)$-marginally bounded and furthermore it holds that,
% \[
% \left( \ell^\-{pad} \right)^{k i} \ell^{4 \Delta^2 k^5 i} \le \left(4 \mathrm{e} \Delta^2 k^4\right)^{-i}.
% \]

% Then the complex systematic scan Glauber dynamics converges. Furthermore, $\forall \tau^* \in \{0,1\}^{\abs{V}}$ it holds that,
 
%  \[
%  \forall \tau  \in \-{supp}(\mu), \lim\limits_{T \to \infty} \abs{\mu^\-{GD}_{T, \tau}(\sigma_0 = \tau^*) - \mu(\tau^*)} = 0,
%  \]
% \end{lemma}
% In order to prove \Cref{theorem:restatement-convergence-area-complex-mcmc}, it suffices to prove \Cref{lemma:convergence-lemma}.
% \begin{proof}[Proof of \Cref{theorem:restatement-convergence-area-complex-mcmc}]
%  It suffices to check the conditions in  \Cref{lemma:convergence-lemma}. By \Cref{lemma:his-lee-yang-bad-tree-decay} and \Cref{lemma:his-fisher-bad-tree-decay}, the conditions of \Cref{lemma:convergence-lemma} hold.
% \end{proof}

% % Recall the analysis in the previous subsection, we will 


% % In this subsection
% % Recall the witness graph (\Cref{definition:witness-graph-indset}) is introduced to bound the marginal measure on an edge. To handle the convergence on $V$, we introduce the extended witness graph and a few properties of it.


% % As the argument in the previous subsection, we introduce the following lemma to control 
% % \[\sum\limits_{\=T(C^\-{bad}) = T^\-{bad}}\abs{\mu_{T}^\-{GD}\left(T^\-{bad}, C^\-{bad}\right)},\] here following .
% % The intuition is that for small bad components whose neighbors do not reach the time $-T$, the measures of them are not related to the starting state. And for large bad components, we show that their contribution of them tends to $0$ when $T \to \infty$.

% % We show the bad tree decay as the next lemma and recall the proof outline, we will use this lemma to show that the contributions of type (2) bad components tend to $0$ when $T \to \infty$.

% Before proving \Cref{lemma:convergence-lemma}, we collect some useful lemmas. The first lemma establishes the decay of bad trees on the extended witness graph under the conditions of \Cref{lemma:convergence-lemma}.

% \begin{lemma}
% \label{lemma:convergence-bad-tree-decay}
%     Suppose the conditions of \Cref{lemma:convergence-lemma}, for any $v \in V$ and extended bad tree $T^{\-{bad}}$. For brevity of the presentation, let $A = \left(\ell^\-{pad}\right)^{-1} \ell^{4 \abs{\+E}^2 \Delta^2 k^5}$ which is a constant with $T$. It holds that,

%     \[
%     \sum\limits_{C:\=T(C) = T^\-{bad}}\abs{\mu_{T}^\-{GD}\left(\+T^\-{bad} = T^\-{bad}, C^\-{bad} =  C\right)} \le A
% \left( 4 \Delta^2 k^4 \right)^{-\abs{T^\-{bad}}}
%     \]
% \end{lemma}

% \begin{proof}
% Recall the definition of decay of bad trees on the extended witness graph (\Cref{definition:framework-bad-tree-decay}) and \Cref{lemma:framework-marginal-lower-bound-to-bad-tree-decay}, it holds that,
% \[
% \sum_{\substack{C: \=T(C) = T^\-{bad} \\ \tau \in \{0,1\}^C}} \left| \mu^\-{GD}_\infty\left(\+T^\-{bad}=T^\-{bad},\+C^\-{bad}= C,\sigma(C) = \tau\right) \right| 
% % \le a^{k \abs{T^*}} b^{\abs{S} + k \abs{N^2(T)}}
% \le \left(\ell^\-{pad}\right)^{k \left(\abs{T^\-{bad}}-1\right)} \ell^{k \abs{N^2(T)} + \abs{V}}.
% \]

% Now we bound $\abs{N^2(T^\-{bad})}$ on $G_H^*$. By \Cref{lemma:maximum-degree-extended-witness-graph} the degree of  $\ts(V, 0)$ is at most $2 \abs{\+E} \Delta k^2$ and the maximum degree of $G_H^*$ is at most $2 \abs{\+E} \Delta k^2$. So $N^2(\{\ts(V, 0)\}) \le 4 \abs{\+E}^2 \Delta^2 k^4$. For any vertex $v$ in $T^\-{bad}$ and $v \neq \ts(V, 0)$, we know their distance is at least $2$ due to \Cref{lemma:2-tree-construction-one-large-degree}. We know for any vertex $v \neq \ts(V, 0)$, the degree of it is at most $2 \Delta k^2$. So $N^2(\{v\}) \le 4\Delta^2 k^4$ for $v \in T^\-{bad}$ and $v \neq \ts(V, 0)$. So it holds that

% \[
% \abs{N^2(T^\-{bad})} \le 4 \abs{\+E}^2 \Delta^2 k^4 + 4\Delta^2 k^4\left(\abs{T^\-{bad}}-1\right).
% \]

% By \Cref{lemma:framework-marginal-lower-bound-to-bad-tree-decay},

% \begin{align*}
%     &\sum\limits_{\substack{C:\=T(C) = T^\-{bad} \\ \tau \in \{0,1\}^C}}\abs{\mu_{T}^\-{GD}\left(\+T^\-{bad}=T^\-{bad}, \+C^\-{bad} = C, \sigma(C) = \tau\right)} \\
%     \le& \left( \ell^\-{pad} \right)^{k \left(\abs{T^\-{bad}}-1\right)} \ell^{k \abs{N^2(T^\-{bad})}+ \abs{V}} \\
%     \le& \left( \ell^\-{pad} \right)^{k \left(\abs{T^\-{bad}}-1\right)} \ell^{4\abs{\+E}^2 \Delta^2 k^5 + \abs{V} + 4\Delta^2 k^5 \abs{T^\-{bad}} } \\
%     \le& A\left( 4 \Delta^2 k^4 \right)^{-\abs{T^\-{bad}}}
% \end{align*}

% % By \Cref{lemma:fram}
% % Given the size $\abs{C^\-{bad}}$, we can use \Cref{lemma:2-tree-construction-one-large-degree} to construct the bad tree $T^\-{bad}$ such that $\abs{T^\-{bad}} \ge \lfloor \abs{(C^\-{bad}} - 2\abs{\+E} \Delta k^2) / (2 \Delta k^2 + 1) \rfloor $.  So $\abs{N^2(T)} \le (2\Delta k^2 + 1) \abs{T} + 2 \abs{\+E}\Delta k^2$.

% % The event $T^\-{bad}$ can be translated to the following:
% % \begin{enumerate}
% %     \item\label{item:extended-bad-tree-case1} for each $x \in T^\-{bad}$, we have $r_t = \bot$ for all $t \in x$;
% %     \item\label{item:extended-bad-tree-case2} the $r_t$s on all other vertices in $G_H^*$ that is within distance $2$ of $T^\-{bad}$ satisfy certain restrictions so that $T^\-{bad}$ forms.
% % \end{enumerate}

% % Note that the event $T^\-{bad}$ is determined only by $\{r_t\}_{t=-T}^{0}$ and $\{r_t\}_{t=-T}^0$ follows a product measure. 
% % Therefore the \Cref{item:extended-bad-tree-case1} contributes a factor at most $\abs{\frac{\lambda}{1+\lambda}}^{k \abs{T^\-{bad}}}$ by the definition of 2-trees that all vertices in $\+T^\-{bad}$ contain disjoint timestamps and there are at most $n$ vertices with containing only one timestamp and $\abs{\frac{\lambda}{1+ \lambda}} \le 1$. 
% % We can use a simple triangle inequality to bound \Cref{item:extended-bad-tree-case2}. 
% % Since there are at most $\abs{T^\-{bad}} \cdot 4 \Delta^2 k^4 + 2 \abs{\+E} \Delta k^2 + 1$ vertices and therefore at most $k \left(\abs{T^\-{bad}} \cdot 4 \Delta^2 k^4 + 2 \abs{\+E} \Delta k^2 + 1\right)$ timestamps included, also consider that the $\sigma_T$ pin the configuration on subset of the possible timestamps which contributes $1 \le \abs{\frac{\lambda}{1+\lambda}} + \abs{\frac{1}{1+\lambda}}$. 
% % For the timestamps that are not pinned, they also contribute at most $\abs{\frac{\lambda}{1+\lambda}} + \abs{\frac{1}{1+\lambda}}$. 
% % So \Cref{item:extended-bad-tree-case2} contributes a factor of at most $\left( \abs{\frac{\lambda}{1+\lambda}} + \abs{\frac{1}{1+\lambda}}\right)^{k \left(\abs{T^\-{bad}} \cdot 4 \Delta^2 k^4 + 2 \abs{\+E} \Delta k^2 + 1\right)}$.

% % \begin{align*}
% % \sum\limits_{\=T(C^\-{bad}) = T^\-{bad}}\abs{\mu_{T}^\-{GD}\left(T^\-{bad}, C^\-{bad}\right)}
% % % \\
% % \le&
% % \abs{\frac{\lambda}{1+\lambda}}^{k \abs{T^\-{bad}}}
% % \left( \abs{\frac{\lambda}{1+\lambda}} + \abs{\frac{1}{1+\lambda}}\right)^{k \left(\abs{T^\-{bad}} \cdot 4 \Delta^2 k^4 + 2 \abs{\+E} \Delta k^2 + 1\right)}
% % \\
% % \le&
% % A
% % \abs{\frac{\lambda}{1+\lambda}}^{k \abs{T^\-{bad}}}
% % \left( \abs{\frac{\lambda}{1+\lambda}} + \abs{\frac{1}{1+\lambda}}\right)^{ \left(\abs{T^\-{bad}} \cdot 4 \Delta^2 k^5\right)}
% % \\
% % \le&
% % A
% % \abs{\frac{\`R(\lambda) + \varepsilon}{1+\`R(\lambda) - \varepsilon}}^{k \abs{T^\-{bad}}}
% % \left( \frac{1+\varepsilon}{1 - \varepsilon} \right)^{4 \abs{T^\-{bad}} \Delta^2 k^5}
% % \\
% % % \le&
% % % \abs{\frac{\lambda}{1+\lambda}}^{-k n}
% % % \left( 2 \mathrm{e} \Delta k^2  \right)^{-2 \abs{T^\-{bad}_v}}
% % % \cdot
% % % \mathrm{e}^{3\abs{T^\-{bad}_v}}
% % % \\
% % \le&
% % A
% % \left( 4 \Delta^2 k^4 \right)^{-\abs{T^\-{bad}}}.
% % \end{align*}



% \end{proof}

% % \Cref{lemma:bad-component-bound-conditioned} implies the following two bounds.

% % \begin{corollary}
% % \label{corollary:bad-component-condition-bound}
% %     Suppose the conditions of \Cref{lemma:his-lee-yang-marginal}, for any $v \in V$ and extended bad vertices $V^{*, \-{bad}}$. Let $I = \{ u \mid C^\-{bad}_u \neq C^\-{bad}_v \}$, for any $S \subseteq I$, it holds that,
% %     \[
% %     \abs{\mu_{T}^\-{GD}\left(C^\-{bad}_v \mid \bigcup_{i \in S} C^\-{bad}_i  \right)} \le \abs{\frac{\lambda}{1+\lambda}}^{-k n}.
% %     \]
% % \end{corollary}

% % \begin{corollary}
% % \label{corollary:bad-component-no-condition-bound}
% %     Suppose the conditions of \Cref{lemma:his-lee-yang-marginal}, for any $v \in V$ and extended bad vertices $V^{*, \-{bad}}$. It holds that,
% %     \[
% %     \abs{\mu_{T}^\-{GD}\left(C^\-{bad}_v\right)} \le \abs{\frac{\lambda}{1+\lambda}}^{-k n}
% %     \left( \frac{4 \Delta^2 k^4}{\mathrm{e}} \right)^{-\abs{T^\-{bad}_v}}.
% %     \]
% % \end{corollary}

% Recall in the beginning of this section, we divide the processes into $2$ types. 
% The next lemma is used to show that the contributions of the first type are equal for different starting states.

% \begin{lemma}\label{lemma:convergence-truncated-equal}
%     Given the starting time $-T$ and a bad component $C^\-{bad}$. If timestamps $t \in C^\-{bad}$ satisfy $t > -T + \abs{V} $, then for arbitrary initialization state $\tau, \tau' \in \{0,1\}^{\abs{V}}$, it holds that,
%     \[
%     \mu^\-{GD}_{T, \tau}\left(\+C^\-{bad} = C^\-{bad}\right) = \mu^\-{GD}_{T, \tau'}\left(\+C^\-{bad} = C^\-{bad}\right)
%     \]
    
% \end{lemma}
% \begin{proof}
%     Recall the \Cref{definition:extend-witness-graph}, if for all $t \in C^\-{bad}$, $t>-T+\abs{V}$, it holds that all timestamps in $N(C^\-{bad})$ are greater than $-T$. 

%     So $\mu^\-{GD}_{T, \tau}(\+C^\-{bad} = C^\-{bad})$ and $\mu^\-{GD}_{T, \tau'}(\+C^\-{bad} = C^\-{bad})$ are not related to the initialization by \Cref{definition:decomposed-systematic-scan-glauber-dynamics}. So they are equal.
%     % This implies that they are equal because they are equal under arbitrary $\{r_i\}_{i=-T}^{0}$.
% \end{proof}

% Now it's ready to prove \Cref{lemma:convergence-lemma}.

% \begin{proof}[Proof of \Cref{lemma:convergence-lemma}]
% Suppose the conditions of \Cref{lemma:convergence-lemma}, we first show that it converges.

% Let $C^{\-{bad}, \top} = \{C^\-{bad} \mid \exists t \in C^\-{bad}, t \le -T + \abs{V}\}$ be the set of possible extended bad components such that the minimal timestamp in them is not greater than $-T + \abs{V}$. With \Cref{lemma:convergence-truncated-equal} and \Cref{lemma:convergence-zero-one-law-outcome}, it holds that

% \begin{align*}
%     &\abs{\mu_{T, \tau}\left(\sigma_0 = \tau^*\right)-\mu_{T, \tau'}\left(\sigma_0 = \tau^*\right)}\\
%     = &\left|
%     \sum\limits_{S} \mu^{\-{GD}}_{T,\tau}\left(\+C^{\-{bad}}=S\right) \mu^{\-{GD}}_{T,\tau}\left(\sigma(\ts(V,0)) = \tau^* \mid \+C^{\-{bad}}=S\right)\right. \\
%     &\qquad \left.-
%     \sum\limits_{S} \mu^{\-{GD}}_{T,\tau}\left(\+C^{\-{bad}}=S\right) \mu^{\-{GD}}_{T,\tau}\left(\sigma(\ts(V,0)) = \tau^* \mid \+C^{\-{bad}}=S\right) 
%     \right|\\
%     =&\left|
%     \sum\limits_{S \in C^{\-{bad}, \top}} \mu^{\-{GD}}_{T,\tau}\left(C^{\-{bad}}=S\right) \mu^{\-{GD}}_{T,\tau}\left(\sigma(\ts(V,0)) = \tau^* \mid \+C^{\-{bad}}=S\right) \right.\\
%     &\qquad \left.-
%     \sum\limits_{S \in C^{\-{bad}, \top}} \mu^{\-{GD}}_{T,\tau'}\left(C^{\-{bad}}=S\right) \mu^{\-{GD}}_{T,\tau'}\left(\sigma(\ts(V,0)) = \tau^* \mid \+C^{\-{bad}}=S\right) \right|
%     \\
%     \le&
%     \sum\limits_{S \in C^{\-{bad}, \top}} \abs{\mu^{\-{GD}}_{T,\tau}\left(C^{\-{bad}}=S\right)}
%     +
%     \sum\limits_{S \in C^{\-{bad}, \top}} \abs{\mu^{\-{GD}}_{T,\tau'}\left(C^{\-{bad}}=S\right)},
% \end{align*}

% We bound the first quantity $\sum_{S \in \+C^{\-{bad}, \top}} \abs{\mu^{\-{GD}}_{T,\tau}\left(\+C^{\-{bad}}=S\right)}$ and the proof for the second quantity is similar.

% For $S \in C^{\-{bad}, \top}$, it holds that $\abs{S} \ge T/\abs{V} - 1$. So
% \begin{align*}
% &\sum\limits_{S \in C^{\-{bad}, \top}} \abs{\mu^{\-{GD}}_{T,\tau}(C^{\-{bad}}=S)}
% \\
% \le&
% \sum\limits_{i\ge T/\abs{V} - 1}
% \sum\limits_{T^\-{bad} \in \+T^\-{bad}_i}
% \sum\limits_{\substack{C: \=T(C) = T^\-{bad} \\ \tau \in \{0,1\}^{C}}}
% \abs{\mu_{T, \tau}^\-{GD}(\+T^\-{bad}=T^\-{bad}, \+C^\-{bad}=C, \sigma(C)=\tau)}
% \\
% (\text{by \Cref{lemma:convergence-bad-tree-decay}})\quad \le&
% A
% \sum\limits_{i\ge T/\abs{V} - 1}
% \sum\limits_{T^\-{bad} \in \+T^\-{bad}_i}
% \left( 4 \Delta^2 k^4 \right)^{-i}
% \\
% (\text{by \Cref{corollary:2-tree-bound-extended-witness-graph}})\quad\le&
% A
% \sum\limits_{i\ge T/\abs{V} - 1}
% \binom{4 \abs{\+E}^2 \Delta^2 k^4 + i - 2}{4 \abs{\+E}^2 \Delta^2 k^4 - 1} (4 \mathrm{e} \Delta^2 k^4)^{i - 1}
% \left( 4 \Delta^2 k^4 \right)^{-i}
% \\
% \le&
% A
% \sum\limits_{i\ge T/\abs{V} - 1}
% \binom{4 \abs{\+E}^2 \Delta^2 k^4 + i - 2}{4 \abs{\+E}^2 \Delta^2 k^4 - 1} 2^{-i}
% \\
% (\text{when $T$ is sufficiently large})\le&
% A
% \sum\limits_{i\ge T/\abs{V} - 1}
% \left(\frac{4 \abs{\+E}^2 \Delta^2 k^4 + i - 2}{4 \abs{\+E}^2 \Delta^2 k^4 - 1}\right)^{4 \abs{\+E}^2 \Delta^2 k^4}
% 2^{-i},
% \end{align*}

% whose limit is $0$ when $T \to \infty$.

% So it holds that 
% \[
% \forall \tau, \tau' \in \-{supp}(\mu), \lim\limits_{T \to \infty} \abs{\mu_{T, \tau}^\-{GD}(\sigma_0 = \tau^*) - \mu_{T, \tau'}^\-{GD}(\sigma_0 = \tau^*)} = 0.
% \]

% We also know $\mu$ is the stationary measure so that, 
% \[
% \forall \tau \in \-{supp}(\mu), \lim\limits_{T \to \infty} \abs{\mu_{T, \tau}^\-{GD}(\sigma_0 = \tau^*) - \mu(\tau^*)} = 0.
% \]
% % Pick $S \in \+C^{\-{bad}, \top}$, assume $S$ contains $j$ disjoint components $S_1, \cdots, S_j$. W.l.o.g. we assume $\exists t \in S_1, \text{s.t. } t \le -T + n$. By the chain rule,

% % \begin{align*}
% % &\abs{\mu_{T, \tau}^\-{GD}(S)} 
% % \\
% % =& \prod\limits_{i=1}^{j} \abs{\mu_{T, \tau}^\-{GD}\left(S_i \mid \bigcup\limits_{l<i} S_l \right)}  
% % \\
% % \text{(by \Cref{corollary:bad-component-condition-bound})} =& \abs{\frac{\lambda}{1 + \lambda}}^{-kn^2} \abs{\mu_{T, \tau}^\-{GD}(S_1)}. 
% % \end{align*}

% % With \Cref{corollary:bad-component-no-condition-bound}, it suffices to bound 

% % So
% % \begin{align*}
% % \sum\limits_{S \in \+C^{\-{bad}, \top}} \abs{\mu^{\-{GD}}_{T,\tau}(\+C^{\-{bad}}=S)}
% % \end{align*}

% \end{proof}

% \begin{comment}

% \begin{definition}[Marginal convergence of the systematic scan Glauber dynamics]
% The marginal measure $\mu_T(\sigma_0(e) = \tau_e)$ for $\forall e \in \+E, \tau_e \in \{0,1\}^{\abs{e}}$ of complex systematic scan Glauber dynamics (\Cref{definition:complex-MCMC}) converges agnostic of the starting state $\sigma_{-T}$ if 
% \[
% \forall e\in \+E, \tau, \tau' \in \-{supp}(\mu), \tau^*_e \in \{0,1\}^{\abs{e}}, \lim\limits_{T \to \infty} \abs{\mu_{T, \tau}^\-{GD}(\sigma_0(e) = \tau^*_e) - \mu_{T, \tau'}^\-{GD}(\sigma_0(e) = \tau^*_e)} = 0.
% \]
% \end{definition}
% \yxtodo{Try to strengthen this definition to make a true convergenc}

% Now we prove that under the assumptions of  \Cref{theorem:zero-freeness-his-lee-yang}, we can prove the following marginal convergence theorem,

% \begin{theorem}[Marginal convergence of the systematic scan Glauber dynamics for hypergraph independent sets]\label{theorem:complex-MCMC-convergence-his}
%     Suppose the condition of \Cref{lemma:his-lee-yang-marginal}. The complex systematic scan Glauber dynamics (\Cref{definition:complex-MCMC}) marginally converges.
% \end{theorem}

% % We define the extended bad components

% Fix $e \in \+E, \tau, \tau' \in \-{supp}(\mu), \tau_e^* \in \{0,1\}^e$,
% Let $\+C$ denote the set of bad components in $G^e_H=(V_H^e, E_H^e)$ that containing $\ts(e,0)$. We also define $\+C_i$ denote the set of bad components in $G^e_H$ containing $\ts(e,0)$ of size $i$.
% For each $i\geq 1$, and let $\+T_i$ denote the set of bad trees. 
% % Note that the induced measure on $\+C^{\-{bad}}$ is the same for the two complex processes with different starting configurations.

% \begin{lemma}\label{lemma:his-convergence-finite-truncation}
%     Fix $T$, let $n = \abs{V}, \forall C \in \bigcup_{i < T/n - 1} \+C_i$, vertices $C$ and its neighbors does not contain the timestamp $-T$. 
% \end{lemma}
% \begin{proof}
% \yxtodo{The bad tree here needs modification due to the specific pinning in e}
%     Assume $\ts(e',t) \in V_H^e$, $t \in [(k-1)n,kn)$, the timestamps of its neighbors must belong to $[(k-2)n, (k+1)n)$. Because we know that $\ts(e, 0) \in [0,-n)$, so the union of $\bigcup_{i < T/n -1} C_i$ and its neighbors' timestamps belong to $[0, -T - n)$ which does not contain $-T$.
% \end{proof}

% Then we introduce the following lemma to separate the $\mu_{T, \tau}^\-{GD}(\sigma_0(e) = \tau^*_e) $ and $ \mu_{T, \tau'}^\-{GD}(\sigma_0(e) = \tau^*_e)$ into two parts.

% \begin{lemma}\label{lemma:his-convergence-truncation}
%     For $S \in \bigcup_{i < T/n - 1} \+C_i$, it holds that for any $T, \tau, \tau' \in \-{supp}(\mu), \tau_e^* \in \{0,1\}^e$
%     \[
%         \mu_{T, \tau}^\-{GD}\left(\+C^\-{bad} = S\right) = \mu_{T, \tau'}^\-{GD}\left(\+C^\-{bad} = S\right).
%     \]
% \end{lemma}
% \begin{proof}
%     By \Cref{lemma:his-convergence-finite-truncation}, we know that for $S \in \bigcup_{i < T/n-1} \+C_i$, the union of $S$ and its neighbors' time tags does not contain the time tag $-T$. So any measure of $S$ does not relate to the $\sigma_{-T}$, so they are equal.
% \end{proof}

% Now it is ready to prove \Cref{theorem:complex-MCMC-convergence-his}

% \begin{proof}[Proof of \Cref{theorem:complex-MCMC-convergence-his}]
    
% \begin{align*}
%     &\abs{\mu_{T, \tau}^\-{GD}(\sigma_0(e) = \tau^*_e)-\mu_{T, \tau'}^\-{GD}(\sigma_0(e) = \tau^*_e)}\\
%     = &\abs{
%     \sum\limits_{S'\in \+C} \mu^{\-{GD}}_{T,\tau}(\+C^{\-{bad}}=S') \mu^{\-{GD}}_{T,\tau}(\sigma_0(e) = \tau^*_e \mid \+C^{\-{bad}}=S') 
%     -
%     \sum\limits_{S'\in \+C} \mu^{\-{GD}}_{T,\tau'}(\+C^{\-{bad}}=S') \mu^{\-{GD}}_{T,\tau'}(\sigma_0(e) = \tau^*_e \mid \+C^{\-{bad}}=S') 
%     }\\
%     =&
%     \abs{
%     \sum\limits_{\substack{i\ge T/n \\S'\in \+C_i}} \mu^{\-{GD}}_{T,\tau}(\+C^{\-{bad}}=S') \mu^{\-{GD}}_{T,\tau}(\sigma_0(e) = \tau^*_e \mid \+C^{\-{bad}}=S') 
%     -
%     \sum\limits_{\substack{i\ge T/n \\S'\in \+C_i}} \mu^{\-{GD}}_{T,\tau'}(\+C^{\-{bad}}=S') \mu^{\-{GD}}_{T,\tau'}(\sigma_0(e) = \tau^*_e \mid \+C^{\-{bad}}=S') 
%     }
%     \\
%     \le&
%     \sum\limits_{\substack{i\ge T/n \\S'\in \+C_i}} \abs{\mu^{\-{GD}}_{T,\tau}(\+C^{\-{bad}}=S')}
%     +
%     \sum\limits_{\substack{i\ge T/n \\S'\in \+C_i}} \abs{\mu^{\-{GD}}_{T,\tau'}(\+C^{\-{bad}}=S')}
%     \\
%     \le&
%     2^{-T/n+1},
% \end{align*}
% whose limit is $0$ when $T \to \infty$.
% \end{proof}
% \end{comment}

==> correlation_decay_witness_graph.tex <==
\section{Connection to complex correlation decay(not sure, constructing)}
\yxtodo{Check the connection between correlation decay and our framework}
In this section, we show the relation between our framework and the classical correlation decay property.

Take hardcore model $G = (V, E)$ as an example, we start the complex-valued systematic scan Glauber dynamics under the regime that the hardcore partition function is nonzero at time $-T$ with stationary distribution $\sigma_{-T}$.

Let the witness graph defined as $G^* = (V^*, E^*)$. 
\[
V^* = \{v^t_{i(t)} \mid 0 \le t < T \} \cup \{v^{-T} \mid v \in V\},
\]
\[
E^* = \{ (v^t_{i(t)}, v^{\mathrm{pred}_u(t)}_{i(\mathrm{pred}_u(t)})) \mid \forall 0 \le t < -T, \forall u (v_{i(t)}, u) \in E \}.
\]

Let $V^*_j = \{v_{i(t)} \mid j \le t < -T \} \cup \{v^{-T} \mid v \in V\}$, $G_j^* = G^*[V_j^*]$. 
Let $\mu_{G_j^*}$ be the hardcore measure on $G_j^*$ with pinning $\sigma_{-T}$.
We give the following lemma mapping the marginal ratio in dynamics into a marginal ratio hardcore model.

\begin{lemma}[Measure mapping]
Fix time $t$, for any configuration $\sigma$ on $V^*_t$, it holds that,
    \[
    \mu_{-T}^\-{GD}(\sigma) = \mu_{G_{t}^*}(\sigma)
    \]
\end{lemma}

\begin{proof}
    We prove this lemma by induction on $t$. For $t = -T$, it holds trivially because of the pinning.

    Now we assume that it holds for $t < k$, when $t = k$, 
    \begin{align*}
    \mu_{-T}^\-{GD}(\sigma) &= \sum_{\tau \in \{0,1\}^{V_{k-1}^*}} \mu_{-T}^\-{GD}(\tau) \mu^{\tau}(\sigma_{v_{i(k)}}) \\
    &= 
    \end{align*}
\end{proof}


==> counting_by_enumeration.tex <==
In this section, we give a simple approximation algorithm for marginal measures in complex settings using almost the same algorithm in \cite{feng2023towards} that simply enumerates all possible configurations on bad components of logarithmic size. Then use the standard edge-wise self-reducibility to reduce the approximating partition function into approximating marginal measures. We show this method for approximating the independence polynomial on Lee-Yang zeroes under almost the same conditions of \Cref{theorem:zero-freeness-his-lee-yang} as an example. Specifically, we prove the following theorem in this section.

\begin{theorem}\label{theorem:approx-his}
Fix $k \ge 2$, and $\Delta \ge 3$. For any $0 < \epsilon < \frac{1}{9k^5 \Delta^2}$, a constant $\eta \in [0, 1)$, let $[0, \lambda_{c, \varepsilon})$ be the real segment such that the following holds for all $\lambda \in [0, \lambda_{c, \varepsilon})$:

\begin{align}\label{eq:condition-counting}
    \left(\frac{\lambda+\varepsilon}{1+\lambda-\varepsilon}\right)^{k/2}< \sqrt{\eta} \cdot \frac{1}{2\sqrt{2}\mathrm{e}\Delta k^2}.
\end{align}

Define $\+D_{\varepsilon}$ as the connected complex region given by $\+D_{\varepsilon} \defeq \{z \in \=C \mid \exists \lambda \in [0, \lambda_{c, \varepsilon}) \text{s.t.} \abs{z - \lambda} \le \varepsilon \}$,
which is the union of disks of radius $\varepsilon$ centered at points on the segment $[0,\lambda_{c,\varepsilon})$. 

% for all $\lambda\in [0,c_{\varepsilon})$. Let $\+D_{\varepsilon}$ be the connected region in the complex plane obtained as the union of disks of radius $\varepsilon_{k,\Delta}$ centred at all points on the segment $[0,c_{\varepsilon})$. 

% define $\+D_{\varepsilon}\defeq\left\{z\in\mathbb{C}\mid \exists \beta\in[0,1]\text{ s.t. }|z-\beta|\le \varepsilon\right\}$ as the connected complex region formed by the union of disks of radius $\varepsilon$, centred at points on the segment $[0,1]$.

Then, for any $k$-uniform hypergraph $H = (V, \+E)$ with maximum degree $\Delta$, there is an FPTAS for the partition function $Z_H^\-{ly}(\*\lambda)$ for all $v \in V, \lambda_v \in \+D_{\varepsilon}^V$.
% with running time $O\left( \left(\frac{\abs{\+E}}{(1 - \eta) \varepsilon}\right)^{2 +2\Delta k^3 } \right)$.

% For $\lambda'\in \+D_{\varepsilon}$, there is an algorithm with approximation ratio $\varepsilon$ and time complexity $O\left( \left( \frac{m}{(1 - \eta)\varepsilon} \right)^{\-{poly}(\Delta, k)}   \right)$
\end{theorem}

% Fix a hypergraph 
For a $k$-uniform hypergraph $H=(V, \+E)$ satisfies the conditions in \Cref{theorem:zero-freeness-his-lee-yang}. Let $\varepsilon$ and $\+D_\varepsilon$ are defined as those in \Cref{theorem:zero-freeness-his-lee-yang}. Let $\*\lambda \in \+D_\varepsilon^{V}$. Let $Z_H^\-{ly}(\*\lambda)$ be the associating partition function.
We first define the approximate marginal measure and approximate partition function formally. 

Fix an arbitrary ordering of hyperedges $\+E = \{e_1, e_2, \ldots, e_m\}$. For each $0 \le i \le m$, let $\+E_i = \{e_1, e_2, \ldots, e_i\}$ and $H_i = (V, \+E_i)$. By \Cref{theorem:zero-freeness-his-lee-yang}, it holds that for each $0\le i \le m$, $Z_{H_i}^\-{ly}(\*\lambda) \neq 0$. Let $\mu_{H_i}$ be the associating stationary measure on $H_i$. For each $0\le i < m$, we define $\+R_i = \frac{Z_{H_{i+1}}^\-{ly}(\*\lambda)}{Z_{H_i}^\-{ly}(\*\lambda)}$ as the marginal measure, and from the proof of \Cref{theorem:zero-freeness-his-lee-yang}, it holds that,
\[\+R_i = \frac{Z_{H_{i+1}}^\-{ly}(\*\lambda)}{Z_{H_i}^\-{ly}(\*\lambda)} = 1 - \mu_{H_i}(\sigma(e_{i+1} = 1^{e_{i+1}})),\]

with this definition, the partition can be expressed by $Z_{H}^\-{ly}(\*\lambda) = Z_{H_{0}}^\-{ly}(\*\lambda) \prod_{i < m} \+R_i$.

Now we define the approximate marginal measure and the approximate partition function. For $0 \le i < m$, Set $S_i = e_{i+1}$, consider the witness graph $G_{H_i}^{S_i}$, let $\+C_j^i$ be the set of all bad components with size $j$.
Let $\gamma$ be a fixed constant that we will set later and $\kappa = 4\Delta^2 k^4\gamma$.
 We define the approximate marginal measure $\+R^*_i$ :
\[
\+R_i^* = 1 - \sum\limits_{\substack{j \le \kappa}}\sum\limits_{\+C \in \+C^i_j} \mu_{\infty, \*b}^\-{GD}(\sigma_0(e_{i+1}) = 1^{e_{i+1}}, \+C^\-{bad} = \+C),
\]
with this definition, we define approximate partition function as $Z_H^{\-{ly}, *}(\*\lambda) = Z_{H_0}^\-{ly}(\*\lambda) \prod_{i<m} \+R_i^*$.

We give the next lemma meaning that if we set $\gamma$ properly, $Z_H^{\-{ly},*}(\*\lambda)$ is an $\varepsilon$ multiplicative approximation of $Z_H^\-{ly}(\*\lambda)$.

\begin{lemma}\label{lemma:approx-partition}
Suppose the conditions in \Cref{theorem:approx-his}, let $\gamma > \left\lceil \log_2 \left( \frac{4 \abs{\+E}}{(1 - \eta)\epsilon} \right) \right\rceil$.
It holds that,
\[
\abs{\frac{Z_H^\-{ly}(\*\lambda) - Z_H^{\-{ly},*}(\*\lambda)}{Z_H^\-{ly}(\*\lambda)}} \le \varepsilon.
\]
\end{lemma}

The rest of this section is devoted to prove \Cref{lemma:approx-partition}. Note we have that,
\[\abs{\frac{Z_H^\-{ly}(\*\lambda) - Z_H^{\-{ly},*}(\*\lambda)}{Z_H^\-{ly}(\*\lambda)}} = \abs{1 - \prod\limits_{i=0}^{m-1} \frac{\+R_i^*}{\+R_i} }.\]

To prove $\Cref{lemma:approx-partition}$, it suffices to show that $\prod\limits_{i=0}^{m-1} \frac{\+R_i^*}{\+R_i}$ is close to $1$. To do that, we give the next lemma about the norms and arguments of $\+R_i$ and $\+R_i^*$ for each $0\le i < m$.

\begin{lemma}\label{lemma:approx-R-norm-argument}
Suppose the conditions in \Cref{theorem:approx-his}, for each $0 \le i < m$,
    It holds that,
    \begin{align}\label{eq:r-i-lowerbound}
        \abs{\+R_i} \ge 1 - \eta,
    \end{align}
    \begin{align}\label{eq:r-i-norm}
    1 - (1 - \eta)^{-1} 2^{-\gamma} \le \frac{\abs{\+R_i^*}}{\abs{\+R_i}} \le 1 + (1 - \eta)^{-1}2^{-\gamma},
    \end{align}
    \begin{align}\label{eq:r-i-argument}
        \abs{\Arg\left(\+R_i, \+R^*_i\right)} \le \frac{2^{-\gamma}}{1 - \eta}.
    \end{align}
\end{lemma}
\begin{proof}
    By going through the proof of \Cref{lemma:unified}-(\ref{item:unified-2}) while taking \eqref{eq:condition-counting} into account, it holds that,
    \[
        \abs{\mu_{\infty, \*b}^\-{GD}(\sigma_0(e_{i+1})) = 1^{e_{i+1}}} < \eta,
    \]
    so $\abs{\+R_i} = \abs{1 - \mu_{\infty, \*b}^\-{GD}(\sigma_0(e_{i+1})) = 1^{e_{i+1}}} \ge 1 - \eta$.
    Next, we bound $\abs{\+R_i - \+R_i^*}$. By the definition of $\+R_i$ and $\+R_i^*$, we have that,
    \begin{align}
        \abs{\+R_i - \+R_i^*}&=\abs{\sum\limits_{j > \kappa}\sum\limits_{\+C \in \+C_j^i} \mu_{\infty, \*b}^\-{GD}(\sigma_0(e_{i+1})= 1^{e_{i+1}}, \+C^\-{bad}=\+C)}\notag\\
        &\le\sum\limits_{j>\gamma}\sum\limits_{\+T \in \+T_j^i}\abs{\sum\limits_{\substack{\+C \in \=T_{i,j}^{-1}(\+T) \\ \abs{\+C} > \kappa}}\mu_{\infty, \*b}^\-{GD}(\sigma_0(e_{i+1})= 1^{e_{i+1}}, \+C^\-{bad}=\+C)} \notag\\
        &\le 2^{-\gamma},\label{eq:r-subtract}
    \end{align}
    % \todo{better to check here}
    where the first inequality is due to triangle inequality, the second inequality can derived by going through the proof of \Cref{lemma:unified}-(\ref{item:unified-2}) while taking \eqref{eq:condition-counting} into account.
    With this bound, we now prove \eqref{eq:r-i-norm}:
    \[
    \abs{\frac{\+R_i^*}{\+R_i}} = \abs{1 - \frac{\+R_i^* - \+R_i}{\+R_i}} \le 1 + (1 - \eta)^{-1}2^{-\gamma},
    \]
    \[
    \abs{\frac{\+R_i^*}{\+R_i}} = \abs{1 - \frac{\+R_i^* - \+R_i}{\+R_i}} \ge 1 - (1 - \eta)^{-1}2^{-\gamma}.
    \]
    Finally, we prove \eqref{eq:r-i-argument}.
    We first give a crude bound of $\abs{\Arg(\+R_i^*, \+R_i)}$. Note $\+R_i^*, \+R_i$ and $\+R_i^* - \+R_i$ form a triangle in the complex plane. We also know that $\abs{R_i} \ge 1 - \eta$ and $\abs{\+R_i - \+R_i^*} \le 2^{-\gamma}$, with $\gamma > \log_2 \left( \frac{4 \abs{\+E}}{(1 - \eta)\varepsilon} \right)$, we know that $\abs{\+R_i} > \abs{\+R_i - \+R_i^*}$ which implies that $\abs{\Arg(\+R_i^*, \+R_i)} < \frac{\pi}{2}$. With this crude bound, we now prove \eqref{eq:r-i-argument}:
    \begin{align*}
    &\abs{\Arg\left(\+R_i^*, \+R_i\right)} \\
    \left( x \le \tan(x) \text{ for } 0 \le x < \frac{\pi}{2} \right)\quad\le&
    \abs{\tan\left( \abs{\Arg\left(\+R_i^*, \+R_i\right)} \right)} \\
    \le &
    \abs{\frac{\abs{\+R_i^* - \+R_i}}{\abs{\+R_i^*}}} \\
    (\text{by \eqref{eq:r-subtract} and \eqref{eq:r-i-lowerbound}})\quad \le &
    \frac{2^{-\gamma}}{1 - \eta},
    \end{align*}
    which finishes the proof.
\end{proof}
% Before proving \Cref{lemma:approx-partition}, we first introduce a few lemmas about the norms and arguments of $\+R_i$ and $\+R_i^*$.

% Recall the definition of the edge-wise self-reducibility in \Cref{section:self-reducibility}, $\+G = (H = (V, \+E), (\phi_v)_{v\in V}, (\phi_e)_{e \in \+E})$. Let $\+R_i = \frac{Z_{\+G_i}}{Z_{\+G_{i-1}}}$, $\mu_i = \mu_{\+G_{i}}$ and we will omit $i$ and write $\mu$ when the context is clear and

% \[
% Z_\+G = Z_{\+G_{0}} \prod\limits_{1 \le i \le m} \+R_i.
% \]

% Fix $\gamma$. Let $\+C_j$ be the set containing all bad components with size $j$,
% \[\+R^*_i = 1 - \sum\limits_{\substack{j \le \gamma \\ C \in \+C_j}} \mu\left(\sigma_{\ts(e_i,0)} = 1^{\abs{e_i}}, \+C^\-{bad} = C\right).\]

% \[
% Z_\+G^* = Z_{\+G_0} \prod\limits_{1 \le i \le m} \+R^*_i
% \]
Now we are ready to prove \Cref{lemma:approx-partition}.
\begin{proof}[Proof of \Cref{lemma:approx-partition}]
\begin{align*}
    \abs{\frac{Z_H^\-{ly}(\*\lambda) - Z_H^{\-{ly},*}(\*\lambda)}{Z_H^\-{ly}(\*\lambda)}}
    = &
    \abs{1 - \prod\limits_{0 \le i < m}\frac{\+R_i^*}{\+R_i}}.
\end{align*}

By \Cref{lemma:approx-R-norm-argument}, we know that 
\[
\abs{\prod\limits_{i=0}^{m-1}\frac{\+R_i^*}{\+R_i}} \le (1 + 2^{-\gamma}/(1 - \eta))^m \le \exp\left( m 2^{-\gamma}/(1 - \eta) \right) \le \exp(\varepsilon/4),
\]

\[
\abs{\Arg\left( \prod\limits_{i=0}^{m-1}\frac{\+R_i^*}{\+R_i} \right)} \le m 2^{-\gamma}/(1 - \eta) \le \varepsilon/4.
\]

By the law of cosines, 

\begin{align*}
\abs{1 - \prod\limits_{i\ge 0}^{m-1}\frac{\+R_i^*}{\+R_i}} 
\le &
\sqrt{1 + \exp(\varepsilon/2) - 2 \exp(\varepsilon/4) \cos(\varepsilon/4) } \\
\le &
\varepsilon,
\end{align*}
which finishes the proof.
\end{proof}
% \begin{comment}
    
% Following the framework in \Cref{subsection:decomposition-schemes}, we introduce the bad tree decay like \Cref{lemma:his-lee-yang-bad-tree-decay} but with different parameters and defer its proof to the end of this section.

% \begin{lemma}\label{lemma:approx-bad-tree-decay}
% % % \end{comment}
% % Fix any $k$-uniform hypergraph $H=(V,\+E)$ with maximum degree $\Delta$, $\eta \in [0,1)$ is a constant. Let $0<\epsilon=\epsilon_{k,\Delta,\eta}<\frac{1}{9k^5\Delta^2}$ be chosen arbitrarily.  Let $[0,c_{\varepsilon})$ be the segment on the real axis such that
% % \begin{equation}\label{eq:his-ly-condition}
% % \left(\frac{\lambda+\varepsilon}{1+\lambda-\varepsilon}\right)^{k/2}< \eta \frac{1}{2\mathrm{e}\Delta k^2}.
% % \end{equation}
% % for all $\lambda\in [0,c_{\varepsilon})$. Let $\+D_{\varepsilon}$ be the connected region in the complex plane obtained as the union of disks of radius $\varepsilon_{k,\Delta}$ centred at all points on the segment $[0,c_{\varepsilon})$. 

% Fix $k \ge 2$, and $\Delta \ge 3$. For any $0 < \epsilon < \frac{1}{9k^5 \Delta^2}$, a constant $\eta \in [0, 1)$, let $[0, \lambda_{c, \varepsilon})$ be the real segment such that the following holds for all $\lambda \in [0, \lambda_{c, \varepsilon})$:

% \[
% \left(\frac{\lambda+\varepsilon}{1+\lambda-\varepsilon}\right)^{k/2}< \sqrt{\eta} \cdot \frac{1}{2\sqrt{2}\mathrm{e}\Delta k^2}.
% \]

% Define $\+D_{\varepsilon}$ as the connected complex region given by $\+D_{\varepsilon} \defeq \{z \in \=C \mid \exists \lambda \in [0, \lambda_{c, \varepsilon}) \text{s.t.} \abs{z - \lambda} \le \varepsilon \}$,
% which is the union of disks of radius $\varepsilon$ centered at points on the segment $[0,\lambda_{c,\varepsilon})$. 

% Let $\+T_i$ be the set of all bad trees with size $i$. Then, for any $k$-uniform hypergraph $H = (V, \+E)$ with maximum degree $\Delta$, $\lambda'\in \+D_{\varepsilon}$, $\forall S \in V$ and $\abs{S} = k$, it holds that, 

% \[
%     \abs{\mu\left( \sigma_S = 1^{\abs{S}} \right)} < \eta,
% \]

% \[
% \sum\limits_{T \in \+T_i}
% \sum\limits_{\substack{\=T(C) = T \\ \tau_C \in \{0,1\}^C}}
% \abs{\mu^{\-{GD}}_{\infty}(\+T^{\-{bad}}=T, \+C^\-{bad} = C, \sigma_C = \tau_C)} \le \eta \cdot 2^{-i}.
% \]
% \end{lemma}

% We now show that the truncated partition function $Z_\+G^*$ is $\varepsilon$-multiplicative approximation of the partition function $Z_\+G$.

% % \begin{lemma}\label{lemma:approx-partition}
% % Let $\gamma > \left\lceil \log_2 \left( \frac{2 \abs{\+E}}{(1 - \eta)\epsilon} \right) \right\rceil$.
% %     It holds that,
% %     \[
% %     \frac{\abs{Z_\+G - Z_\+G^*}}{\abs{Z_\+G}} \le \varepsilon.
% %     \]
% % \end{lemma}

% % Before proving \Cref{lemma:approx-partition}, we first introduce a few lemmas about the norms and arguments of $\+R_i$ and $\+R_i^*$.

% \begin{lemma}\label{lemma:approx-R-norm-argument}
%     It holds that,
%     \[
%     1 - (1 - \eta) 2^{-\gamma} \le \frac{\abs{\+R_i^*}}{\abs{\+R_i}} \le 1 + \frac{2^{-\gamma}}{1 - \eta}.
%     \]
%     \[
%         \abs{\Arg\left(\+R_i, \+R^*_i\right)} \le \frac{2^{-\gamma}}{1 - \eta} .
%     \]
% \end{lemma}

% \begin{lemma}\label{lemma:approx-lowerbound}
%     It holds that,
%     \[
%         \abs{\+R_i} \ge 1 - \eta,
%     \]
% \end{lemma}

% \begin{proof}[Proof of \Cref{lemma:approx-lowerbound}]
%     By \Cref{lemma:approx-bad-tree-decay}, 
%     \[
%     \abs{\+R_i} \ge 1 - \abs{\mu \left(\sigma_{\ts(e_{i},0)} = 1^{\abs{e_{i}}} \right)} \ge 1 - \eta.
%     \]
% \end{proof}

% \begin{proof}[Proof of \Cref{lemma:approx-R-norm-argument}]
% \begin{align*}
% &\frac{\abs{\+R_i^*}}{\abs{\+R_i}} \\
% \le&
% 1 + \frac{\abs{\+R_i^* - \+R_i}}{\abs{\+R_i}} \\
% \le &
% 1 + \frac{\abs{\+R_i^* - \+R_i}}{1 - \eta}  \\
% (\text{by \Cref{lemma:outcome-correspondence} and \Cref{lemma:approx-bad-tree-decay}}) \quad \le &
% 1 + \frac{2^{-\gamma}}{1 - \eta}.
% \end{align*}

% \begin{align*}
% &\frac{\abs{\+R_i^*}}{\abs{\+R_i}} \\
% \ge&
% 1 - \frac{\abs{\+R_i^* - \+R_i}}{\abs{\+R_i}} \\
% \ge &
% 1 - \frac{\abs{\+R_i^* - \+R_i}}{1 - \eta}  \\
% (\text{by \Cref{lemma:outcome-correspondence} and \Cref{lemma:approx-bad-tree-decay}}) \quad \ge &
% 1 - \frac{2^{-\gamma}}{1 - \eta}.
% \end{align*}
% % \yxtodo{Small bug here.}
% We first give a crude bound of $\abs{\Arg(\+R_i^*, \+R_i)}$. Note $\+R_i^*, \+R_i$ and $\+R_i^* - \+R_i$ form a triangle in the complex plane. We also know that $\abs{R_i} \ge 1 - \eta$ and $\abs{\+R_i - \+R_i^*} \le 2^{-\gamma}$, with $\gamma > \log_2 \left( \frac{2 \abs{\+E}}{(1 - \eta)\varepsilon} \right)$, we know that $\abs{\+R_i} > \abs{\+R_i - \+R_i^*}$ which implies that $\abs{\Arg(\+R_i^*, \+R_i)} < \frac{\pi}{2}$.
% \begin{align*}
% &\abs{\Arg\left(\+R_i^*, \+R_i\right)} \\
% \left( x \le \tan(x) \text{ for } 0 \le x < \frac{\pi}{2} \right)\quad\le&
% \abs{\tan\left( \abs{\Arg\left(\+R_i^*, \+R_i\right)} \right)} \\
% \le &
% \abs{\frac{\abs{\+R_i^* - \+R_i}}{\abs{\+R_i^*}}} \\
% (\text{by \Cref{lemma:outcome-correspondence} and \Cref{lemma:approx-bad-tree-decay}})\quad \le &
% \frac{2^{-\gamma}}{1 - \eta}
% \end{align*}

% \end{proof}

% \begin{proof}[Proof of \Cref{lemma:approx-partition}]
% \begin{align*}
%     \frac{\abs{Z_\+G - Z_\+G^*}}{\abs{Z_\+G}}
%     = &
%     \abs{1 - \prod\limits_{1 \le i \le m}\frac{\+R_i^*}{\+R_i}}.
% \end{align*}

% By \Cref{lemma:approx-R-norm-argument}, we know that 
% \[
% \abs{\prod\limits_{1 \le i \le m}\frac{\+R_i^*}{\+R_i}} \le (1 + 2^{-\gamma}/(1 - \eta))^m \le \exp\left( m 2^{-\gamma}/(1 - \eta) \right) \le \exp(\varepsilon/2),
% \]

% \[
% \abs{\Arg\left( \prod\limits_{1 \le i \le m}\frac{\+R_i^*}{\+R_i} \right)} \le m 2^{-\gamma}/(1 - \eta) \le \varepsilon/2.
% \]

% By the law of cosines, 

% \begin{align*}
% \abs{1 - \prod\limits_{1 \le i \le m}\frac{\+R_i^*}{\+R_i}} 
% \le &
% \sqrt{1 + \exp(\varepsilon) - 2 \exp(\varepsilon/2) \cos(\varepsilon/2) } \\
% \le &
% \varepsilon
% \end{align*}

% \end{proof}

% \begin{lemma}\label{lemma:}
    
% \end{lemma}

Now we can give our algorithm consisting \reveal ~(\Cref{Alg:reveal}), \perco ~(\Cref{Alg:percolation}) and \appmgn ~(\Cref{Alg:approxmarginal}). 
Our algorithm follows the general framework in \cite{feng2023towards}.
We first describe how our algorithm goes. 
For a $k$-uniform hypergraph $H = (V, \+E)$ with maximum degree $\Delta$, let $\varepsilon$ and $\+D_\varepsilon$ be defined as those in \Cref{theorem:zero-freeness-his-lee-yang}.
Let $\*\lambda \in \+D_\varepsilon^V$ and $\mu$ be its stationary measure.

Our algorithm simulates \Cref{Alg:complex-GD-decomposed-his} from $t=0$ backwardly. Let $S = e \in \+E$, it enumerates all possible bad components within size $\gamma \Delta(G_H^S)$ then calculates their contributions to $\mu(\sigma(e)=1^{e})$. Recall in \Cref{Alg:complex-GD-decomposed-his}, every timestamp $t$ associates with $r_t$ and $c_t$.

Now we introduce these three parts of our algorithm.
We first introduce \reveal~(\Cref{Alg:reveal}). It inputs a timestamp $t$, then generate $r_t$ by a global variable $\*r$ which we will introduce later.
It also computes the contribution of $r_t$'s.
Then we introduce \perco~(\Cref{Alg:percolation}). It inputs a timestamp $t$, then determines the $c_t$ recursively.
\appmgn~ inputs a hypergraph and an edge $e$, approximate the marginal measure of $\mu(\sigma(e)=1^e)$.
\appmgn~ begins by enumerating possible sequences $\*r = (r_i)_{i=1}^{m}$, where $m = \gamma k \Delta(G_H^S)$. Then, it calls \reveal~(\Cref{Alg:reveal}) to get the $r_t$'s in $\ts(e, 0)$, where $r_t$'s are determined by the generated $\*r$. After that, if one can not determine if configurations in $e$ are $1'$s or not. It then calls \perco~ (\Cref{Alg:percolation}) to recursively determine the configuration of each $v\in \ts(e, 0)$. 


% $\*r$ serves as ``random bits''. inputs a time $t$ outputs the configuration on time $t$ by information percolation. And \Cref{Alg:reveal} inputs a time $t$ and reveals its $r$ and counts the contribution of it into $\mathrm{mass}$.

% Specifically we run  \Cref{Alg:approxmarginal} with initialization $e = e_i$ and $\gamma = \left\lceil \log_2  \frac{4 m}{(1 - \eta)\epsilon} \right\rceil$.

% \begin{algorithm} \label{algorithm:margional-approximation}
% %\caption{$\resolve_{\mu, X_{-T}, T}(t; M,R)$} \label{Alg:resolve}
% \caption{$\text{ApproxMarginal}(S,M,R,r;\text{ANS},e^*)$} \label{Alg:resolve}
%   \SetKwInput{KwPar}{Parameter}
%   \SetKwInput{KwData}{Global variables}
%  \KwIn{a subset $S$, a map $M: \mathbb{Z}\to [2] \cup \{\bot\}$ and a set $R$;}
% \KwData{global answer summation $\text{ANS}$, current answer $r$, initial edge $e$;}
% \If{$|S| = 0$}{
%     \While{$|R| \neq 0$}{ \label{algorithm:approxmarginal-backward-detect}
%         Let $t \in \{t | t \in R, \forall e, v(t) \in e, \ts(e, t) \subseteq \text{dom}(M)\}$;  \label{algorithm:approxmarginal-t} \\
%         \lIf{$\exists e, v(t)\in e, \exists t', v(t')\in e, t' \in \ts(e, t), M(t') = 0$}{$M(t)\gets 1$} 
%         \lElse{$M(t) \gets 0$} 
%         $R \gets R - \{t\}$;
%     }
%     \If{$\forall v \in e^*, M(\ts(v,0)) = 1$}{
%         $\text{ANS} \gets \text{ANS} + r$;
%     }
%     \Return
% }
% \If{$|S| + |M| + |R| > \gamma$}{
% \Return
% }
% \For{ $\sigma \in  \{0,\bot\}^{S \backslash (M \cup R)}$ }{
% $M' \gets M \cup \{(t, 0) | \sigma_t = 0\}$; \\
% $R' \gets R \cup \{t | \sigma_t = \bot\}$;\\
% $T' \gets \{v | v \in N(S), \}$
% $S' \gets \{ N(v) | \sigma_v = \bot \} \backslash (\text{dom}(M) \cup R)$; \\
% $r' \gets r \cdot \left(\frac{1}{1 + \lambda}\right)^{\abs{\{t|\sigma_t = 0\}}}\left(\frac{\lambda}{1 + \lambda}\right)^{\abs{\{t|\sigma_t = \bot\}}}$; \\
% % $D \gets \{v | v \in R', N(v) \subseteq \text{ dom}(M) \}$;
% ApproxMarginal($S', M', R',r';\text{ANS},e$); \label{algorithm:approxmarginal-recursion}
% }
% \end{algorithm}

\begin{algorithm}
%\caption{$\resolve_{\mu, X_{-T}, T}(t; M,R)$} \label{Alg:resolve}
\caption{$\text{Reveal}(t; b, \text{mass},M, \*r, \text{cnt})$} \label{Alg:reveal}
  \SetKwInput{KwPar}{Parameter}
  \SetKwInput{KwData}{Global variables}
 \KwIn{a timestamp $t$, a hypergraph $H=(V,\+E)$;}
\KwData{a map $M: \mathbb{Z}\to \{0,1,\bot\}$, measure of bad component: mass, sequence: $\*r$, number of used bits: $\text{cnt}$;}
\lIf{$t \in M$}{\Return $M(t)$}
$M(t) = \vec{r}_{\text{cnt}};$\\
$\text{cnt} \gets \text{cnt} + 1;$ \\
\lIf{$M(t)=0$}{$\text{mass} \gets \text{mass} \cdot \frac{1}{1 + \lambda_{v_{i(t)}}}$}
\lElse{$\text{mass} \gets \text{mass} \cdot \frac{\lambda_{v_{i(t)}}}{1 + \lambda_{v_{i(t)}}}$}
\Return $M(t)$
\end{algorithm}

\begin{algorithm} 
%\caption{$\resolve_{\mu, X_{-T}, T}(t; M,R)$} \label{Alg:resolve}
\caption{$\text{Percolation}(t;b, \text{mass},M, \*r, \text{cnt})$} \label{Alg:percolation}
  \SetKwInput{KwPar}{Parameter}
  \SetKwInput{KwData}{Global variables}
 \KwIn{a timestamp $t$, a hypergraph $H=(V,\+E)$;}
\KwData{bad component size: $b$,a map $M: \mathbb{Z}\to \{0,1,\bot\}$, measure of bad component: mass, sequence: $\*r$, number of used bits: $\text{cnt}$;}
\lIf{$M(t)=0$}{\Return}
\For{$e \in v_{i(t)}$}{
    \For{$ t' \in \ts(e, t)$ }{
        Reveal($t'$);
    }
    \lIf{$\exists t' \in \ts(e, t) \text{ s.t. } M(t') = 0$}{\textbf{Break}}
    \Else{
        $b \gets b + 1$; \\
        \lIf{$b > \gamma$}{$\text{mass} \gets 0$; \Return}
        \lFor{$t' \in \ts(e, t)$}{Reveal($t'$)}
    }
}
\lIf{$\forall e , v_{i(t)} \in e, \exists t' \in \ts(e, t), M(t')=0$}{$M(t)\gets 1$}
\lElse{$M(t) \gets 0$}
\end{algorithm}

\begin{algorithm} 
%\caption{$\resolve_{\mu, X_{-T}, T}(t; M,R)$} \label{Alg:resolve}
\caption{$\text{ApproxMarginal}(e, H; b, \text{mass},M, \*r, \text{cnt})$}
\label{Alg:approxmarginal}
  \SetKwInput{KwPar}{Parameter}
  \SetKwInput{KwData}{Global variables}
 \KwIn{an edge $e\in\+E$, a hypergraph $H=(V,\+E)$}
\KwData{bad component size: $b$, a map $M: \mathbb{Z}\to \{0,1,\bot\}$, measure of bad component: mass, sequence: $\*r$, number of used bits: $\text{cnt}$;}
\KwOut{a complex number $\+R$;}
$\+R \gets 0$; \\
\For{$\*r \in \{0, \bot\}^{\gamma k \Delta(G_H^e)}$}{
    $M \gets \emptyset$;\\
    $b \gets 0, \text{mass} \gets 0, \text{cnt} \gets 0$;\\
    \lFor{$t \in \ts(e, 0)$}{Reveal($t$)}
    \lIf{$\exists t \in \ts(e, 0) \text{ s.t. } M(t) = 0$}{\textbf{Break}}
    \lFor{$t \in \ts(e, 0)$}{Percolation($t$)}
    \lIf{$\exists t \in \ts(e, 0) \text{ s.t. } M(t) \neq 1$}{\textbf{Break}}
    $\+R \gets \+R + \text{mass}$;
}
\Return $\+R$;
\end{algorithm}

Recall the definition of $\+R_i^*$ for each $0 \le i < m$,  we now prove the following theorem,
% Specifically we run  \Cref{Alg:approxmarginal} with initialization $e = e_i$ and $\gamma = \left\lceil \log_2  \frac{4 m}{(1 - \eta)\epsilon} \right\rceil$.
\begin{lemma}
% For a $k$-uniform hypergraph $H=(V, \+E)$ with maximum degree $\Delta$, let $\varepsilon$ and $\+D_\varepsilon$ be as defined in \Cref{theorem:approx-his}. Let $\*\lambda \in \+D_\varepsilon^V$ and $\mu$ be its stationary measure. 
Suppose the conditions in \Cref{theorem:approx-his}. 
% Fix an arbitrary ordering of hyperedges $\+E = \{e_1, e_2, \ldots, e_m\}$. For each $0 \le i \le m$, let $\+E_i = \{e_1, e_2, \ldots, e_i\}$ and $H_i = (V, \+E_i)$.
\appmgn$(e, H_i)$ outputs $\+R^*_i$ with the time complexity $O\left((2\gamma \Delta^2 k^5) \cdot 2^{2\gamma \Delta^2 k^5 }\right)$.
\end{lemma}

\begin{proof} 
% For a $k$
Let $S = e \in \+E$, and consider the witness graph $G_H^S$ (\Cref{definition:witness-graph-indset}).
The correctness is due to that we enumerate all possible bad components with in size $\gamma$ by running \appmgn~(\Cref{Alg:approxmarginal}). Note by \Cref{Alg:complex-GD-decomposed-his} and \Cref{definition:witness-graph-indset}, it holds that we only need to enumerate a sequence $\*r = \{0, \perp\}^{\gamma k \Delta(G_H^S)}$ to enumerate all possible bad components within size $\gamma$. The time complexity is due to the enumeration of $\*r$ and the steps to determine the configuration in $e_i$.
% In \Cref{Alg:approxpartition}, we reveal at most $\gamma k (\Delta(G_H^S))$
% In \Cref{Alg:approxpartition}, we enumerate 
% Because we enumerate all bad components and their neighbors at most size $\gamma$, we only reveal at most $\gamma k \left(\Delta\left(G_e^H\right) + 1\right)$ timestamps of $\vec{r}$.
% And the approximation ratio directly follows from \Cref{lemma:approx-partition}.

    
\end{proof}
Now we are ready to prove \Cref{theorem:approx-his}.
\begin{proof}
    Fix an arbitrary ordering of hyperedges $\+E = \{e_1, e_2, \ldots, e_m\}$. For each $0 \le i \le m$, let $\+E_i = \{e_1, e_2, \ldots, e_i\}$ and $H_i = (V, \+E_i)$. $Z_{H_0}^\-{ly}(\*\lambda)$ is easy to compute. For each $0\le i <m$, we call \appmgn$(e_i, H_i)$ to compute $\+R^*_{i}$. After that we compute $Z_{H}^{\-{ly},*}(\*\lambda)$. Then by \Cref{lemma:approx-partition}, it holds that $Z_H^{\-{ly},*}(\*\lambda)$ is a $\varepsilon$ multiplicative approximation of $Z_H^\-{ly}(\*\lambda)$.
\end{proof}
    % We first prove that this algorithm terminates. 

    % With the increasing depth of the recursion at \Cref{algorithm:approxmarginal-recursion}, the size of $\abs{S} + \abs{R} + \abs{M}$ is strictly increasing when $\abs{S} \neq 0$. With the bound $\gamma$, the recursion depth is up-bounded by $\gamma$. When $\abs{S} = 0$, it will start the while loop at \Cref{algorithm:approxmarginal-backward-detect}. So it suffices to prove the while loop at \Cref{algorithm:approxmarginal-backward-detect} terminates. We first provide some observations,
    % \begin{observation}\label{observation:approximarginal-R-S}
    % It holds that,
    % \begin{itemize}
    %     \item  $R$ contains all time tags $t$ with $r_t = \bot$;
    %     % \item For all time tags $t \in R$, for all edges $e$ containing $v(t)$, if for time tag $t' \in \ts(e, t)$, $r_{t'}$ is not decide yet, then $t' \in S$.
    %     \item For all time tags $t \in R$, for all its neighbors $t'$ with $t' > t$, $t'$ must belong to one of the three sets $\text{dom}(M)$, $R$, $S$.
    % \end{itemize}
    % \end{observation}
    % \begin{lemma}
    %     The while loop at \Cref{algorithm:approxmarginal-backward-detect} terminates.
    % \end{lemma}
    % \begin{proof}
    %     If $|R| = 0$, this loop terminates. For $|R| \neq 0$, we provide a procedure to find the $t$ at \Cref{algorithm:approxmarginal-t}. Pick an arbitrary time tag $t \in R$.  
    %     If all its neighbors with greater time tags are in $\text{dom}(M)$, then we choose $t$, otherwise there must be one time tag $t'$ belonging to $R$ by \Cref{observation:approximarginal-R-S}. Then check $t'$ again until this procedure ends. 
    %     This procedure terminates because of the finite size of $R$.
    % \end{proof}
    
    % Then we show the time complexity of this algorithm.

    % The algorithm enumerate all connected components containing $\ts(e^*, 0)$ within size $(1 + \Delta(G_H^{e^*}))\gamma$. We introduce the following bound of the number of connected components.

    % \begin{lemma}[Lemma 2.1 of \cite{borgs2013left}]
    %     Let $G$ be a graph with maximum degree $\Delta$, let $v \in V(G)$, the number of vertex induced connected subgraphs with $k$ vertices containing $v$ is at most $\frac{(e \Delta)^{k-1}}{2}$.
    % \end{lemma}

    % The algorithm enumerates all possible bad components and the possible configurations in their neighbors. There are at most,

    % \[
    % \sum\limits_{i \le \gamma} 2^{\Delta i} 2^{\Delta^2 i} \le 2^{2 \Delta^2 (\gamma+1) }.
    % \]
    % possible cases.

    % With some subtle data structures, the time complexity of the algorithm is $O\left( 2^{2 \Delta^2 (\gamma+1)} \right)$.



% This also implies \Cref{theorem:approx-his}. Finally, we prove the bad tree decay \Cref{lemma:approx-bad-tree-decay}.
% \begin{proof}[Proof of \Cref{lemma:approx-bad-tree-decay}]
% Recall the proof of \Cref{lemma:his-lee-yang-marginal}, it suffices to show that 

% % \[
% % \sum\limits_{T \in \+T_i}
% % \sum\limits_{\substack{\=T(C) = T \\ \tau_C \in \{0,1\}^C}}
% % \abs{\mu^{\-{GD}}_{\infty}(\+T^{\-{bad}}=T, \+C^\-{bad} = C, \sigma_C = \tau_C)} \le \eta \cdot 2^{-i}.
% % \]
% \[
% \sum_{\substack{\=T(C) = T \\ \tau_C \in \{0,1\}^C}} \left| \mu^\-{GD}_\infty\left(\+T^\-{bad}=T,\+C^\-{bad}= C,\sigma_C = \tau_C\right) \right| 
% \le \eta \left( 4\mathrm{e} \Delta^2 k^4 \right)^{-\abs{T}}.
% \]
% %    Recall the deterministic process in \Cref{definition:2-tree-construction} for the construction of the $2$ tree $\+T^{\-{bad}}$ from $\+C^{\-{bad}}$. Note that for the event $\+T^{\-{bad}}=T$ to occur, $\+C^{\-{bad}}$ must only contain vertices in $G_H^S$ that are within distance $1$ of $T$, and it is sufficient to check for all vertices in $G_H^S$ that are within distance $2$ of $T$ whether they are in $V^{\-{bad }}$ or not. Therefore, to  the event $\+T^{\-{bad}}=T$  can be translated to the following:
% %    \begin{enumerate}
% %        \item for each $e\in T$, we have $r_t=\bot$ for all $t\in e$;\label{item:modulus-bound-1}
% %        \item the $r_t$s on all other vertices in $G^H_S$ that is within distance $2$ of $T$ satisfy certain restrictions so that $\+T^{\-{bad}}=T$.\label{item:modulus-bound-2}
% %    \end{enumerate}

% % Note that the event $\+T^{\-{bad}}=T$ is determined only by $\{r_t\}_{t=-\infty}^{0}$, and $\{r_t\}_{t=-\infty}^{0}$ follows a product measure. Therefore, the \Cref{item:modulus-bound-1} contributes a factor of $\abs{\frac{\lambda}{1+\lambda}}^{k|T|}$ by the definition of $2$-trees that all vertices in $T$ contain disjoint timestamps. We can use a simple triangle inequality to bound \Cref{item:modulus-bound-2}. Since there are at most $|T|\Delta(G^S_H)^2$ vertices and therefore $k|T|\Delta(G^S_H)^2$ timestamps included, this contributes a factor of at most $\left(\abs{\frac{\lambda}{1+\lambda}}+\abs{\frac{1}{1+\lambda}}\right)^{k|T|\Delta(G^S_H)^2}$, where $\Delta(G^S_H)$ is the maximum degree of $G^S_H$.

% % Overall, we have

% % Follow the proof of \Cref{lemma:modulus-bound},

% By \Cref{lemma:his-lee-yang-bad-tree-decay}, it holds that

%     \[
%     \sum_{\substack{\=T(C) = T \\ \tau_C \in \{0,1\}^C}} \left| \mu^\-{GD}_\infty\left(\+T^\-{bad}=T,\+C^\-{bad}= C,\sigma_C = \tau_C\right) \right| 
% \le \left( \ell^\-{pad} \right)^{\abs{T}} \ell^{k \Delta(G_H^S)^2 \abs{T}}.
%     \]

%     \begin{align*}
%         &\left( \ell^\-{pad} \right)^{\abs{T}} \ell^{k \Delta(G_H^S)^2 \abs{T}}  \\
%         (\text{by \Cref{lemma:witness-graph-degree-bound}})\quad\leq &\left( \ell^\-{pad} \right)^{|T|}\cdot \ell^{4 \Delta^2k^5 |T|}\\
% (\text{by conditions in \Cref{lemma:approx-bad-tree-decay} and \Cref{lemma:his-lee-yang-bad-tree-decay}})\quad \leq & \eta \left(2\mathrm{e}\Delta k^2\right)^{-2|T|}\cdot \mathrm{e}^{|T|}\\
% \le& \eta \left(4 \mathrm{e} \Delta^2 k^4\right)^{-\abs{T}}
%     \end{align*}

% % \begin{align*}
% % &\sum\limits_{\substack{\=T(C) = T}}
% % \abs{\mu^{\-{GD}}_{\infty}(\+T^{\-{bad}}=T, \+C^\-{bad} = C)}\\
% % \leq &\abs{\frac{\lambda}{1+\lambda}}^{k|T|}\cdot \left(\abs{\frac{\lambda}{1+\lambda}}+\abs{\frac{1}{1+\lambda}}\right)^{k|T|\Delta(G^S_H)^2}\\
% % (\text{by \Cref{lemma:witness-graph-degree-bound}})\quad\leq &\left(\abs{\frac{\lambda}{1+\lambda}}^{k|T|}\cdot \left(\abs{\frac{\lambda}{1+\lambda}}+\abs{\frac{1}{1+\lambda}}\right)^{4|T|\Delta^2k^5}\right)\\
% % \leq & \left(\frac{\`R(\lambda)+\varepsilon}{1+\`R(\lambda)-\varepsilon}\right)^{k|T|}\cdot \left(\frac{1+\varepsilon}{1-\varepsilon}\right)^{4|T|\Delta^2k^5}\\
% % \leq &\eta \cdot \left(2\mathrm{e}\Delta k^2\right)^{-2|T|}\cdot \mathrm{e}^{|T|}\\
% % =&\eta \cdot \left(4\mathrm{e}\Delta^2 k^4\right)^{-|T|}.
% % \end{align*}

% % So it holds that

% % \[
% % \sum\limits_{T \in \+T_i}
% % \sum\limits_{\substack{\=T(C) = T}}
% % \abs{\mu^{\-{GD}}_{\infty}(\+T^{\-{bad}}=T, \+C^\-{bad} = C)} \le \eta \cdot 2^{-i},
% % \]

% % which implies that
% % \[
% %     \abs{\mu\left( \sigma_S = 1^{\abs{S}} \right)} < \eta,
% % \]



% % finishing the proof of the lemma.
% \end{proof}

% \begin{tikzpicture}[node distance=2cm, auto, thick]
%     % Define custom arrow style
%     \tikzset{>={Latex[width=3mm,length=3mm]}}

%     % Define nodes with smaller size and larger font
%     \node (zero) [draw, rounded corners, minimum width=2.5cm, minimum height=0.8cm, font=\large] {zero-freeness};
%     \node (mixing) [below left=1.5cm and 1.5cm of zero, draw, rounded corners, minimum width=2.5cm, minimum height=0.8cm, font=\large] {rapid mixing};
%     \node (decay) [below right=1.5cm and 1.5cm of zero, draw, rounded corners, minimum width=2.5cm, minimum height=0.8cm, font=\large] {decay of correlations};

%     % Draw arrows with labels and larger font
%     \draw[->] (zero) -- (mixing) node[midway, above, font=\large] {\cite{Alimohammadi2021FractionallyLA,Chen2021SpectralIV}};
%     \draw[->] (zero) -- (decay) node[midway, above, font=\large] {\cite{regts2023absence}};
%     \draw[->] (decay) -- (zero) node[midway, above, font=\large] {\cite{liu2019correlation,Shao2019ContractionAU}};
%     \draw[->, xshift=2cm] (decay) -- (mixing) node[midway, above, font=\large] {\cite{anari2020spectral, chen2021optimal}};


% \end{tikzpicture}
% \begin{figure}[H]
%     \centering
%     % \includegraphics[width=0.5\linewidth]{}
%     \begin{tikzpicture}[node distance=2cm, thick][shift={(10,10)}]
%         \tikzset{>={Latex[width=3mm,length=3mm]}}
%           \node (zero) [draw, rounded corners, minimum width=2.5cm, minimum height=0.8cm, font=\large] {zero-freeness};
%           \node (mixing) [draw, rectangle, below left=of zero, rounded corners, minimum width=2.5cm, minimum height=0.8cm, font=\large] {rapid mixing};
%           \node (decay) [draw, rectangle, below right=of zero, rounded corners, minimum width=2.5cm, minimum height=0.8cm, font=\large] {decay of correlations};
        
%           \draw[->] (zero) to[bend left=10] node[above, xshift=0.5cm] {\cite{regts2023absence}} (decay);
%           \draw[->] (decay) to[bend left=10] node[below, xshift=-1cm] {\cite{liu2019correlation,Shao2019ContractionAU}} (zero);
%           \draw[->] (mixing) -- node[below] {\cite{anari2020spectral, chen2021optimal}} (decay);
%           \draw[->] (zero) -- node[above, xshift=-1.4cm] {\cite{Alimohammadi2021FractionallyLA,Chen2021SpectralIV}} (mixing);
%     \end{tikzpicture}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}


==> fisher.tex <==

In this subsection, we prove the zero-freeness result on fisher zeroes following the framework defined in \Cref{subsection:framework-marginal-ratio}. The independence polynomial of the hypergraph $H$ on fisher zeroes is defined as

\[
Z^\-{fs}_H(\*\beta) = \sum_{\sigma \in \{0,1\}^V} \prod_{\sigma_e=1^k} \beta_e,
\]

with the associated measure $\mu_{\*\beta} = \mu_{\*\beta,H} : \{0,1\}^V \to \={C}$ defined as

\[
\forall \sigma \in \{0,1\}^V, \quad \mu_{\*\beta}(\sigma) = \frac{\prod_{\forall v \in e, \sigma_v = 1}\beta_e}{Z^\-{fs}_H(\*\beta)},
\]

when $Z^\-{fs}_H(\*\beta) \neq 0$. For the brevity of notation, we will regard $\mu$ as $\mu_{\*\beta}$ in this subsection. Given $v$ and $\sigma_{V \backslash \{v\}}$, let $\tilde{E} = \{e \mid \forall u, v \in e, u \neq v, \sigma_u = 1\}$.



\[
\mu_v^{\sigma(V \backslash \{v\})}(0) = \frac{1}{1 + \prod_{e \in \tilde{E}} \beta_e}, \quad \mu_v^{\sigma(V \backslash \{v\})}(1) = \frac{\prod_{e \in \tilde{E}} \beta_e}{1 + \prod_{e \in \tilde{E}} \beta_e}.
\]

The marginal measure $\mu_v^{\sigma(V \backslash \{v\})}$ is also well-defined by the next lemma which we defer the proof to the end of this section. 
% when $\forall 0 \le i \le \Delta, \beta^{i} \neq -1$ for any $\sigma \in \{0,1\}^V$ and $v$ where $\Delta$ is the maximum degree of the graph $H$.

\begin{lemma}\label{lemma:his-fisher-well-define-transition}
    Suppose that the conditions in \Cref{theorem:zero-freeness-his-lee-yang}, for any $v$ and $\sigma_{V \backslash \{v\}}$, the marginal measure $\mu_v^{\sigma(V \backslash \{v\})}$ is well defined.
\end{lemma}

Again we utilize the edge-wise self-reducibility and it suffices to prove the following lemma.

\begin{lemma}\label{lemma:his-fisher-marginal}
Let $H(V, \+E)$ be a $k$-uniform hypergraph with maximum degree $\Delta$, let $\varepsilon = \varepsilon_{k, \Delta}$ and $\+D_\varepsilon$ be as defined in \Cref{theorem:zero-freeness-his-fisher}. Suppose that $Z^\-{fs}_H(\*\beta) \neq 0$ and therefore $\mu_{\*\beta}$ is well-defined. For any $S \subseteq V$, $|S|=k$ and $\*\beta \in \+D_\varepsilon^V$, it holds that
\[
(1 - \beta)\mu\left(\sigma(S) = 1^{|S|}\right) \neq 1.
\]
\end{lemma}

Like \Cref{lemma:his-lee-yang-marginal}, it suffices to prove \Cref{lemma:his-fisher-marginal} to prove \Cref{theorem:zero-freeness-his-fisher}.

\begin{proof}[Proof of \Cref{theorem:zero-freeness-his-fisher}]
    Let $\+E = \{e_1, e_2, \dots, e_m\}$. For $0 \le i \le m$ we let $\+E_i = \{e_1, e_2, \dots, e_i\}$ and let $H_i = (V, \+E_i)$. We prove by induction that $Z_{H_i}^\-{fs}(\*\beta) \neq 0$ for each $0 \le i \le m$.

    The base case is when $i = 0$, and we have $Z_{H_0}^\-{fs} = 2^{\abs{V}}$.

    For the induction step, we fix $0 \le i < m$ and assume that $Z_{H_i}^\-{fs} \neq 0$. Then the measure $\mu_{H_i}$ is well-defined. Note that

    \[
    \frac{Z_{H_{i+1}}^\-{fs}(\*\beta)}{Z_{H_i}^\-{fs}(\*\beta)}=\frac{Z_{H_i}^\-{fs}(\*\beta) - (1 - \beta_{e_{i+1}})\sum\limits_{\substack{\sigma \in \{0,1\}^{V} \\ \sigma(e_{i+1}) = 1^{k}}} \prod_{\forall v \in e, \sigma(v)=1}\beta_e  }{Z_{H_i}^\-{fs}(\*\beta)} = 1 - (1 - \beta_{e_{i+1}})\mu_{H_i}\left(\sigma(e_{i+1}) = 1^k \right) \neq 0,
    \]
    % \yxtodo{Here is a small error to fix: the wrong telescoping.}
    where the last inequality is by \Cref{lemma:his-fisher-marginal}. Therefore $Z_{H_i}^\-{fs} \neq 0$, completing the induction step and the proof of the lemma.
\end{proof}

% Note that according to the above definition, when $\forall 0 \le i \le \Delta, \beta^{i} \neq -1$, the marginal probability $\mu_v^{\sigma_{V \backslash v}}$ is always well-defined for any $\sigma \{0,1\}^V$ and $v \in V$.

We set the lower bound measures for any $v \in V$ (\Cref{definition:marginal-lower-bounds}) as follows for hypergraph independent sets:


% Wait
% \[
% \mu^{\text{LB}}(0) = \frac{1}{1 + |\beta|^\Delta}, \quad \mu^{\text{LB}}(1) = 0, \quad \mu^{\text{LB}}(\perp) = \frac{|\beta|^\Delta}{1 + |\beta|^\Delta}.
% \]

% For $|\beta| < 1$, we set 

\[
\mu^{\text{LB}}(0) = \frac{1}{2}, \quad \mu^{\text{LB}}(1) = 0, \quad \mu^{\text{LB}}(\perp) = \frac{1}{2}.
\]

We then set $\ell^\-{pad}$ and $\ell$, so that $\mu$ is $(\ell^\-{pad}, \ell)$-marginally lower bounded (\Cref{definition:marginal-lower-bounds}).

Let 
\[\ell^{\-{pad}} = \max\limits_{v, \sigma_{V \backslash v}}\left(\abs{ \mu^\-{LB}(\perp) \mu_{V}^{\-{pad},\sigma_{V \backslash v}}(0)} + \abs{\mu^\-{LB}(\perp)\mu_{V}^{\-{pad},\sigma_{V \backslash v}}(1)}\right),\]

\[
\ell = \mu^\-{LB}(0) + \ell^\-{pad}.
\]
We also need the following lemmas and we delay all proofs of them to the end of this subsection.


\begin{lemma}\label{lemma:his-fisher-l1norm-pad}

    Let $\varepsilon = \varepsilon_{k, \Delta}$ and $\+D_\varepsilon$ as defined in \Cref{theorem:zero-freeness-his-fisher} $\*\beta \in \+D_\varepsilon^V$, it holds that

    % \[
    % \ell^\-{pad}
    % \le \frac{1}{2} + \max \left(\frac{1 + 200 \pi \Delta \sqrt{\varepsilon}}{1 - 200 \pi \Delta \sqrt{\varepsilon}},  \frac{8(1 + \varepsilon)^{2\Delta} \varepsilon}{625 \pi} \right)
    % \]
    \[
    \ell^\-{pad}
    % \le \frac{1}{2} + 800 \Delta \pi \sqrt{\varepsilon}.
    \le \frac{1}{2} + 32 \mathrm{e} \Delta \sqrt{\varepsilon}, \quad \ell \le  1  + 32 \mathrm{e} \Delta \sqrt{\varepsilon}
    \]    
    
\end{lemma}

% \begin{corollary} \label{corollary:his-fisher-l1norm}

% Let $\varepsilon = \varepsilon_{k, \Delta}$ and $\+D_\varepsilon$ as defined in \Cref{theorem:zero-freeness-his-fisher} $\beta \in \+D_\varepsilon$, it holds that

%     \[
%     \ell \le  1  + 8 \mathrm{e} \Delta \sqrt{\varepsilon}
%     \]
% \end{corollary}

Recall the witness graph (\Cref{definition:witness-graph-indset}), by \Cref{lemma:framework-marginal-lower-bound-to-bad-tree-decay}, we can prove the next lemma. We defer the proof of it to the end of this section.

\begin{lemma}[Decay of bad tree]\label{lemma:his-fisher-bad-tree-decay}
    Suppose the conditions of \Cref{lemma:his-fisher-marginal}.
    Let $T$ be any finite non-empty $2$-tree of $G_H^S$ containing $\ts(S, 0)$. Then
    \[
    \sum_{\substack{C: \=T(C) = T \\ \tau \in \{0,1\}^C}} \left| \mu^\-{GD}_\infty\left(\+T^\-{bad}=T,\+C^\-{bad}= C,\sigma(C) = \tau\right) \right| \le
    % \left(\mu^\-{LB}(\perp)\right)^{k|T|} \left( \ell^\-{pad}\right)^{k |T| \Delta(G_H^S)^2}
    \left( \ell^\-{pad} \right)^{k \abs{T}} \ell^{k  \Delta(G_H^S)^2 \abs{T}} \le \frac{1}{1+\varepsilon}\left( 4 \mathrm{e} \Delta^2 k^4 \right)^{-\abs{T}}.
    \]
\end{lemma}

% \begin{lemma}\label{lemma:his-fisher-tree-pinning-bound}
%     Suppose the conditions of \Cref{lemma:his-fisher-marginal}. Let $T$ be any finite non-empty $2$-tree of $G_H^S$ containing $\ts(S,0)$. Then 
%     \[\sum_{\tau_T \in \{0,1\}^T} \abs{\mu^\-{GD}_\infty(\+T^\-{bad}=T, \sigma_{T}=\tau_{T}) } \le  \left(\ell^\-{pad}\right)^{k |T|} \ell^{k |T| \Delta(G_H^S)^2}. \]
% \end{lemma}

% \begin{corollary}\label{corollary:his-fisher-modulus-bound}
%     Suppose the conditions of \Cref{lemma:his-fisher-marginal}. Let $T$ be any finite non-empty $2$-tree of $G_H^S$ containing $\ts(S,0)$. Then
%     \[\abs{\mu^\-{GD}_\infty\left(\+T^\-{bad}=T \right) } \le  \left( \ell^\-{pad} \right)^{k \abs{T}}  \ell^{k  \Delta(G_H^S)^2 \abs{T}} \le \frac{1}{1+\varepsilon}\left( 4 \mathrm{e} \Delta^2 k^4 \right)^{-\abs{T}}.\]
% \end{corollary}

% \begin{proof}
%     Triangle inequality and \Cref{lemma:his-fisher-component-pinning-bound} imply this corollary.   
% \end{proof}

% \begin{lemma}\label{lemma:his-fisher-component-pinning-bound]}
%     Suppose the conditions of \Cref{lemma:his-fisher-marginal}. Let $T$ be any finite non-empty $2$-tree of $G^H_S$ containing $\ts(S,0)$ and $\tau_T$ be the pinning on $T$. Then
%     \[\sum_{\substack{\=T^\-{bad}(C) = T \\ \tau_{C \backslash T} \in \{0,1\}^{C \backslash T}}}\abs{\mu^{\-{GD}}_{\infty}(\+C^{\-{bad}}=C, \sigma_{C\backslash T}=\tau_{C\backslash T} \mid \+T^\-{bad}=T, \sigma_{T}=\tau_{T})} \le \ell^{k \Delta(G_H^S)^2|T|}. \]
% \end{lemma}

\begin{comment}

\begin{corollary}\label{corollary:his-fisher-component-bound}
    Suppose the conditions of \Cref{lemma:his-fisher-marginal}. Then given bad tree $T$ and the pinning on bad tree $\tau_T$ it holds,
    \[\sum_{\substack{T(C) = T \\ \tau_{C \backslash T} \in \{0,1\}^{C \backslash T}}}\abs{\mu^{\-{GD}}_{T}(\+C^{\-{bad}}=C, \sigma_{C\backslash T}=\tau_{C\backslash T} \mid \+T^\-{bad}=T, \sigma_{T}=\tau_{T})} \le \ell^{k \Delta(G_H^S)^2|T|} \]
\end{corollary}
    
\end{comment}

We then check the zero-one law of the outcome (\Cref{definition:framework-zero-one-law-outcome}) showing that the outcome of the event $\sigma_0(S) = 1^{\abs{S}}$ can be solely determined by the configuration on the bad component.

\begin{lemma}[Zero-one law of the outcome]\label{lemma:his-fisher-outcome-correspondence}
Let $S'\subseteq V^{S}_{H}$ be a finite subset of vertices in $G^S_H$  and configuration $\tau \in \{0,1\}^{S'}$ on it such that $\mu^{\-{GD}}_{\infty}\left(\+C^{\-{bad}}=S', \sigma(S') = \tau\right)\neq 0$. Then, for arbitrary $\tau \in \{0,1\}^{S'}$ it holds that
\[
\mu^{\-{GD}}_{\infty}\left(\sigma(\ts(S,0)) =  1^{|S|}\mid \+C^{\-{bad}}=S', \sigma(S') = \tau\right) = 0 \text{ or }1.
\]
\end{lemma}

\begin{proof}
If $\ts(S, 0) \in C^{\-{bad}} = S'$ and $\sigma(\ts(S,0))$ = $\tau(\ts(S,0))$. Otherwise, it holds that $\sigma(\ts(S,0)) \neq 1^{\abs{S}}$ due to the setting of the lower bound measure.
\end{proof}





We also check the finiteness of bad trees (\Cref{definition:framework-finiteness-bad-trees}) so that we do not need to consider the case that $\+C^\-{bad}$ and $\+T^\-{bad}$ are infinite.

\begin{lemma}[Finiteness of bad trees]\label{lemma:his-fisher-finite-component}
Suppose the conditions of \Cref{lemma:his-fisher-marginal}. Then
\[
\mu^{\-{GD}}_{\infty}(\+T^{\-{bad}}\text{ is infinite})=0.
\]
\end{lemma}

% To prove this lemma, we prove the following stronger lemma which implies \Cref{lemma:his-fisher-finite-component}.

\begin{comment}

\begin{lemma}\label{lemma:his-fisher-modulus-bound}
Suppose the conditions of \Cref{lemma:his-fisher-marginal}. Let $T$ be any finite non-empty $2$-tree of $G^H_S$ containing $\ts(S,0)$. Then
\begin{equation}\label{eq:his-fisher-tree-modulus-bound}
    \mu^{\-{GD}}_\infty(\+T^\-{bad} = T) \le \left( 4 e \Delta^2 k^4 \right)^{-|T|}.
\end{equation}
\end{lemma}
\end{comment}
% \begin{equation}\label{eq:2-tree-modulus-bound}
% \sum_{\substack{C \in \=C_i \\ \sigma \in \{0,1\}^C}}
% \abs{\mu^{\-{GD}}_{\infty}(\+C^{\-{bad}}=C, \sigma_C = \sigma)} < \left(\frac{1}{2}\right)^i
% \end{equation}

% We are now ready to prove \Cref{lemma:his-fisher-finite-component}.

\begin{proof}[Proof of \Cref{lemma:his-fisher-finite-component}]
    For each $i \ge 1$, and let $\+T_i$ denote the set of 2-trees in $G_H^S$ containing $\ts(S, 0)$. Note that for each $i \ge 1$, 
    \begin{align*}
        & \left| \mu_\infty^\-{GD}\left(\left|\+T^\-{bad}\right| = i\right) \right| \\
        \le & \sum\limits_{T \in \+T_i} \left| \mu_\infty^\-{GD}\left(\+T^\-{bad}=T\right) \right| \\
    (\text{by \Cref{lemma:his-fisher-bad-tree-decay} and triangle inequality })\quad \leq &\sum\limits_{T\in \+T_i} \frac{1}{1+\varepsilon}\left(4\mathrm{e}\Delta^2 k^4\right)^{-i}\\
    (\text{by \Cref{lemma:2-tree-number-bound} and \Cref{lemma:witness-graph-degree-bound}})\quad \leq& \frac{1}{1+\varepsilon}\left(2\mathrm{e}\Delta^2 k^4\right)^{i-1}\cdot\left(4\mathrm{e}\Delta^2 k^4\right)^{-i}\\
    <&\frac{1}{1+\varepsilon}2^{-i},
    \end{align*}
    which implies the lemma.
\end{proof}

We are now ready to prove \Cref{lemma:his-fisher-marginal}.
\begin{proof}[Proof of \Cref{lemma:his-fisher-marginal}]
If $\beta = 1$, it holds trivially. If $\beta \neq 0$, it holds that $\frac{1}{1+\epsilon} \le \frac{1}{\abs{1 - \beta}}$. So it suffices to prove $\abs{\mu\left(\sigma(S) = 1^{\abs{S}}\right)} < 1 + \epsilon$.
\begin{align*}
&\abs{\mu\left(\sigma(S)=1^{|S|}\right)}
\\
% (\text{by \Cref{lemma:his-fisher-finite-component}}) \quad \le& 
% \sum\limits_{\substack{i \ge 1 \\ T \in \+T_i}} \sum\limits_{\substack{\=T(C) = T \\ \tau_C \in \{0,1\}^C}} \left| \mu^\-{GD}_\infty\left(\+T^\-{bad}=T,\+C^\-{bad}= C,\sigma_C = \tau_C\right) \right| \\
% &\qquad \cdot 
% \abs{\mu^{\-{GD}}_{\infty}\left(\sigma_{\ts(S,0)}=1^{|S|}\mid\+C^{ \-{bad}}=C, \sigma_C = \tau\right)}
% \\
% (\text{by \Cref{lemma:framework-marginal-bound}}) \quad \le& 
% \sum\limits_{\substack{i \ge 1 \\ T \in \+T_i}} \sum\limits_{\substack{\=T(C) = T \\ \tau_C \in \{0,1\}^C}} \left| \mu^\-{GD}_\infty\left(\+T^\-{bad}=T,\+C^\-{bad}= C,\sigma_C = \tau_C\right) \right|
% \\
(\text{by \Cref{lemma:framework-marginal-bound} and \Cref{lemma:his-fisher-bad-tree-decay}})\quad \le& \frac{1}{1+\varepsilon} \sum\limits_{\substack{i \ge 1 \\ T \in \+T_i}}\left(4\mathrm{e}\Delta^2 k^4\right)^{-i} 
\\
(\text{by \Cref{lemma:2-tree-number-bound} and  \Cref{lemma:witness-graph-degree-bound}})\quad \leq& \frac{1}{1+\varepsilon}\sum\limits_{i \ge 1}\left(2\mathrm{e}\Delta^2 k^4\right)^{i-1} \cdot \left(4\mathrm{e}\Delta^2 k^4\right)^{-i} 
\\
<& \frac{1}{1+\varepsilon}
\end{align*}

% \begin{align*}
% &\abs{\mu_\infty^\-{GD}\left(\sigma_S=1^{|S|}\right)}
% \\
% \le& \sum\limits_{i\geq 1}\sum\limits_{C\in \+C_i} \sum\limits_{\tau \in \{0,1\}^C} 
% \abs{\mu^{\-{GD}}_{\infty}\left(\+C^{\-{bad}}=C, \sigma_C=\tau \right)} \\
% &\qquad \times 
% \abs{\mu^{\-{GD}}_{\infty}\left(\sigma_S=1^{|S|}\mid\+C^{ \-{bad}}=C, \sigma_C = \tau\right)}
% \\
% (\text{by \Cref{lemma:his-fisher-outcome-correspondence}})\le&\sum\limits_{i\geq 1}\sum\limits_{C\in \+C_i} \sum\limits_{\tau \in \{0,1\}^C} 
% \abs{\mu^{\-{GD}}_{\infty}\left(\+C^{\-{bad}}=C, \sigma_C=\tau \right)}
% \\
% \le&\sum\limits_{i\geq 1}\sum\limits_{C\in \+C_i} \sum\limits_{\sigma \in \{0,1\}^C} 
% \abs{\mu^\-{GD}_\infty\left(\+T^\-{bad}=\=T^\-{bad}(C), \sigma_{\=T^\-{bad}(C)}=\tau_{\=T^\-{bad}(C)}\right) }\\
% &\qquad \times
% \abs{\mu^{\-{GD}}_{\infty}\left(\+C^{\-{bad}}=C, \sigma_C=\tau \mid \+T^\-{bad}=\=T^\-{bad}(C), \sigma_{\=T^\-{bad}(C)}=\tau_{\=T^\-{bad}(C)}\right)}
% \\
% \le& \sum_{\substack{i\ge 1 \\ T \in \+T_i} } \left( \sum_{\tau_T \in \{0,1\}^T} \abs{\mu^\-{GD}_\infty\left(\+T^\-{bad}=T, \sigma_{T}=\tau_{T}\right) } \right) \\
% &\qquad \times \left( \sum_{\substack{\=T^\-{bad}(C) = T \\ \sigma_{C \backslash T} \in \{0,1\}^{C \backslash T}}}\abs{\mu^{\-{GD}}_{\infty}\left(\+C^{\-{bad}}=C, \sigma_C=\tau \mid \+T^\-{bad}=T, \sigma_{T}=\tau_{T}\right)} \right)
% % \le& \sum\limits_{i \ge 1}\sum\limits_{C \in \+C_i}\sum_{\substack{\tau_T \in \{0,1\}^T(C) \\ \tau_{C \backslash T(C)} \in \{0,1\}^{C \backslash T(C)}}} \abs{\mu^{\-{GD}}_{T}(\+C^{\-{bad}}=C, \sigma_{T(C)}=\tau_{T(C)}, \sigma_{})}
% \\
% (\text{by \Cref{lemma:his-fisher-tree-pinning-bound}, \Cref{lemma:his-fisher-component-pinning-bound]}}) \quad \le& \sum_{\substack{i\ge 1 \\ T \in \+T_i} } \left(\ell^\-{pad}\right)^{k |T|} \ell^{2 k \Delta(G_H^S)^2|T|} \\
% (\text{by \Cref{lemma:2-tree-number-bound} and \Cref{lemma:witness-graph-degree-bound}})\quad \leq& \sum\limits_{i \ge 1}\left(2\mathrm{e}\Delta^2 k^4\right)^{i-1} \left(4\mathrm{e}\Delta^2 k^4\right)^{-i} \\
% <& 1.
% \end{align*}
\end{proof}
\begin{comment}

\begin{align*}
&\abs{\mu(\sigma_S=1^{|S|})}\\
\leq &
\abs{\sum\limits_{i\geq 1}\sum\limits_{C\in \+C_i} \sum\limits_{\sigma \in \{0,1\}^C} \mu^{\-{GD}}_{T}(\+C^{\-{bad}}=C, \sigma_C=\sigma)\cdot \mu^{\-{GD}}_{T}(\sigma_S=1^{|S|}\mid\+C^{ \-{bad}}=C, \sigma_C = \sigma)}\\
\le&
\sum\limits_{i\geq 1}\sum\limits_{C\in \+C_i} \sum\limits_{\sigma \in \{0,1\}^C} 
\abs{\mu^{\-{GD}}_{T}(\+C^{\-{bad}}=C, \sigma_C=\sigma)}
\cdot 
\abs{\mu^{\-{GD}}_{T}(\sigma_S=1^{|S|}\mid\+C^{ \-{bad}}=C, \sigma_C = \sigma)}\\
\le&
\sum\limits_{i\geq 1}\sum\limits_{C\in \+C_i} \sum\limits_{\sigma \in \{0,1\}^C} 
\abs{\mu^{\-{GD}}_{T}(\+C^{\-{bad}}=C, \sigma_C=\sigma)}\\
\le&
\sum\limits_{i\geq 1}
\sum\limits_{C\in \+C_i} 
\sum\limits_{\sigma \in \{0,1\}^C} 
\prod_{v \in T(C)}
\abs{\mu^{\text{LB}}(\perp)\mu^{\text{pad}}(\sigma_v)}
\prod_{v \in C \land v \notin T(C)}
\abs{\mu^{\text{LB}}(\perp)\mu^{\text{pad}}(\sigma_v)} \\
&\quad \times 
\left(
\abs{\mu^{\text{LB}}(0)} + \abs{\mu^{\text{LB}}(\perp) \mu^{\text{pad}}(0)} + \abs{\mu^{\text{LB}}(\perp) \mu^{\text{pad}}(1)}
\right)^{\Delta(G^H_S) |C|}
\\
\le&
\sum\limits_{i\geq 1}
\sum\limits_{C\in \+C_i} 
\sum\limits_{\sigma \in \{0,1\}^C} 
\prod_{v \in T(C)}
\abs{\mu^{\text{LB}}(\perp)\mu^{\text{pad}}(\sigma_v)}
\prod_{v \in C \land v \notin T(C)}
\abs{\mu^{\text{LB}}(\perp)\mu^{\text{pad}}(\sigma_v)} \\
&\quad \times 
\left(
\abs{\mu^{\text{LB}}(0)} + \abs{\mu^{\text{LB}}(\perp) \mu^{\text{pad}}(0)} + \abs{\mu^{\text{LB}}(\perp) \mu^{\text{pad}}(1)}
\right)^{\Delta(G^H_S)^2 |T|} 
\\
=&
\sum_{i\ge 1} 
\left(\abs{\mu^{\text{LB}}(0)} + \abs{\mu^{\text{LB}}(\perp) \mu^{\text{pad}}(0)} + \abs{\mu^{\text{LB}}(\perp) \mu^{\text{pad}}(1)}\right)^{\Delta(G^H_S)^2 i} \\
&\quad \times
\sum\limits_{T \in \+T_i, \sigma \in\{0,1\}^T}
\prod_{v \in T}
\abs{\mu^{\text{LB}}(\perp)\mu^{\text{pad}}(\sigma_v)}
\sum\limits_{C \in \=C_i, T=T(C), \tau \in \{0,1\}^{C \backslash T}}
\prod_{v \in C \land v \notin T(C)}
\abs{\mu^{\text{LB}}(\perp)\mu^{\text{pad}}(\sigma_v)} 
\\
\le&
\sum_{i\ge 1} 
\left(\abs{\mu^{\text{LB}}(0)} + \abs{\mu^{\text{LB}}(\perp) \mu^{\text{pad}}(0)} + \abs{\mu^{\text{LB}}(\perp) \mu^{\text{pad}}(1)}\right)^{\Delta(G^H_S)^2 i + \Delta(G^H_S) i}
\sum_{T \in \+T_i} \left( \abs{\mu^{\-{LB}}(\perp) \mu^{\-{pad}}(0)} + \abs{\mu^{\-{LB}}(\perp) \mu^{\-{pad}}(1)} \right)^{i}
% (\text{by \Cref{lemma:outcome-correspondence}})\quad\leq & \sum\limits_{i\geq 1}\sum\limits_{T\in \+T_i}\abs{\mu^{\-{GD}}_{T}(\+T^{\-{bad}}=T)}\\
% (\text{by \Cref{lemma:modulus-bound}})\quad \leq &\sum\limits_{i\geq 1}\sum\limits_{T\in \+T_i} \left(4\mathrm{e}\Delta^2 k^4\right)^{-i}\\
% (\text{by \Cref{lemma:2-tree-number-bound} and \Cref{lemma:witness-graph-degree-bound}})\quad \leq& \sum\limits_{i\geq 1}\left(2\mathrm{e}\Delta^2 k^4\right)^{i-i}\cdot\left(4\mathrm{e}\Delta^2 k^4\right)^{-i}\\
% <&1.
\end{align*}
    
\end{comment}
Now we give the omitted proofs of \Cref{lemma:his-fisher-well-define-transition}, \Cref{lemma:his-fisher-l1norm-pad} and \Cref{lemma:his-fisher-bad-tree-decay}.

\begin{proof}[Proof of \Cref{lemma:his-fisher-well-define-transition}]
    Given $v$ and $\sigma_{V \backslash \{v\}}$, let $\tilde{E} = \{e \mid \forall u,v \in e, u \neq v, \sigma_u = 1\}$. Let $\+R = \prod_{e \in \tilde{E}} \beta_e$, if $\abs{\+R} \ge 1$, then $\forall e \in \tilde{E}$, $\abs{\beta_e} \ge \frac{1}{2}$. otherwise $\abs{\+R} \le \frac{1}{2}(1 + \varepsilon)^{\Delta} < 1$. Also when $\abs{\beta} \ge \frac{1}{2}$, we know $\Arg(\beta) \le \frac{\pi}{2}$ and furthermore,
    \[
    \left|\Arg(\beta)\right| \le \tan \left|\Arg(\beta)\right| \le 2 \varepsilon.
    \]
    The first inequality is due to $x \le \tan(x)$ for $0 \le x < \frac{\pi}{2}$. The second inequality is due to the conditions in \Cref{theorem:zero-freeness-his-fisher}. 
    So $\abs{\+R} \le 2 \Delta \varepsilon < \frac{\pi}{2}$, then $\+R$ can not be $-1$. So the marginal measure is well-defined.
\end{proof}

\begin{proof}[Proof of \Cref{lemma:his-fisher-l1norm-pad}]
    % We first assume $|\beta|<1$.
    
    \begin{align*}
        % &|\mu^\-{LB}(\perp) \mu^\-{LB}(0)| + |\mu^\-{LB}(\perp)\mu^\-{pad}(1)| \\
        \ell^\-{pad} 
        =& \max_{v, \sigma_{V \backslash \{v\}}}\left( \left|\frac{1}{1 + \prod\limits_{\forall u,v\in e, u\neq v, \sigma(u)=1}\beta_e}-\frac{1}{2}\right| + \left|\frac{\prod\limits_{\forall u,v\in e, u\neq v, \sigma(u)=1}\beta_e}{1+\prod\limits_{\forall u,v\in e, u\neq v, \sigma(u)=1}\beta_e}\right| \right) \\
        % = &\max_{0 \le t \le \Delta} \left( \left|\frac{1}{1 + \beta^t}-\frac{1}{2}\right| + \left| 1 - \frac{1}{1 + \beta^t} \right| \right)
    \end{align*}
    Let $v, \sigma_{V \backslash \{v\}}$ be the parameter that maximizes $\ell^\-{pad}$. 
    Let $\tilde{E} = \{e \mid \forall u,v\in e, u\neq v, \sigma(u)=1\}$.
    Let $\+R = \prod\limits_{e \in \tilde{E}}\beta_e$. So 
     \[\ell^\-{pad} = \abs{\frac{1}{1+\+R} - \frac{1}{2}} + \abs{\frac{\+R}{1 + \+R}} = \abs{\frac{1}{1+\+R} - \frac{1}{2}} + \abs{\frac{1}{1 + \+R} - 1}. \]
    
    If $|\`R{\+R}| < \sqrt{\varepsilon}$, then there must be one $e \in \tilde{E}$, $\abs{\`R{\beta_e}} \le \sqrt{\varepsilon}$,  then $|\+R| \le \sqrt{\epsilon^2 + \sqrt{\varepsilon}^2}(1 + \varepsilon)^\Delta \le 2 \mathrm{e} \sqrt{\varepsilon}$, under the assumption of \Cref{lemma:his-fisher-marginal}, $|\+R| < 1$ ,we know that 

    \[
    \abs{\frac{1}{1 + \+R} - \frac{1}{2}}
    =\abs{\frac{1 - \+R}{2(1 + \+R)}}
    \le \frac{1 + 2 \mathrm{e} \sqrt{\varepsilon}}{2 - 4 \mathrm{e} \sqrt{\varepsilon}}
    \]

    \[
   \left|\frac{\+R}{1+\+R} \right| \le \frac{2 \mathrm{e} \sqrt{\varepsilon}}{1 - 2 \mathrm{e} \sqrt{\varepsilon}}
    \]
    So for $|\`{\+R}\beta| < \sqrt{\varepsilon}$, 
    \[
    \left|\mu^\-{LB}(\perp) \mu^\-{LB}(0)\right| + \left|\mu^\-{LB}(\perp)\mu^\-{pad}(1) \right| \le \frac{1 + 6 \mathrm{e} \sqrt{\varepsilon}}{2 - 4 \mathrm{e} \sqrt{\varepsilon}} 
    =
    \frac{1}{2} + \frac{8 \mathrm{e} \sqrt{\varepsilon}}{2 - 4\sqrt{\varepsilon}} \le \frac{1}{2} + 32 \mathrm{e} \Delta \sqrt{\varepsilon}
    \]
    
    If $\sqrt{\varepsilon} \le \`R{\+R} \le (1+\varepsilon)^\Delta$,  

    Note $ \left|\frac{1}{1 + \+R}-\frac{1}{2}\right| + \left| 1 - \frac{1}{1 + \+R} \right| $ can be seen as the sum of the distances from a complex point $\frac{1}{1 + \+R}$ to $(\frac{1}{2},0)$ and $(1,0)$. Now we characterize the possible location for $\frac{1}{1 + \+R}$.

    For $e \in \tilde{E}$, $\`R(\beta_e) \ge \sqrt{\varepsilon}/2$,  we can get that,
    \[
    \left|\Arg(\beta)\right| \le \tan \left|\Arg(\beta)\right| \le 2\frac{\varepsilon}{\sqrt{\varepsilon}} = 2\sqrt{\varepsilon}.
    \]
    So 
    \[
    \abs{\Arg(\+R)} \le 2\Delta \sqrt{\epsilon} < 1, \abs{\Arg(1 + \+R)} \le 2\Delta \sqrt{\epsilon} < 1.
    \]
    Then for $\frac{1}{1+\+R}$,
    \begin{align*}
    &\left|\Arg\left(\frac{1}{1+\+R}\right) \right| \\
    =& \left|\Arg\left(1 + \+R\right)\right| \\
    \left(x \le \tan x, \text{ for } 0\le x < \frac{\pi}{2}\right)\quad \le& \tan{\left|\Arg\left(1 + \+R\right)\right|} \\
    =& \left|\frac{\`I(1 + \+R)}{\`R(1 + \+R)}\right|
    \end{align*}



    So $\left| \Arg\left(\+R\right) \right| \le 2\Delta \sqrt{\varepsilon}$, so $\left| \`R(1+\+R) \right| \ge 1$, 
    
    \begin{align*}
    &\left|\Arg\left(\frac{1}{1+\+R}\right) \right|   \\
    \le& \left| \`I(1 + \+R) \right| \\
    \le& \left| \`I(\+R) \right| \\
    =& \left| \+R \right| \abs{\tan\left(\Arg\left(\+R\right)\right)} \\
    (\tan x \le 2 x, \text{for } 0\le x \le 1) \quad \le& \left| \+R \right| \left|2 \Arg\left(\+R\right) \right| \\
    \le& 4(1 + \varepsilon)^{\Delta} \Delta \sqrt{\varepsilon}
    \end{align*}

    Also, we know $\left| \Arg\left(\+R\right) \right| \le 2\Delta \sqrt{\varepsilon}$, so $1 + (1 + \epsilon)^\Delta \ge \left| 1 + \+R \right| > 1$.
    So we get $\frac{1}{1 + (1 + \epsilon)^\Delta} \le \left| \frac{1}{1 + \+R} \right| \le 1$,
    \[\left|\`I\left(\frac{1}{1 + \+R}\right)\right| \le 2 \left| \Arg\left( \frac{1}{1 + \+R} \right) \right| \cdot \left| \`R\left( \frac{1}{1 + \+R} \right) \right| \le 8(1 + \varepsilon)^{\Delta} \Delta \sqrt{\varepsilon},\] 
    so it holds that 

    \[
    \frac{1}{1 + \+R} \in \left\{x + y \`i \mid \frac{1}{1+(1+\varepsilon)^\Delta} \le \sqrt{x^2+y^2} \le 1, \abs{y} \le 8(1 + \varepsilon)^{\Delta} \Delta \sqrt{\varepsilon} \right\}.
    \]

    \begin{align*}
        \`R\left( \frac{1}{1+\+R} \right) &= \cos\left( \Arg\left( \frac{1}{1+\+R} \right) \right) \abs{\frac{1}{1+\+R}} 
        \ge \frac{1}{1+(1+\varepsilon)^\Delta} - \frac{1}{2} \left(8(1 + \varepsilon)^{\Delta} \Delta \sqrt{\varepsilon}\right)^2.
    \end{align*}
The location of $\frac{1}{1 + \+R}$ implies that, 
    \begin{align*}
    &\left( \left|\frac{1}{1 + \+R}-\frac{1}{2}\right| + \left| 1 - \frac{1}{1 + \+R} \right| \right)
    \\
    (\text{by triangle inequality})&\le \frac{1}{2} + 2\left( \frac{1}{2} - \frac{1}{1+(1+\varepsilon)^\Delta} + \frac{1}{2} \left(8(1 + \varepsilon)^{\Delta} \Delta \sqrt{\varepsilon}\right)^2  + 8(1 + \varepsilon)^{\Delta} \Delta \sqrt{\varepsilon} \right) 
    \\
    &\le 
    \frac{1}{2}
    +
    2\frac{(1 + \varepsilon)^\Delta - 1}{1 + (1 + \varepsilon)^\Delta} + 16(1 + \varepsilon)^{\Delta} \Delta \sqrt{\varepsilon}
    \\
    (\text{$e^x \le 1 + 2x$ for } 0 \le  x \le 1)&\le
    \frac{1}{2}
    +
    4\Delta \epsilon + 16(1 + \varepsilon)^{\Delta} \Delta \sqrt{\varepsilon}
    \\
    &\le
    \frac{1}{2}
    + 
    32 \mathrm{e} \Delta \sqrt{\varepsilon}.
    \end{align*}
    
    % \begin{align*}
    % &\max_{0 \le i \le \Delta} \left( \left|\frac{1}{1 + \beta^t}-\frac{1}{2}\right| + \left| 1 - \frac{1}{1 + \beta^t} \right| \right)  \\
    % &\le 2 \sqrt{\left(\frac{1}{4}\right)^2 + \left(\frac{(1 + \varepsilon)^\Delta \sqrt{\varepsilon}}{25 \pi}\right)^2} \\
    % &= \frac{1}{2} \sqrt{1 + \left(\frac{4(1 + \varepsilon)^\Delta \sqrt{\varepsilon}}{25 \pi}\right)^2} \\
    % \left(\sqrt{1 + x} \le 1 + \frac{x}{2}\right) \quad &\le \frac{1}{2} + \frac{8(1 + \varepsilon)^{2\Delta} \varepsilon}{625 \pi^2} \\
    % (\text{by conditions in \Cref{lemma:his-fisher-marginal}})\quad &\le \frac{1}{2} + \frac{8 \mathrm{e} \varepsilon}{625 \pi^2} \\
    % &\le \frac{1}{2} + 800 \pi \Delta \sqrt{\varepsilon}
    % \end{align*}
    % $\left|\Arg(\beta)\right| \le \`I(1 + \beta^t) = \`I(\beta^t) = |\beta^t| \tan(\Arg(\beta^t))$
\end{proof}

% \begin{proof}[Proof of \Cref{lemma:his-fisher-tree-pinning-bound}]

% Recall the proof of \Cref{lemma:modulus-bound}, the event $\+T^\-{bad} = T$ can be translated to the following:

% \begin{enumerate}
%     \item \label{item:his-fisher-modulus-bound-1} for each $e \in T$, we have $r_t = \perp$ for all $t \in e$;
%     \item \label{item:his-fisher-modulus-bound-2} the $r_t$s on all other vertices in $G^S_H$ that are within distance $2$ of $T$ satisfy certain resctrictions so that $\+T^\-{bad} = T$.
% \end{enumerate}

% Here, the \Cref{item:his-fisher-modulus-bound-1} contributes a factor $\left(\ell^\-{pad}\right)^{k |T|}$ by the definition of 2-trees that all vertices in $T$ contain disjoint timestamps and triangle inequality. We can also use a simple triangle inequality to bound \Cref{item:his-fisher-modulus-bound-2}. Since there are at most $|T|\Delta(G_S^H)^2$ vertices and therefore $k|T|\Delta(G_H^S)$ timestamps included, this contributes a factor at most $\ell^{k|T|\Delta(G_H^S)}$, where $\Delta(G_H^S)$ is the maximum degree of $G_H^S$.

% Overall, we have

% \begin{align*}
%     &\mu_\infty^\-{GD}(\+T^\-{bad} = T) \\
%     \le& \left(\ell^\-{pad}\right)^{k |T|} \ell^{k  \Delta\left(G_H^S\right)^2 |T|} \\
%     (\text{by \Cref{lemma:2-tree-number-bound}}) \quad \le& \left(\ell^\-{pad}\right)^{k |T|} \ell^{4  \Delta^2 k^5 |T|} \\
%     \le& \left(\frac{1}{2} + 800 \Delta \pi \sqrt{\varepsilon} \right)^{k |T|} \left( 1 + 800 \Delta \pi \sqrt{\varepsilon} \right)^{4 \Delta^2 k^5 |T|} \\
%     \text{(by conditions in \Cref{lemma:his-fisher-marginal})} \le& \left( 4 \mathrm{e} \Delta^2 k^4 \right)^{-|T|}.
% \end{align*}
% \end{proof}

% To prove \Cref{lemma:his-fisher-component-pinning-bound}, we prove a stronger lemma (\Cref{lemma:his-fisher-rc-bound}) which can implies \Cref{lemma:his-fisher-component-pinning-bound}. Before we give \Cref{lemma:his-fisher-rc-bound}, we define some notations.

% Given $\+T^\-{bad} = T$, let $U$ include all vertices in $G_H^S$ whose distance to $T$ are less than $2$. Note $U$ contains all vertices for all possible bad components and their neighbours due to \Cref{definition:stationary-start} and \Cref{definition:bad-vertices-his}. 
% We sort the timestamps in $U$ forming a sequence $\-{TP} = (t_1, t_2, \dots, t_m)$ such that $t_1 < t_2 < \dots < t_m$.
% Recall the definition of the decomposed systematics scan Glauber dynamics (\Cref{definition:decomposed-systematic-scan-glauber-dynamics}), each time $t$ associate with $r_t$ and $c_t$. We define the vector form of $r$'s and $c$'s as $\vec{r} = (r_{t_1},r_{t_2}, \dots, r_{t_m})$, $\vec{c} = (c_{t_1}, c_{t_2}, \dots, c_{t_m})$.
% Note once $\vec{c}$ is fixed, the configuration on $C$ is fixed.
% Define $\Omega_T = \{(\vec{r}, \vec{c}) \times \{0,1\}^C \mid \=T(C) = T, (\vec{r}, \vec{c}) \in \{0,\perp\}^{C}\}$ be the set containing all possible $(\vec{r},\vec{c})$'s on all possible bad components, note this set is finite due to the size limit of bad component given the bad tree. 
% We abuse the notation a little, let $\mu^{\-{pad}, \vec{r}, \vec{c}}_{v(t_i)}(c_{t_i})$ be the padding measure condition on $\vec{r}, \vec{c}$ except $r_{t_i}$ and $c_{t_i}$ as \Cref{definition:marginal-lower-bounds}. 
% Let $\tilde{G} = (U, \tilde{E})$ be the vertex induced subgraph of $G_H^S[U]$. We transfer $\tilde{G}$ to a directed $\vec{G} = (U, \vec{E})$ that we will use induction on its topological order to prove this lemma. 

% $\vec{G}$ is constructed as follows: 
% for every $(\ts(e_1, t_1), \ts(e_2, t_2)) \in E_H^S$, w.l.o.g. we assume $t_1 < t_2$, then we add $\ts(e_1, t_1) \to \ts(e_2, t_2)$ into 
% $\vec{E}$.

% \yxtodo{The notation for vector r should be modified}
% Fix an arbitrary order of the possible topological orders $\text{TP} = (v_1, v_2, \dots, v_{|U|})$.
% $\text{TP} = (\ts(e_1, t_1), \ts(e_2, t_2), \dots, \ts(e_{|U|}, t_{|U|}))$.
% Consider given $\+C^\-{bad}=C$ and $$.

% Fix a component $C$ and corresponding $(\vec{r}, \vec{c})$, if $v \notin C$, we say that $v \notin (\vec{r}, \vec{c})$. We also abuse this notation we denote $\vec{r} \in \Omega_T$ if $\exists \vec{c}$ such that $(\vec{r}, \vec{c}) \in \Omega_T$. And for $\vec{c} \in \{0,1\}^{i}$, we denote $(\vec{r}, \vec{c}) \in \Omega_T$ if there is a extension $\vec{c}^*$ of $\vec{c}$ such that $(\vec{r}, \vec{c}) \in \Omega_T$.

% We give the following lemma,
% \begin{lemma}\label{lemma:his-fisher-rc-bound}
% Suppose the conditions of \Cref{lemma:his-fisher-marginal}.
%     Let $T$ be any finite non-empty $2$-tree of $G_H^S$ containing $\ts(S, 0)$. Then,
%     \[
% \sum\limits_{
% \substack{
% \=T(C) = T \\
% (\vec{r},\vec{c}) \in \Omega_T
% }}
% \abs{\mu^\-{GD}_\infty \left( \+T^\-{bad} = T, \+C^\-{bad} = C, \vec{r}, \vec{c} \right)}
% \le 
% \left( \ell^\-{pad} \right)^{k |T|} \ell^{k\Delta(G_H^S)^2 \abs{T}}.
%     \]
% \end{lemma}

% We first show \Cref{lemma:his-fisher-rc-bound} implies \Cref{lemma:his-fisher-component-pinning-bound}. 
\begin{proof}[Proof of \Cref{lemma:his-fisher-bad-tree-decay}]
% \yxtodo{Change the enumeration of c's.}
~

% Given a bad component $C$ and the configuration on it $\sigma_C$. Let $\vec{c} = (\sigma_{t_1}, \sigma_{t_2}, \dots, \sigma_{t_m})$. By triangle inequality, 
% \[
% \abs{\mu^\-{GD}_\infty\left( \+T^\-{bad}=T, \+C^\-{bad}=C, \sigma_C = \tau_C \right)} 
% \le
% \sum\limits_{\vec{r} \in \{0,1\}^C}
% \abs{\mu^\-{GD}_\infty \left( \+T^\-{bad}=T, \+C^\-{bad}=C, \vec{r}, \vec{c}  \right)}.
% \]

By \Cref{lemma:framework-marginal-lower-bound-to-bad-tree-decay}, we only need to verify that $\left(\ell^\-{pad}\right)^{k \abs{T}} \ell^{k \Delta(G_H^S)^2 \abs{T}} \le \frac{1}{1+\varepsilon} \left( 4 \mathrm{e} \Delta^2 k^4 \right)^{-\abs{T}}$.

\[
\left(\ell^{\-{pad}}\right)^{k \abs{T}} \le \left(\frac{1}{2}+32\mathrm{e}\Delta \sqrt{\varepsilon}\right)^{k \abs{T}} \le \mathrm{pow}\left(2, \left(-1+96\mathrm{e}\Delta \sqrt{\varepsilon} \right) k \abs{T}\right),
\]
where $\mathrm{pow}(a,b) = a^b$,
the first inequality is by \Cref{lemma:his-fisher-l1norm-pad} and the second inequality is by $32 \mathrm{e} \Delta \sqrt{\varepsilon} < 1$ and $\log_2\left(\frac{1}{2}+x\right) \le -1+3x$ for $0 \le x \le 1$.

\[
\ell^{k \Delta(G_H^S)^2 \abs{T}} \le \ell^{4 \Delta^2 k^5 \abs{T}} \le \left(1 + 32\mathrm{e}\Delta \sqrt{\varepsilon} \right)^{4 \Delta^2 k^5 \abs{T}} \le \mathrm{pow}\left(2, 256 \mathrm{e} \Delta^3 k^5 \sqrt{\varepsilon} \abs{T} \right),
\]
the first inequality is by \Cref{lemma:witness-graph-degree-bound}, the second inequality is by \Cref{lemma:his-fisher-l1norm-pad} and the last inequality is by $32\mathrm{e}\Delta\sqrt{\varepsilon}< \frac{1}{2}$ and $1 + \frac{x}{2}\le 2^x$ for $x > 0$.

\begin{align*}
\frac{1}{1+\varepsilon} \left( 4 \mathrm{e} \Delta^2 k^4 \right)^{-\abs{T}} 
&= \mathrm{pow}\left(2, -\abs{T} \log_2(4 \mathrm{e} \Delta^2 k^4) + \log_2 \left(\frac{1}{1 + \varepsilon} \right) \right) \\
&\ge 
 \mathrm{pow}\left(2, -\abs{T} \log_2(4 \mathrm{e} \Delta^2 k^4) - 2\sqrt{\varepsilon} \right),
\end{align*}
the last inequality is by $\log_2 \left(\frac{1}{1+x}\right) > -2 \sqrt{x}$ for $0 < x \le 1$. Let $f(x) = \log_2\left(\frac{1}{1+x}\right) + 2 \sqrt{x}$, $f'(x) = \frac{1}{\sqrt{x}} - \frac{1}{(1+x)\log 2} \ge \frac{1}{\sqrt{x}} - \frac{1}{\log 2} = \frac{-\sqrt{x}+\log 2 + x \log 2}{\sqrt{x}(1+x)\log 2} > 0$ for $0 < x \le 1$. And $f(0) = 0$ so $f(x)>0$ for $0 < x \le 1$. 

Finally, we can verify that under the conditions of \Cref{lemma:his-fisher-marginal}, it holds that,
\[
\left(-1+96\mathrm{e}\Delta \sqrt{\varepsilon} \right) k \abs{T} + 256 \mathrm{e} \Delta^3 k^5 \sqrt{\varepsilon} \abs{T}  \le -\abs{T} \log_2(4 \mathrm{e} \Delta^2 k^4) - 2\sqrt{\varepsilon}.
\]
Simplifying the above inequality gives that
\[
\varepsilon \le \left(\frac{k - \log_2(4 \mathrm{e} \Delta^2 k^4)}{2 + 96\mathrm{e}\Delta + 256 \mathrm{e} \Delta^3 k^5}\right)^2.
\]

% \yxtodo{alter the number into ell.}
\end{proof}

% Now we prove \Cref{lemma:his-fisher-rc-bound}
% \begin{proof}[Proof of \Cref{lemma:his-fisher-rc-bound}]
% Given $\+C^\-{bad} = C, \vec{r}, \vec{c}$, we can calculate $\abs{\mu_\infty^\-{GD}\left( \+T^\-{bad} = T, \+C^\-{bad} = C, \vec{r}, \vec{c} \right)}$ via the following procedure.

% \begin{enumerate}
%     \item We enumerate all timestamps in $C$ by the order $\-{TP}$;
%     \item For the $i$-th timestamps,
%     \begin{itemize}
%         \item if $r_{t_i} = \perp$, it contributes $\abs{\mu^\-{LB}(\perp)} \cdot \abs{\mu^{\-{pad}, \vec{r}, \vec{c}}_{t_i}(c_i)}$.
%         \item otherwise, it contributes $\abs{\mu^\-{LB}(0)}$.
%     \end{itemize}
% \end{enumerate}
% % \begin{enumerate}
% % \item Set $B = \emptyset$, we enumerate all timestamps in $C$ by the order $\-{TP}$;
% % \item For $t_i$,
% % \begin{itemize}
% %     \item If $r_{v(t_i)} = 0$, the contribution of it bounded by $\abs{\mu^\-{LB}(0)}$;
% %     \item otherwise, $B \gets B \cup \{t_i\}$.
% % \end{itemize}
% % For $t_j \in B$ satisfying $\forall a, \exists v \in V_H^S, \text{s.t.}  $. Compute the contribution of $a$ via the following sub-procedure.
% % \begin{itemize}
% %     \item If $r_a = \perp$, contribute $\abs{\mu^\-{LB}(\perp) \mu^{\-{pad}, \vec{r}, \vec{c}}_{a}(c_a)} $;
% %     \item Otherwise, contribute $\abs{\mu^\-{LB}(0)}$.
% % \end{itemize}

% % Set $S \gets S \backslash \{a\}$.
% % \end{enumerate}

% Now let $R_i = \{\{(r_1,\tau_{1}), (r_2,\tau_2), \dots, (r_i,\tau_i)\} \mid \vec{r}\}$ be the set containing all possible $r$'s and $\tau$'s of the first $i$ timestamps in the order of $\-{TP}$.

% Set 
% \[
% A_i = \sum\limits_{(\vec{r},\vec{\tau}) \in R_i} \prod\limits_{j \le i} \left( \mu^\-{LB}(0)\cdot \=I[r_j = 0] + \ell^\-{pad} \cdot \=I[r_j = \perp] \right).
% \]

% By the aforementioned procedure, it holds that,

% \[
% \sum\limits_{
% \substack{
% \=T(C) = T \\
% (\vec{r},\vec{c}) \in \Omega_T
% }}
% \abs{\mu^\-{GD}_\infty \left( \+T^\-{bad} = T, \+C^\-{bad} = C, \vec{r}, \vec{c} \right)}
% \le A_m.
% \]

% We show that $A_m \le \left( \ell^\-{pad} \right)^{k |T|} \ell^{k \Delta(G_H^S)^2 \abs{T}}$ by induction. Specifically, we prove 

% \[A_i \le \left( \ell^\-{pad} \right)^{\abs{\{t_j \mid t_j \in T, j\le p \}}} \ell^{i - \abs{\{t_j \mid t_j \in T, j\le p \}}}.\]

% For the base case, we set $A_0 = 1$.
% Assume it holds for $i < p$, for $i = p$,
% \begin{itemize}
%     \item if $t_i \in T$, it contributes at most $\ell^\-{pad}$ in all possible bad component. So 
%     \[A_p \le A_{p-1} \ell^\-{pad} \le \left( \ell^\-{pad} \right)^{\abs{\{t_j \mid t_j \in T, j\le p \}}} \ell^{i - \abs{\{t_j \mid t_j \in T, j\le p \}}}.\]
%     \item otherwise if $t_i$ is the bad component, it contributes $1$. If $t_i$ is in the bad component, it contributes at most $\ell$. So it contributes at most $\ell$. So
%     \[A_p \le A_{p-1} \ell \le \left( \ell^\-{pad} \right)^{\abs{\{t_j \mid t_j \in T, j\le p \}}} \ell^{i - \abs{\{t_j \mid t_j \in T, j\le p \}}}.\]
% \end{itemize}

% So it holds that,

% \[
% \sum\limits_{
% \substack{
% \=T(C) = T \\
% (\vec{r},\vec{c}) \in \Omega_T
% }}
% \abs{\mu^\-{GD}_\infty \left( \+T^\-{bad} = T, \+C^\-{bad} = C, \vec{r}, \vec{c} \right)}
% \le \left( \ell^\-{pad} \right)^{k |T|} \ell^{k \Delta(G_H^S)^2 \abs{T}}.
% \]

% Now we can upper bound the total contribution of all possible $\vec{r},\vec{c}$ by addition principle and multiplication principle.

% \begin{itemize}
%     \item For $a \in T$, it may contribute $\max\limits_{\vec{r}, \vec{c}}\abs{\mu^\-{LB}(\perp) \mu^{\-{pad}, \vec{r}, \vec{c}}_{a}(0)} + \abs{\mu^\-{LB}(\perp) \mu^{\-{pad}, \vec{r}, \vec{c}}_{a}(1)} \le \ell^\-{pad}$;
%     \item For $a \notin T$, it may contribute
%     $ \abs{\mu^\-{pad}(0)} +  \max\limits_{\vec{r}, \vec{c}}\abs{\mu^\-{LB}(\perp) \mu^{\-{pad}, \vec{r}, \vec{c}}_{a}(0)} + \abs{\mu^\-{LB}(\perp) \mu^{\-{pad}, \vec{r}, \vec{c}}_{a}(1)} \le \ell^\-{pad} \le \ell$.
% \end{itemize}
% \end{proof}

==> interpolation.tex <==
In this section, we prove \Cref{corollary:fptas-his}.
Fix $k \ge 2$, $\Delta \ge 3$  and $0 < \epsilon < \frac{1}{9k^5 \Delta^2}$ for $k$-uniform hypergraph $H = (V, \+E)$ with maximum degree $\Delta$, we can get the zero-free region $\+D_\epsilon$ by \Cref{theorem:zero-freeness-his-lee-yang} and we express its partition function by
\[
Z^\-{ly}(\lambda) = \sum\limits_{i=1}^{\abs{V}} a_i \lambda^i,
\]
where $a_i$ stands for the number of $i$-size independent sets of $H$.

We first introduce a well-known lemma that can map the zero-free strip into a zero-free disk centered at the origin by Barvinok.

\begin{lemma}[\text{\cite[Lemma 2.2.3]{barvinok2016combinatorics} }]
\label{lemma:zero-free-region-mapping}
There is a polynomial $\phi$, mapping 
\[
\+D' = \{x \in \=C \mid  -\tau \le \`R x \le 1 + \tau, \abs{\`I x} \le \tau \}
\]

to a disk $D(0, 1 + \delta)$ centered at the origin. Moreover, it holds that $\phi(0) = 0$, $\phi(1) = 1$ and the degree of $\phi$ is $\exp (\Theta(\tau^{-1}))$ and with $\delta = \exp(-\Theta(\tau^{-1}))$.
\end{lemma}

Let $g(x) = Z(\lambda x)$, with \Cref{lemma:zero-free-region-mapping}, we can reduce the computation of $Z^\-{ly}(\lambda)$ to that of polynomial $f(1)$ which $f(x) = g(\phi(x))$ with degree at most $\abs{V} \exp(\Theta(\tau^{-1}))$ that is zero-free on the disk $D(0, 1 + \delta)$.


let $T_r(x)$ be the order-$r$ truncation of the Taylor series for $\log f(x)$ around 0. The following lemma shows that $T_r(x)$ can be used to approximate $\log f(x)$.

\begin{lemma}[\cite{barvinok2016combinatorics} Lemma 2.2.1]
\label{lemma:truncation-log-pf}
    Let $f(x)$ be a polynomial with degree at most $N$, and suppose that $f(x) \neq 0$ when $\abs{x} \le 1 + \delta$, then for $\abs{x} < 1 + \delta$,

    \[
    \abs{T_r(x) - \log f(x)} \le \frac{N(\abs{x}/(1 + \delta))^{r+1}}{(r + 1)(1 - \abs{x}/(1 + \delta))}.
    \]

\end{lemma}

Then we introduce the last remaining part to prove \Cref{corollary:fptas-his}.

\begin{lemma}[\text{\cite[Lemma 3.1]{Liu2017TheIP}}]
\label{lemma:computing_leading_coefficents}
    Fix $k, \Delta$ and $C > 0$. For hypergraph $H = (V, \+E)$ with maximum degree $\Delta$ and maximal edge size $k$. There is an algorithm running in time polynomial in $n/\varepsilon$ that computes $e_i$ for $i=1, \dots, r$, where $r = \lceil C \log \left(n/\varepsilon \right) \rceil$.
\end{lemma}

Now it is ready to prove \Cref{corollary:fptas-his}.

\begin{proof}[Proof of \Cref{corollary:fptas-his}]
    With \Cref{lemma:zero-free-region-mapping}, we first get a polynomial $\phi$ which maps $\+D_\varepsilon$ to the disk $D(0, \delta)$ where $\delta = \exp(-\Theta(9k^5 \Delta^2))$. The degree of $\phi$ is $\exp(\Theta(9k^5 \Delta^2))$.
    Let $f(x) = Z(\lambda \phi(x))$, we know that $f$ is a polynomial with maximum degree $\abs{V} \exp(\Theta(9 k^5 \Delta^2))$. By \Cref{lemma:truncation-log-pf}, there exists a constant $C = C(\delta)$ and $r = C \log\left( \frac{ \abs{V} \exp(\Theta(9k^5 \Delta^2)) }{\varepsilon} \right)$ such that $\abs{T_r(1) - \log f(1)} \le \varepsilon$.

    Now the remaining part is to compute $T_r(1)$. 
    Since the coefficients of the truncated Taylor series $T_r(1)$ can be expressed as the first $r$ inverse power sum of roots which can be computed through a triangular system of linear equations given the first $r$ coefficients of $f(x)$ in time $O(r^3)$.
    
    Note $f(x) = Z(\lambda \phi(x))$ which is a function composed by $Z, \lambda$ and $\phi$. We can calculate the first $r$ coefficients of $f(x)$ in time $O(r^2)$ given $a_i$ for $i = 1, \dots , r$ and $\phi$. 
    And $a_i$ for $i=1,\dots,r$ can be computed via \Cref{lemma:computing_leading_coefficents} in time polynomial in $\exp(r)/\epsilon$.

    So the algorithm runs in time polynomial in $\abs{V} \exp(\Theta(9 k^5 \Delta^2))/\varepsilon$ which is a FPTAS.
\end{proof}

==> refined_fisher.tex <==

\subsection{Fisher zeroes}

% In this subsection, we show a reduction from Fisher zeroes to Lee-yang zeroes. Then we use multivariate Lee-yang zero-free region to prove \Cref{theorem:zero-freeness-his-fisher}.

We begin by introducing some necessary notation. Consider a $k$-uniform hypergraph $H=(V,\+E)$ with maximum degree $\Delta$.
A configuration $\sigma\in \{0,1\}^V$ is called an \emph{independent set} of $H$ if for every hyperedge $e \in \+E$.
The independence polynomial of the hypergraph $H$ on Fisher zeroes is defined as
\[
Z_H^\-{fs}(\*\beta) = \sum\limits_{\sigma \in \{0,1\}^V} \prod\limits_{\substack{e: \sigma(e)=1^k}} \beta_e,
\]

% where we assume $\beta_{e} \neq 1$, otherwise we can remove edge $e$ without changing the partition function's value.
\begin{comment}
We give the reduction.
\begin{lemma}[reduction from Lee-yang zeroes to Fisher zeroes]
\label{lemma:reduction-lee-yang-fisher}
Let $H=(V, \+E)$ be a $k$-uniform hypergraph with maximum degree $\Delta$. For $\*\beta \in \=C^\-{\abs{\+E}}$, we can construct a $k+1$-uniform hypergraph $H^*=(V^*, \+E^*)$ with maximum degree $\Delta$ and $\*\lambda_{\*\beta}$ such that $Z_H^\-{fs}(\*\beta) = Z_{H^*}^\-{ly}(\*\lambda_{\*\beta})$ by the following procedure:
\begin{enumerate}
    \item let $V = \{v_1, v_2, \dots, v_{\abs{V}}\},  \tilde{\+E} = \{e \mid e \in \+E, \beta_e \neq 1\}  , \tilde{\+E} = \{e_1, e_2, \dots, e_{\abs{\tilde{\+E}}}\}$, for each edge $e_i$, add a new vertex $u_i$, i.e. 
    \[
    V^* = V \cup \{u_1, u_2, \dots, u_{\abs{\tilde{\+E}}}\},\quad \+E^* = \{ e_i \cup \{u_i\} \mid \forall e_i \in \tilde{\+E} \}.
    \]
    \item set $\lambda_{v_i}=1$ for $v_{i}\in V$ and $\lambda_{u_i} = \frac{1 - \beta_{e_i}}{\beta_{e_i}}$ for $u_1, u_2, \dots u_{\abs{\tilde{\+E}}}$.
\end{enumerate}
\end{lemma}
\begin{proof}
    It can be verify that $H^*$ is a $k+1$-uniform hypergraph with maximum degree $\Delta$: for each edge in $\+E$, we add a new vertex. Now we verify that $Z_H^\-{fs}(\*\beta) = \prod_{e_i} (1 - \beta_{e_i}) \cdot Z_{H^*}^\-{ly}(\*\lambda_{\*\beta})$.
    First we remove all edges $e$ with $\beta_e=1$ which does not affect the partition function's value. Then we verify the equivalence:
    \begin{align*}
        Z^\-{fs}_H(\*\beta) &=  \sum\limits_{\sigma \in \{0,1\}^V} \prod\limits_{\substack{e: \forall v \in e, \sigma(v)=1}} \beta_e \\
        &= \sum\limits_{\sigma \in \{0,1\}^V} \prod\limits_{\substack{e_i: \forall v \in e_i, \sigma(v)=1}} (1 - \beta_{e_i})\lambda_{u_i}  \\
        &= \sum\limits_{\sigma \in \{0,1\}^V} \left(\left(\prod\limits_{\substack{e_i: \forall v \in e_i, \sigma(v)=1}} (1 - \beta_{e_i})\lambda_{u_i}\right) \cdot \left(\prod\limits_{e_i: \exists v_j \in e_i, \sigma(v_j) = 0} (1-\beta_{e_i})(1 + \lambda_{u_i}) \right) \right)\\
        &= \prod_{e_i} (1 - \beta_{e_i}) \cdot Z_{H^*}^\-{ly}(\*\lambda_{\*\beta}).
    \end{align*}
\end{proof}

Then \Cref{theorem:zero-freeness-his-lee-yang} implies \Cref{theorem:zero-freeness-his-fisher}.

\begin{proof}[Proof of \Cref{theorem:zero-freeness-his-fisher}]
    Let $H=(V, \+E)$ be a $k$-uniform hypergraph with maximum degree $\Delta$. Let $\*\beta \in \+D_{\epsilon}^\+{E}$. Then we use \Cref{lemma:reduction-lee-yang-fisher} to construct $k+1$ uniform hypergraph  $H^* = (V^*, \+E^*)$ with maximum degree $\Delta$. It suffices to check that $Z_{H^*}^\-{ly}(\*\lambda_{\*\beta})$ is non-zero. By \Cref{theorem:zero-freeness-his-lee-yang}, we know $Z_{H^*}^\-{ly}(\*\lambda_{\*\beta})$ is indeed non-zero.
\end{proof}
\end{comment}
with the associated measure $\mu_{\*\beta} = \mu_{\*\beta,H} : \{0,1\}^V \to \={C}$ defined as

\[
\forall \sigma \in \{0,1\}^V, \quad \mu_{\*\beta}(\sigma) = \frac{\prod_{e: \sigma(e) = 1^k}\beta_e}{Z^\-{fs}_H(\*\beta)},
\]

when $Z^\-{fs}_H(\*\beta) \neq 0$. For the brevity of notation, we will regard $\mu$ as $\mu_{\*\beta}$ in this subsection. Given $v$ and $\sigma_{V \backslash \{v\}}$, let $\tilde{E} = \{e \mid \forall u, v \in e, u \neq v, \sigma_u = 1\}$.



\[
\mu_v^{\sigma(V \backslash \{v\})}(0) = \frac{1}{1 + \prod_{e \in \tilde{E}} \beta_e}, \quad \mu_v^{\sigma(V \backslash \{v\})}(1) = \frac{\prod_{e \in \tilde{E}} \beta_e}{1 + \prod_{e \in \tilde{E}} \beta_e}.
\]

Again we utilize the edge-wise self-reducibility and it suffices to prove the following lemma.

\begin{lemma}\label{lemma:his-fisher-marginal}
Let $H(V, \+E)$ be a $k$-uniform hypergraph with maximum degree $\Delta$, Let $\varepsilon = \varepsilon_{k, \Delta}$ and $\+D_\varepsilon$ be as defined in \Cref{theorem:zero-freeness-his-fisher}. Suppse $Z^\-{fs}_H(\*\beta) \neq 0$ and therefore $\mu_{\*\beta}$ is well-defined. For any $S \subseteq V$, $|S|=k$ and $\*\beta \in \+D_\varepsilon^V$, it holds that
\[
(1 - \beta)\mu\left(\sigma(S) = 1^{|S|}\right) \neq 1.
\]
\end{lemma}

Like \Cref{lemma:his-lee-yang-marginal}, It suffice to prove \Cref{lemma:his-fisher-marginal} to prove \Cref{theorem:zero-freeness-his-fisher}.

\begin{proof}[Proof of \Cref{theorem:zero-freeness-his-fisher}]
    Let $\+E = \{e_1, e_2, \dots, e_m\}$. For $0 \le i \le m$ we let $\+E_i = \{e_1, e_2, \dots, e_i\}$ and let $H_i = (V, \+E_i)$. We prove by induction that $Z_{H_i}^\-{fs}(\*\beta) \neq 0$ for each $0 \le i \le m$.

    The base case is when $i = 0$, and we have $Z_{H_0}^\-{fs} = 2^{\abs{V}}$.

    For the induction step, we fix $0 \le i < m$ and assume that $Z_{H_i}^\-{fs} \neq 0$. Then the measure $\mu_{H_i}$ is well-defined. Note that

    \[
    \frac{Z_{H_{i+1}}^\-{fs}(\*\beta)}{Z_{H_i}^\-{fs}(\*\beta)}=\frac{Z_{H_i}^\-{fs}(\*\beta) - (1 - \beta_{e_{i+1}})\sum\limits_{\substack{\sigma \in \{0,1\}^{V} \\ \sigma(e_{i+1}) = 1^{k}}} \prod_{\forall v \in e, \sigma(v)=1}\beta_e  }{Z_{H_i}^\-{fs}(\*\beta)} = 1 - (1 - \beta_{e_{i+1}})\mu_{H_i}\left(\sigma(e_{i+1}) = 1^k \right) \neq 0,
    \]
    % \yxtodo{Here is a small error to fix: the wrong telescoping.}
    where the last inequality is by \Cref{lemma:his-fisher-marginal}. Therefore $Z_{H_i}^\-{fs} \neq 0$, completing the induction step and the proof of the lemma.
\end{proof}

In order to apply our framework, we first check that the systematic scan Glauber dynamics's transitions are well-defined by the next lemma.
% The marginal measure $\mu_v^{\sigma(V \backslash \{v\})}$ is also well-defined by the next lemma which 
We defer the proof to the end of this subsection. 
% when $\forall 0 \le i \le \Delta, \beta^{i} \neq -1$ for any $\sigma \in \{0,1\}^V$ and $v$ where $\Delta$ is the maximum degree of the graph $H$.

\begin{lemma}\label{lemma:his-fisher-well-define-transition}
    Suppose the conditions in \Cref{lemma:his-fisher-marginal}, for any $v$ and $\sigma_{V \backslash \{v\}}$, the marginal measure $\mu_v^{\sigma(V \backslash \{v\})}$ is well defined.
\end{lemma}

We set the lower bound measures for any $v \in V$ (\Cref{definition:decomposition-scheme}) as follows for hypergraph independent sets:


% Wait
% \[
% \mu^{\text{LB}}(0) = \frac{1}{1 + |\beta|^\Delta}, \quad \mu^{\text{LB}}(1) = 0, \quad \mu^{\text{LB}}(\perp) = \frac{|\beta|^\Delta}{1 + |\beta|^\Delta}.
% \]

% For $|\beta| < 1$, we set 

\[
\mu^{\-{fs, LB}}(0) = \frac{1}{2}, \quad \mu^{\-{fs, LB}}(1) = 0, \quad \mu^{\-{fs, LB}}(\perp) = \frac{1}{2},
\]
so that $\mu$ is $(\ell^\-{fs, pad}, \ell^\-{fs})$-marginally lower bounded (\Cref{definition:decomposition-scheme}).

Let 
\[\ell^{\-{pad}} = \max\limits_{v, \sigma_{V \backslash v}}\left(\abs{ \mu^\-{fs, LB}(\perp) \mu_{v}^{\-{fs, pad},\sigma_{V \backslash v}}(0)} + \abs{\mu^\-{fs, LB}(\perp)\mu_{v}^{\-{fs, pad},\sigma_{V \backslash v}}(1)}\right),\]

\[
\ell = \mu^\-{fs, LB}(0) + \ell^\-{fs, pad}.
\]
We also need the following lemma to bound $\ell^\-{pad}$ and $\ell$, we delay its proof to the end of this subsection.

\begin{lemma}[bounds on $\ell^\-{fs, pad}$ and $\ell^\-{fs}$]
\label{lemma:his-fisher-bound-fs-l-l-pad}
    Suppose the condition of \Cref{lemma:his-fisher-marginal}, it holds that,
    \[
    \ell^\-{fs, pad} \le \frac{1}{2} + 6 \Delta \varepsilon,\quad \ell^\-{fs} \le 1 + 6 \Delta \varepsilon.
    \]
\end{lemma}

Then we give the decay of bad trees by \Cref{lemma:bad-tree-decay}. We defer its proof to the end of this subsection.

\begin{lemma}[decay of bad trees]\label{lemma:his-fisher-bad-tree-decay} Suppose the conditions of \Cref{lemma:his-fisher-marginal}, it holds that,
    \[
    \sum_{\substack{C: \=T(C) = T \\ \tau \in \{0,1\}^C}} \left| \mu^\-{GD}_\infty\left(\+T^\-{bad}=T,\+C^\-{bad}= C,\sigma(C) = \tau\right) \right| 
\le \left( \ell^\-{fs, pad} \right)^{k \abs{T}} \left(\ell^\-{fs}\right)^{k \Delta(G_H^S)^2 \abs{T}} \le \frac{1}{1+\varepsilon} \left(4 \mathrm{e} \Delta^2 k^4\right)^{-\abs{T}}.
    \]
\end{lemma}

We also verify the zero-one law of outcomes.

\begin{lemma}[zero-one law of outcome]\label{lemma:his-fisher-outcome-correspondence}
Let $S'\subseteq V^{S}_{H}$ be a finite subset of vertices in $G^S_H$  and configuration $\tau \in \{0,1\}^{S'}$ on it such that $\mu^{\-{GD}}_{\infty}\left(\+C^{\-{bad}}=S', \sigma(S') = \tau\right)\neq 0$. Then, for arbitrary $\tau \in \{0,1\}^{S'}$ it holds that
\[
\mu^{\-{GD}}_{\infty}\left(\sigma(\ts(S,0)) =  1^{|S|}\mid \+C^{\-{bad}}=S', \sigma(S') = \tau\right) = 0 \text{ or }1.
\]
\end{lemma}

We are now ready to prove \Cref{lemma:his-fisher-marginal}.
\begin{proof}[Proof of \Cref{lemma:his-fisher-marginal}]
If $\beta = 1$, it holds trivially. If $\beta \neq 0$, it holds that $\frac{1}{1+\epsilon} \le \frac{1}{\abs{1 - \beta}}$. So it suffices to prove $\abs{\mu\left(\sigma(S) = 1^{\abs{S}}\right)} < 1 + \epsilon$.
\begin{align*}
&\abs{\mu\left(\sigma(S)=1^{|S|}\right)}\\
% (\text{by \Cref{lemma:framework-marginal-bound}})\quad
\leq &\sum\limits_{i \ge 1} \abs{\+T_i} \left( \ell^\-{fs, pad} \right)^{k \abs{T}} \left(\ell^\-{fs}\right)^{k \Delta(G_H^S)^2 \abs{T}}\\
(\text{by \Cref{lemma:his-fisher-bad-tree-decay}})\quad\leq &\frac{1}{1+\varepsilon}\sum\limits_{i \ge 1} \abs{\+T_i} \left(4\mathrm{e}\Delta^2 k^4\right)^{-i} \\
(\text{by \Cref{lemma:2-tree-number-bound} and \Cref{lemma:witness-graph-degree-bound}})\quad \leq& \frac{1}{1+\varepsilon}\sum\limits_{i\geq 1}\left(2\mathrm{e}\Delta^2 k^4\right)^{i-1}\cdot\left(4\mathrm{e}\Delta^2 k^4\right)^{-i}\\
<&\frac{1}{1+\varepsilon}.
\end{align*}
\end{proof}

Now we give the omitted proofs of \Cref{lemma:his-fisher-well-define-transition}, \Cref{lemma:his-fisher-bound-fs-l-l-pad} and \Cref{lemma:his-fisher-bad-tree-decay}.

\begin{proof}[Proof of \Cref{lemma:his-fisher-well-define-transition}]
    Given $v$ and $\sigma_{V \backslash \{v\}}$, let $\tilde{E} = \{e \mid \forall u,v \in e, u \neq v, \sigma_u = 1\}$. Let $\+R = \prod_{e \in \tilde{E}} \beta_e$, if $\abs{\+R} \ge 1$, then $\forall e \in \tilde{E}$, $\abs{\beta_e} \ge \frac{1}{2}$. otherwise $\abs{\+R} \le \frac{1}{2}(1 + \varepsilon)^{\Delta} < 1$. Also when $\abs{\beta} \ge \frac{1}{2}$, we know $\Arg(\beta) \le \frac{\pi}{2}$ and furthermore,
    \[
    \left|\Arg(\beta)\right| \le \tan \left|\Arg(\beta)\right| \le 2 \varepsilon.
    \]
    The first inequality is due to $x \le \tan(x)$ for $0 \le x < \frac{\pi}{2}$. The second inequality is due to the conditions in \Cref{theorem:zero-freeness-his-fisher}. 
    So $\abs{\+R} \le 2 \Delta \varepsilon < \frac{\pi}{2}$, then $\+R$ can not be $-1$. So the marginal measure is well-defined.
\end{proof}

\begin{proof}[Proof of \Cref{lemma:his-fisher-bound-fs-l-l-pad}]
    We first analyze the transition measure. Given $v$ and $\sigma_{V \backslash \{v\}}$, let $\tilde{E}(v, \sigma_{V \backslash \{v\}}) = \{e \mid \forall u, v \in e, u\neq v, \sigma_u = 1\}$.
    \[
    \mu^{\sigma_{V \backslash \{v\}}}_v(0) = \frac{1}{1 + \prod_{e\in \tilde{E}(v, \sigma_{V \backslash \{v\}})} \beta_e },\quad \mu^{\sigma_{V \backslash \{v\}}}_v(1)=\frac{\prod_{e\in \tilde{E}(v, \sigma_{V \backslash \{v\}})} \beta_e}{1 + \prod_{e\in \tilde{E}(v, \sigma_{V \backslash \{v\}})} \beta_e}.
    \]
    So, 
    \[
    \ell^\-{fs, pad} = \max_{v, \sigma_{V \backslash \{v\}}} \left( \abs{\frac{1}{1 + \prod_{e\in \tilde{E}(v, \sigma_{V \backslash \{v\}})} \beta_e }-\frac{1}{2}} + \abs{\frac{\prod_{e\in \tilde{E}(v, \sigma_{V \backslash \{v\}})} \beta_e}{1 + \prod_{e\in \tilde{E}(v, \sigma_{V \backslash \{v\}})} \beta_e}} \right).
    \]
    Let $v$ and $\sigma_{V \backslash \{v\}}$ be the parameters that maximize $\ell^\-{fs, pad}$. Let $\+R = \prod_{e \in \tilde{E}(v, \sigma_{V \backslash \{v\}})}\beta_e$. So
    \[
    \ell^\-{fs, pad} = \abs{\frac{1}{1+\+R}-\frac{1}{2}} + \abs{\frac{\+R}{1 + \+R}} = \abs{\frac{1 - \+R}{2(1 + \+R)}} + \abs{\frac{\+R}{1 + \+R}} = \frac{\abs{1 - \+R} + 2\abs{\+R}}{\abs{2(1 + \+R)}}.
    \]
    Next, we show that 
    \[
    \+R \in \{(x, y) \mid -2\varepsilon \le x \le 1 + 2 \Delta \varepsilon, \abs{y} \le 2\varepsilon \}.
    \]
    
    For the real part of $\+R$, $\`R(\+R) = \`R(\prod_{e \in \tilde{E}(v, \sigma_{V \backslash \{v\}})} \beta_e) \le (1 + \varepsilon)^{\Delta} \le \exp(\varepsilon \Delta) \le 1 + 2 \Delta \varepsilon$. $\`R(\+R) \ge -\varepsilon (1 + \varepsilon)^{\Delta - 1} \ge -\varepsilon \exp(\varepsilon(\Delta-1)) \ge -2 \varepsilon$.

    For the imaginary part of $\+R$,$\abs{\`I(\+R)} \le 2\varepsilon(1 + \varepsilon)^{\Delta -1} \le 4 \varepsilon$.

    Let $\+R^*$ be the nearest point in $[0, 1 + 2 \Delta \epsilon]$ to $\+R$.

    \[
    \ell^\-{fs, pad} \le \frac{\abs{1-\+R^*} + 4\varepsilon + 2 \+R^* + 8\varepsilon}{2(1 + \+R^* - 4 \varepsilon)}.
    \]
    When $\+R^* > 1$, 
    \[
    \ell^\-{fs, pad} \le \frac{2 \Delta \varepsilon + 4\varepsilon + 2 \+R^* + 8\varepsilon}{2(1 + \+R^* - 4 \varepsilon)} = 1 + \frac{-2 + 20 \varepsilon + 2 \Delta \varepsilon}{2(1 + \+R^* - 4 \varepsilon)} \le \frac{1}{2} + 6 \Delta \epsilon.
    \]

    When $\+R^* \le 1$,
    \[
    \ell^\-{fs, pad} = \frac{1 + \+R^* + 12\varepsilon}{2(1 + \+R^* - 4 \varepsilon)} = \frac{1}{2} + \frac{16 \varepsilon}{2(1 + \+R^* - 4 \varepsilon)} \le \frac{1}{2} + 16 \epsilon.
    \]
    
\end{proof}


\begin{proof}[Proof of \Cref{lemma:his-fisher-bad-tree-decay}]
    By \Cref{lemma:bad-tree-decay}, we only need to verify that $\left(\ell^\-{fs, pad}\right)^{k \abs{T}} \left(\ell^\-{fs}\right)^{k \Delta(G_H^S)^2 \abs{T}} \le \frac{1}{1+\varepsilon} \left( 4 \mathrm{e} \Delta^2 k^4 \right)^{-\abs{T}}$.

\[
\left(\ell^{\-{fs, pad}}\right)^{k \abs{T}} \le \left(\frac{1}{2}+6\Delta \varepsilon\right)^{k \abs{T}} \le \mathrm{pow}\left(2, \left(-1+18 \Delta \varepsilon \right) k \abs{T}\right),
\]
where $\mathrm{pow}(a,b) = a^b$,
the first inequality is by \Cref{lemma:his-fisher-bound-fs-l-l-pad} and the second inequality is by $6 \Delta \varepsilon < 1$ and $\log_2\left(\frac{1}{2}+x\right) \le -1+3x$ for $0 \le x \le 1$.

\[
\left(\ell^\-{fs}\right)^{k \Delta(G_H^S)^2 \abs{T}} \le \left(\ell^\-{fs}\right)^{4 \Delta^2 k^5 \abs{T}} \le \left(1 + 6\Delta  \varepsilon \right)^{4 \Delta^2 k^5 \abs{T}} \le \mathrm{pow}\left(2, 48 \Delta^3 k^5 \varepsilon \abs{T} \right),
\]
the first inequality is by \Cref{lemma:witness-graph-degree-bound}, the second inequality is by \Cref{lemma:his-fisher-bound-fs-l-l-pad} and the last inequality is by $6\Delta\varepsilon< \frac{1}{2}$ and $1 + \frac{x}{2}\le 2^x$ for $x > 0$.

\begin{align*}
\frac{1}{1+\varepsilon} \left( 4 \mathrm{e} \Delta^2 k^4 \right)^{-\abs{T}} 
&= \mathrm{pow}\left(2, -\abs{T} \log_2(4 \mathrm{e} \Delta^2 k^4) + \log_2 \left(\frac{1}{1 + \varepsilon} \right) \right) \\
&\ge 
 \mathrm{pow}\left(2, -\abs{T} \log_2(4 \mathrm{e} \Delta^2 k^4) - 2\varepsilon \right),
\end{align*}
the last inequality is by $\log_2 \left(\frac{1}{1+x}\right) > -2x$ for $0 < x \le 1$. Let $f(x) = \log_2\left(\frac{1}{1+x}\right) + 2 x$, $f'(x) = 2 > 0$ for $0 < x \le 1$. And $f(0) = 0$ so $f(x)>0$ for $0 < x \le 1$. 

Finally, we can verify that under the conditions of \Cref{lemma:his-fisher-marginal}, it holds that,
\[
\left(-1+18\Delta \varepsilon \right) k \abs{T} + 48 \Delta^3 k^5 \varepsilon \abs{T}  \le -\abs{T} \log_2(4 \mathrm{e} \Delta^2 k^4) - 2\varepsilon.
\]
Simplifying the above inequality gives that
\[
\varepsilon \le \frac{k - \log_2(4 \mathrm{e} \Delta^2 k^4)}{2 + 18\Delta + 48 \Delta^3 k^5}.
\]

\end{proof}

==> the_other_proof_fisher.tex <==

\begin{comment}

\yxtodo{This proof is old.}


    Given $\+T^\-{bad} = T$, let $U$ include all vertices in $G_H^S$ whose distance to $T$ are less than $2$. Note $U$ contains all vertices for all possible bad components and their neighbors due to \Cref{definition:stationary-start} and \Cref{definition:bad-vertices-his}. 
    Let $\tilde{G} = (U, \tilde{E})$ be the vertex induced subgraph of $G_H^S[U]$. We transfer $\tilde{G}$ to a directed $\vec{G} = (U, \vec{E})$ that we will use induction on its topological order to prove this lemma. 

    $\vec{G}$ is constructed as follows: 
    for every $(\ts(e_1, t_1), \ts(e_2, t_2)) \in E_H^S$, w.l.o.g. we assume $t_1 > t_2$, then we add $\ts(e_1, t_1) \to \ts(e_2, t_2)$ into 
    $\vec{E}$.
    
    Fix an arbitrary order of the possible topological orders 
    % $\text{TP} = (\ts(e_1, t_1), \ts(e_2, t_2), \dots, \ts(e_{|U|}, t_{|U|}))$.
    $\text{TP} = (v_1, v_2, \dots, v_{|U|})$.

    % \begin{comment}

%     Let 
%     \[
%     S_i = \begin{cases}
%         \{(r_i,c_i)=(0,0), (r_i,c_i)=(\perp,0), (r_i,c_i)=(\perp,1) \} & v_i \notin T \\
%         \{(r_i,c_i)=(\perp,0), (r_i,c_i)=(\perp,1) \} & v_i \in T
%     \end{cases},
%     \]

%         \[
%     \text{Prefix}_m = \prod_{i=1}^m S_i ,
%     \]
    
%     which contains the all possible $(r, c)$s for the vertices in $m$-length prefix in $\text{TP}$. 
    
%     We represent the element in $\text{Prefix}_m$ as vector $(\textbf{r}, \textbf{t})$. 
%     Let 
%     \[
%         w(\textbf{r}, \textbf{c}) = \prod_{i=1}^m \left(\=I[r_i = 0] \mu^{\-{LB}}(0) + \=I[r_i = \perp] \ell^{\-{pad}} \right),
%     \]
%     be the product prefix measure of $(\vec{r}, \vec{c})$,
%     \[
%         w_m = \sum_{(\textbf{r}, \textbf{c}) \in \text{Prefix}_m} w(\textbf{r}, \textbf{c}),
%     \]

%     be the product prefix measure.

%     Define $\Omega_T = \{(\vec{r}, \vec{c}) \in \{0,\perp\}^{C} \times \{0,1\}^C \mid \=T(C) = T\}$ be the set containing  $(\textbf{r},\textbf{s})$s on all possible components. Fix a component $C$ and corresponding $(\vec{r}, \vec{c})$, if $v \notin C$, we say that $v \notin (\vec{r}, \vec{c})$.

% Let $w^\-{LB}(\vec{r}, \vec{c})$ be the lower bound weight of $(\vec{r}, \vec{c})$ defined as,

%     \[w^\-{LB}(\vec{r}, \vec{c}) = \prod\limits_{\substack{j \le |U| \\ v(i) \in (\vec{r}, \vec{c})}} \left(\=I[r_j = 0] \mu^\-{LB}(0) + \=I[r_j = \perp] \mu^\-{LB}(\perp)\right). \]

% Define $i$-th lower bound weight of $(\vec{r}, \vec{c})$ as,
% \[
% w_i(\vec{r}, \vec{c}) = \prod\limits_{\substack{j \le |U| \\ v(i) \in (\vec{r}, \vec{c})}} \left(\=I[r_i = 0] \mu^\-{LB}(0) + \=I[r_i = \perp] \mu^\-{LB}(\perp)\right) 
% \prod\limits_{\substack{j \le i \\ v(j) \in (\vec{r}, \vec{c}) \\ r_j = \perp}}\mu^{\-{pad}, (\vec{r}, \vec{c})}_{v(j)}(c_j).
% \]

%     Let $i$-th lower bound defined as,
%     \[
%     w_i = \sum_{(\vec{r}, \vec{c}) \in \Omega_T} w_i(\vec{r}, \vec{c}).
%     \]


%     Let $ \mu^{\-{pad}, \vec{r}, \vec{c}}_{v(i)}(c_i)$ be the padding measure condition on $\vec{r}, \vec{c}$ as \Cref{definition:marginal-lower-bounds} and $wt^*_m: \{0,1,\perp\}^C \times \{0,1\}^C \to \=R$

%     \begin{align*}
%      wt^*_m(\vec{r},\vec{c}) &=  \left( \prod\limits_{\substack{i \le m \\ v(i) \in (\vec{r}, \vec{c})}} \left|\=I[r_i = 0]\mu^\-{LB}(0) + \=I[r_i = \perp] \mu^\-{LB}(\perp) \mu^{\-{pad}, \vec{r}, \vec{c}}_{v(i)}(c_i) \right|\right) \\
%      % &\quad \times \=I[v(m) \in (\vec{r},\vec{c})] \cdot \abs{\=I[r_m = 0]\mu^\-{LB}(0) + \=I[r_m = \perp] \mu^\-{LB}(\perp)},   
%     \end{align*}


%     be the prefix measure of $(\vec{r}, \vec{c})$.
    
%     Let $w^*_m: (\vec{r}, \vec{c}) \in \{0,\perp\}^{m} \times \{0,1\}^m$
%     \[
%     w^*_m(\vec{r}, \vec{c}) = \max_{\substack{(\vec{r}^*, \vec{c}^*) \in \Omega_T \\\forall i\le m, v_i \notin (\vec{r}^*, \vec{c}^*)  \lor \vec{r}^*_i = \vec{r}_i, \vec{c}^*_i = \vec{c}_i}} wt_m^*(\vec{r}^*, \vec{c}^*)
%     ,
%     \]

%     \[
%     w^*_m = \sum\limits_{ (\vec{r}, \vec{c}) \in \{0,\perp\}^{m} \times \{0,1\}^m} w^*_m(\vec{r},\vec{c}).
%     \]

%     be the prefix measure of length $m$.

%     Note 
%     \[
%     \sum_{\substack{\=T(C) = T \\ \tau_C \in \{0,1\}^C}} \left| \mu^\-{GD}_\infty\left(\+T^\-{bad}=T,\+C^\-{bad}= C,\sigma_C = \tau_C\right) \right| \le w_{|U|}^*
%     \]
%     as all $(\vec{r},\vec{c})$ in $\Omega_T$ is different and the last vertex in the topological order must has $r = \perp$ due to the construction process.
    
%     Now we want to use induction on prefix length to prove that 
%     \[
%     w^*_i \le w_i.
%     \]

%     For base case, $i=1$,
%     $w^*_m = \abs{\mu^\-{pad}(\perp)} \le \ell^\-{pad} =w_1$. 

%     Suppose $w_i^* \le w_i$, pick $(\vec{r}, \vec{c}) \in \{0,1,\perp\}^i \times \{0,1\}^i$, consider $v_{i+1}$, 
%     There are cases 
%     \begin{enumerate}
%         \item If $v_{i + 1} \in T$, $w_{i+1}^* \le w_{i}^* \mu^\-{LB}(\perp)$ and $w_{i+1} = w_i \ell^\-{pad}$. So $w_{i+1}^* \le w_{i + 1}$.
%         \item If $v_{i + 1}$ is not in any extension of $(\vec{r}, \vec{c})$, $w_{i + 1}^* = w_i^*$, $w_{i + 1} = \ell w_i $. So $w_{i + 1}^* \le w_{i + 1}$.
%         \item Otherwise, $w_{i+1}^* \le w_{i}^* \ell$ and $w_{i + 1} = \ell w_i$. So $w_{i + 1}^* \le w_{i + 1}$.
%     \end{enumerate}

%     So we get $w_{|U|}^* \le w_{|U|} = $
%     % Let $B$ be the set of all $(\textbf{r}, \textbf{c})$ condition on $\+T^\-{bad} = T, \sigma_T = \tau_T$, we know that $B \subseteq A$, and we can check that $\mu^\-{GD}_T(B) \le w(A) = \ell^{k \Delta(G_H^S)^2|T|}$.

% Define $\Omega_T = \{(\vec{r}, \vec{c}) \in \{0,\perp\}^{C} \times \{0,1\}^C \mid \=T(C) = T\}$ be the set containing  $(\textbf{r},\textbf{s})$s on all possible components. Fix a component $C$ and corresponding $(\vec{r}, \vec{c})$, if $v \notin C$, we say that $v \notin (\vec{r}, \vec{c})$.

% Let $w^\-{LB}(\vec{r}, \vec{c})$ be the lower bound weight of $(\vec{r}, \vec{c})$ defined as,

%     \[w^\-{LB}(\vec{r}, \vec{c}) = \prod\limits_{\substack{j \le |U| \\ v(i) \in (\vec{r}, \vec{c})}} \left(\=I[r_j = 0] \mu^\-{LB}(0) + \=I[r_j = \perp] \mu^\-{LB}(\perp)\right). \]
        

    Define $\Omega_T = \{(\vec{r}, \vec{c}) \in \{0,\perp\}^{C} \times \{0,1\}^C \mid \=T(C) = T\}$ be the set containing  $(\textbf{r},\textbf{s})$s on all possible components. Fix a component $C$ and corresponding $(\vec{r}, \vec{c})$, if $v \notin C$, we say that $v \notin (\vec{r}, \vec{c})$. We also abuse this notation we denote $\vec{r} \in \Omega_T$ if $\exists \vec{c}$ such that $(\vec{r}, \vec{c}) \in \Omega_T$. And for $\vec{c} \in \{0,1\}^{i}$, we denote $(\vec{r}, \vec{c}) \in \Omega_T$ if there is a extension $\vec{c}^*$ of $\vec{c}$ such that $(\vec{r}, \vec{c}) \in \Omega_T$.

Let $ \mu^{\-{pad}, \vec{r}, \vec{c}}_{v(i)}(c_i)$ be the padding measure condition on $\vec{r}, \vec{c}$ as \Cref{definition:marginal-lower-bounds}.
    
Define $i$-th extension weight of $(\vec{r})$, $w_i(\vec{r}): \Omega_T \to \=R$ defined as,
\[
w_i(\vec{r}) = 
\prod\limits_{\substack{v(j)\in(\vec{r}, \vec{c})}} \left( \=I[r_j = 0]\mu^\-{LB}(0) +  \=I[r_j = \perp] \mu^\-{LB}(\perp)\right) 
\sum\limits_{\substack{\vec{c} \in \{0,1\}^i \\ (\vec{r}, \vec{c}) \in \Omega_T}}
\prod\limits_{\substack{j \le i \\ v(j) \in (\vec{r},\vec{c}) \\ r_j = \perp}} \left(  \mu^{\-{pad}, \vec{r}, \vec{c}}_{v(j)}(c_j)\right),
\]

\[
w_i = \sum_{\substack{\vec{r} \in \Omega_T}} w_i(\vec{r}).
\]

Note that 
\[w_{|U|} = \sum_{\substack{\=T(C) = T \\ \tau_C \in \{0,1\}^C}} \left| \mu^\-{GD}_\infty\left(\+T^\-{bad}=T,\+C^\-{bad}= C,\sigma_C = \tau_C\right) \right|\]

We abuse the notation that we denote $v(i) \in T$ if $\exists \ts(e, t) \in T$, $v(i) \in \ts(e,t)$. Let $b_i = \abs{\{ i | v(i) \in T \}}$. We prove 

\[
w_i \le  \left(\mu^\-{LB}(\perp)\right)^{k|T|} \left(\ell^\-{pad}\right)^{i},
\]

by induction on $i$.
For base case $i = 0$, Consider all $\vec{r}$s in $\Omega_T$, there must be $k|T|$ vertices with $r = \perp$ due to the bad tree $T$. For other vertices, fix vertex $v$, there are $2$ possible cases, 
\begin{enumerate}
    \item $\forall u, v \to u$, $r_u = 0$, then $v \notin \vec{r}$.
    \item $\exists u, v \to u$, $r_u = \perp$, then $r_v$ can choose $0$ or $\perp$.
\end{enumerate}
So for vertices do not in bad tree, it will contribution $\max\left(1, \mu^\-{LB}(0) + \mu^\-{LB}(\perp)\right) \le 1$.
So 
\[
w_0 \le \left(\mu^\-{LB}(\perp)\right)^{k|T|} 
\]

Suppose $w_{i-1} \le \left(\mu^\-{LB}(\perp)\right)^{k|T|} \left(\ell^\-{pad}\right)^{i}$. 

Pick $(\vec{r}, \vec{c}) \in \Omega_T$, which contributes to $w_{i-1}$, the contribution its extension to $w_{i}(\vec{r})$ have following $3$ possible cases:

% \begin{enumerate}
%     \item If $r_{i+1} = 0$, this part is less than $ \left(\ell^\-{pad}\right)^{b_{i-1}} \left(\ell\right)^{i-1} \abs{\mu^\-{LB}(0)}$;
%     \item If $r_{i + 1} = \perp$, this part is less than $w_{i-1}  $
% \end{enumerate}

\begin{enumerate}
    \item If $v(i) \notin \vec{r}$, then the contribution does not change;
    \item If $v(i) \in \vec{r}$, $r_i = \perp$ then $c_i = 0$ or $c_i = 1$ which imples $w_{i}(\vec{r}, \vec{c}) \le w_{i-1}(\vec{r}, \vec{c}) \left( \left|\mu_{v(i)}^{\-{pad}, \vec{r}, \vec{c}}(0)\right| +\left| \mu_{v(i)}^{\-{pad}, \vec{r}, \vec{c}}(1)\right|\right)$. So that
    this contribution will multiply by $\ell^\-{pad}$;
    \item If $v(i) \in \vec{r}$, $r_i = 0$ then the contribution does not change.
\end{enumerate}

So 
\[
w_i \le w_{i-1} \max(1, \ell^\-{pad}) \le \left(\mu^\-{LB}(\perp)\right)^{k|T|} \left(\ell^\-{pad} \right)^{i}
\]

which imples \Cref{lemma:his-fisher-component-pinning-bound}.
\end{proof}
    
\end{comment}

\begin{comment}
%
Given a hypergraph $H=(V,\+E)$, we introduce the following definition of the witness graph $G_H=(V_H, E_H)$. 

\begin{definition}[witness graph]\label{definition:witness-graph-indset}
For a hypergraph $H=(V,\+E)$, the \emph{witness graph} $G_H=(V_H,E_H)$ is an infinite graph with a vertex set 
\[
V_H=\{\ts{}(e,t)\mid e\in \+E,t\in \mathbb{Z}_{\leq 0}\},
\] 
and there is an undirected edge between $x,y \in V_H$ in $G_H$ if and only if $x\neq y$ and $x\cap y\neq\emptyset$.
\end{definition}
We remark that the vertex set $V_H$ is not a multiset, i.e., it does not allow multiple instances of the same element. 
For example, it is possible that for some $t\neq t'$, $\ts{}(e,t)=\ts{}(e,t')$. 
In this case, the two correspond to the same vertex even if $t\neq t'$. 
In addition, the witness graph $G_H$ is decided only by the hypergraph $H$ as $\upd_x(t)$ is a deterministic function. 
For any vertex $x \in V_H$ in the witness graph,
let $e_H(x) \in \+E$ be the edge in the original hypergraph that corresponds to $x$. 

We first bound the degree of the witness graph.   
Define the following neighbourhoods of $x$ in the witness graph $G_H$: 
\begin{align}\label{eq-def-ng}
\begin{split}
	N_{\-{self}}(x) &\defeq \{y \in V_H \mid \{x,y\} \in E_H   \text{ and } e_H(x) =  e_H(y)\},\\
	N_{\-{out}}(x) &\defeq \{y \in V_H \mid \{x,y\} \in E_H  \text{ and } e_H(x) \neq  e_H(y)\},\\
	N(x) &\defeq N_{\-{self}}(x) \uplus N_{\-{out}}(x).
	\end{split}
\end{align}
In other words, we partition the neighbourhood $N(x)$ of $x$ in the witness graph $G_H$ into two parts, one containing those corresponding to the same edge in the original hypergraph, and the other one collecting the rest. 
\begin{lemma}\label{lemma:wg-degree-bound}
For any vertex $x \in V_H$, it holds that $|N_{\-{self}}(x)| \leq 2k-2$ and $|N_{\-{out}}(x)| \leq (2k-1)k(\Delta - 1)$, and therefore, the maximum degree of $G_H$ is bounded by $2\Delta k^2 -2$.
\end{lemma}

\begin{proof}

Fix arbitrarily an edge $e\in \+{E}$ in the original hypergraph $H$ and a time $t\in \mathbb{Z}_{\leq 0}$. 
This induces a vertex $x$ in the witness graph $G_H$. 
We claim that for any $e'\in \+{E}$ such that $e\cap e'\neq \emptyset$, it holds that
%\[\abs{\{\ts{}(e',t')\mid t' \in \mathbb{Z}_{\geq 0} \text{ and } \ts{}(e',t')\cap \ts{}(e,t)\neq \emptyset\}}\leq 2k-1.\]
\[\abs{\{\ts(e',t') \mid t'\in \mathbb{Z}_{\geq 0} \text{ and } \ts{}(e',t')\cap \ts{}(e,t)\neq \emptyset\}}\leq 2k-1.\]
This claim implies the lemma because
\begin{itemize}
\item by taking $e'=e$, we have $|N_{\-{self}}(x)| \leq 2k-2$ (we need to exclude $x$ itself); and
\item by taking $e'$ such that $e'\neq e$ and $e' \cap e \neq \emptyset$, we have $|N_{\-{out}}(x)| \leq (2k-1)k(\Delta - 1)$, since there are at most $(\Delta - 1) k$ choices for such $e'$. 
\end{itemize}

%Observe by \eqref{eq:update-time} and \eqref{eq:timestamp} that $\ts{}(e,t)\cap \ts{}(e',t')\neq \emptyset$ only if $e\cap e'\neq \emptyset$. 
%Then the lemma holds by noting $\abs{\{e'\mid e\cap e'\neq \emptyset\}}\leq \Delta k$ and there's no edge in $G_H$ from $\ts{}(e,t)$ to itself.

We then verify the claim. 
Assume $\ts(e,t)=(t_1,t_2,\dots,t_k)$ where $t_1<t_2<\dots<t_k<t_1+n$, and $\ts(e',t')=(t'_1,t'_2,\dots,t'_k)$ where $t'_1<t'_2<\dots<t'_k<t'_1+n$. 
Observe that $\ts{}(e',t')\cap \ts{}(e,t)\neq \varnothing$ implies $e\cap e'\neq \varnothing$. 
This means the following two quantities
\begin{align*}
  j_{\-{min}}\defeq&\min\left\{j\in[k] \mid v_{i(t_j)}\in e'\right\},~\text{and}\\
  j_{\-{max}}\defeq&\max\left\{j\in[k] \mid v_{i(t_j)}\in e'\right\}
\end{align*}
are well defined.  

Observe that $t'_k\geq t_{j_{\-{min}}}$ and $t'_1\leq t_{j_{\-{max}}}$. 
This can be argued as follows. 
Assume towards contradiction that $t'_k<t_{j_{\-{min}}}$. 
As $\ts{}(e',t')\cap \ts{}(e,t)\neq \varnothing$, there must be such $j$ and $j'$ that $t_j=t'_{j'}\in\ts{}(e',t')\cap \ts{}(e,t)$. 
Note that $t_j=t'_{j'}<t_{j_{\-{min}}}$ because of the ordering $t'_{j'}\leq t'_{k}$ and the assumption. 
This contradicts with the choice of $j_{\min}$. 
The same argument goes for the other inequality. 

The two inequalities above, together with $t'_k<t'_1+n$, implies $t'_1\in (t_{j_{\-{min}}}-n,t_{j_{\-{max}}}]$.  
Note further that in the interval $[t_{j_{\-{min}}}-n,t_{j_{\-{max}}}]$, there are at most $2k$ timestamps when there is a vertex in $e'$ that gets updated: 
$k$ from $[t_{j_{\-{min}}}-n,t_{j_{\-{min}}})$ and at most $k$ from $[t_{j_{\-{min}}},t_{j_{\-{max}}}]$
By definition of $j_{\-{min}}$, the vertex that gets updated at time $t_{j_{\-{min}}}$ must come from $e'$. 
Therefore, there are at most $2k-1$ timestamps in the interval $(t_{j_{\-{min}}}-n,t_{j_{\-{max}}}]$ that update vertices in $e'$,
and hence at most $2k-1$ choices for $t'_1$. 
The claim then follows by observing that the sequence $\ts{}(e',t')=(t'_1,t'_2,\cdots,t'_k)$ is uniquely determined by $t'_1$. 
\end{proof}


To prove , we need the notion of $2$-trees~\cite{Alon91}. 
Given a graph $G=(V,E)$, its power graph $G^2=(V,E_2)$ has the same vertex set, while an edge $(u,v)\in E_2$ if and only if $1\leq \dist_G(u,v)\leq 2$. 

\begin{definition}[$2$-tree]\label{definition:2-tree}
%Let $G=(V,E)$ be a graph and $\text{dist}_G(\cdot,\cdot)$ denote the shortest path distance in $G$.
%A \emph{$2$-tree} in $G$ is a subset of vertices $T\subseteq V$ such that: 
Let $G=(V,E)$ be a graph. A set of vertices $T\subseteq V$ is called a \emph{$2$-tree} of $G$, if
\begin{itemize}
    \item  for any $u,v\in T$, $\text{dist}_G(u,v)\geq 2$, and
    \item  $T$ is connected on $G^2$.
\end{itemize}
\end{definition}

Intuitively, a $2$-tree is an independent set that does not spread far away. 
%We will also need the following two lemmata. 
The next lemma bounds the number of $2$-trees of a certain size containing a given vertex.
\begin{lemma}[{\cite[Corollary 5.7]{feng2021rapid}}]\label{lemma:2-tree-number-bound}
Let $G=(V,E)$ be a graph with maximum degree $D$, and $v\in V$ be a vertex. 
The number of 2-trees in $G$ of size $\ell\geq 2$ containing $v$ is at most $\frac{(\mathrm{e}D^2)^{\ell-1}}{2}$.
\end{lemma}

The next lemma shows the existence of a large $2$-tree.
\begin{lemma}[{\cite[Observation 5.5]{feng2021rapid}} and {\cite[Lemma 4.5]{Vishesh21towards}}]\label{lemma:big-2-tree}
Let $G = (V, E)$ be a graph of maximum degree $D$, 
$H =(V(H),E(H))$ be a connected finite subgraph of $G$, and $v \in V (H)$ a vertex in $H$. 
Then there exists a $2$-tree $T$ of $H$ containing $v$
such that $\abs{T} = \lfloor |V (H)|/(D + 1) \rfloor$.
\end{lemma} 

\end{comment}

\begin{comment}

\section{Application: hypergraph coloring}
In this section, we prove zero-freeness results for hypergraph colorings.

Given a $k$-uniform hypergraph $H=(V,\+{E})$ with maximum degree $\Delta$, $\sigma\in [q]^V$ is a proper coloring of $H$ if no hyperedge is monochromatic. We use $\Omega_H\subseteq [q]^V$ to denote the set of all proper $q$-colourings of $H$.
For a particular color $c\in [q]$, the $c$-chromatic polynomial of the hypergraph $H$ is defined as
\[
Z_{H,c}(\lambda)=\sum\limits_{\sigma\in \Omega_H}\lambda^{\abs{\{v\in V\mid \sigma(v)=c\}}}.
\]
Note that the definition of $Z_{H,c}$ is symmetric with respect to all $c\in [q]$. so we simply fix any $c\in [q]$ and write $Z_H$ instead of $Z_{H,c}$.

The associated measure $\mu=\mu_{c}:\Omega_H\to \=C$  with respect to $Z_H$ is then defined as
\[
\forall \sigma\in \Omega_H,\quad \mu(\sigma)=\frac{\lambda^{\abs{\{v\in V\mid \sigma(v)=c\}}}}{Z_{H}(\lambda)}
\]
when $Z_{H}(\lambda)\neq 0$.

As usual, proving zero-freeness of $Z_{H}(\lambda)$ boils down to proving certain marginal properties.
\begin{lemma}\label{lemma:color-lee-yang-marginal}
Let $H=(V,\+E)$ be a $k$-uniform hypergraph with maximum degree $\Delta$. Let $\varepsilon=\varepsilon_{k,\Delta}$ and $\+D_{\varepsilon}$ be as defined in \Cref{theorem:zero-freeness-color-lee-yang} and let $\lambda\in \+D_{\varepsilon}$. Suppose $Z_{H}(\lambda)\neq 0$ and therefore $\mu$ is well-defined. For any $S \subseteq v$ such that $|S|=k$, it holds that
\[
\mu(\sigma_S\neq c^k)\neq 1.
\]
\end{lemma}

We then show that \Cref{lemma:color-lee-yang-marginal} already implies \Cref{theorem:zero-freeness-color-lee-yang}.
\begin{proof}[Proof of \Cref{theorem:zero-freeness-color-lee-yang}]
Let $\+E=\{e_1,e_2,\dots,e_m\}$. For $0\leq i\leq m$ we let $\+E_i=\{e_1,e_2,\dots,e_i\}$ and let $H_i=(V,\+E_i)$. We prove by induction that $Z_{H_i}(\lambda)\neq 0$ for each $0\leq i\leq m$.

The base case is when $i=0$, and we have $Z_{H_0}=(q-1+\lambda)^{|V|}\neq 0$ since $\lambda\neq -(q-1)$.

For the induction step, we fix $0\leq i<m$ and assume that $Z_{H_{i}}\neq 0$. Then the measure $\mu_{H_i}$ is well-defined. Note that
\[
\frac{Z_{H_{i+1}}(\lambda)}{Z_{H_{i}}(\lambda)}=\frac{Z_{H_{i}}(\lambda)-\sum\limits_{\substack{\sigma\in \{0,1\}^V\\ \sigma(e_{i+1})=c^{k}}}\lambda^{\abs{\{v\in V\mid \sigma(v)=c\}}}}{Z_{H_{i}}(\lambda)}=1-\mu_{H_i}(\sigma(e_{i+1})=c^{k})\neq 0,
\]
where the last inequality is by \Cref{lemma:color-lee-yang-marginal}. Therefore $Z_{H_{i+1}}\neq 0$, completing the induction step and the proof of the lemma.
\end{proof}

Similar as the case of hypergraph independent sets, when $\lambda\neq q-1$, \yxtodo{It seems we can only count feasible colors instead of $q$} for any $v\in V$ , the conditional measure $\mu^{\sigma(V\setminus \{v\})}_v$ is always well-defined for any coloring $\sigma \in \Omega_H$ and any $v\in V$. However, the marginal measure $\mu^{\sigma(V\setminus \{v\})}_v$ does not exhibit any non-trivial lower bounds. Here, it is helpful to consider a relaxed measure than $\mu$ itself, which is a result of the ``entropy compression'' technique in sampling and counting hypergraph colorings~\cite{feng2021sampling,Vishesh21sampling,HSW21,feng2023towards}.


\begin{definition}[Projection scheme and projected measure]
Let $s=\lfloor \sqrt{q}\rfloor$. A (balanced) projection scheme $h:[q]\to [s]$ satisfy that $h^{-1}(i)\in\{\lfloor\frac{q}{s}\rfloor,\lceil\frac{q}{s}\rceil\}$ for all $i\in [s]$.

We also extend $h$ to colorings and partial colorings, i.e., for any $\sigma\in [q]^{\Lambda}$ specified on a subset of vertices $\Lambda\subseteq V$, we let $h(\sigma)\in [s]^{\Lambda}$ to denote the projected coloring $\left(h(\sigma(v))\right)_{v\in \Lambda}$.

Let $h:[q]\to [s]$ be a balanced projection scheme. The projected measure $\psi:[s]^V\to \=C$ is defined as the induced measure $\mu(h(\cdot))$. Formally, 
\[
\forall \sigma\in [s]^V, \quad \psi(\sigma)=\sum\limits_{\tau\in h^{-1}(\sigma)} \mu(\tau).
\]
\end{definition}    

Due to the symmetric definition of colors, we let $c = q$ in this section.

\begin{definition}[Projection scheme and projected measure]
Let $s=\lfloor \sqrt{q}\rfloor$. A $q$-projection scheme $h:[q]\to [3]$ satisfy that 

\[
h(i) = \begin{cases}
    0 &\quad i \le \lceil \frac{q-1}{2} \rceil \\
    1 &\quad \lceil \frac{q-1}{2} \rceil < i \le q - 1 \\
    2 &\quad  i = q
\end{cases}
\].

We also extend $h$ to colorings and partial colorings, i.e., for any $\sigma\in [q]^{\Lambda}$ specified on a subset of vertices $\Lambda\subseteq V$, we let $h(\sigma)\in [3]^{\Lambda}$ to denote the projected coloring $\left(h(\sigma(v))\right)_{v\in \Lambda}$.

Let $h:[q]\to [3]$ be a $q$-projection scheme. The projected measure $\psi:[3]^V\to \=C$ is defined as the induced measure $\mu(h(\cdot))$. Formally, 
\[
\forall \sigma\in [3]^V, \quad \psi(\sigma)=\sum\limits_{\tau\in h^{-1}(\sigma)} \mu(\tau).
\]
\end{definition}

We consider the systematic scan Glauber dynamics with stationary start (\Cref{definition:stationary-start}) with respect to the projected measure $\psi$, where we set $T=\infty$ and the lower bound measure (\Cref{definition:marginal-lower-bounds}) as follows for hypergraph colorings:
\begin{align*}
\psi^\-{LB}(0) = \frac{1}{2}\left(1 - \frac{1}{r}\right),\quad \psi^\-{LB}(1) = \frac{1}{2}\left(1 - \frac{1}{r}\right), \quad \psi^\-{LB}(2) = 0,\quad \psi^\-{LB}(\perp) = \frac{1}{r}
% \forall i\in [s]\setminus \{c\}, \quad \psi^{\-{LB}}(i)=.
\end{align*}
We denote the induced measure of the systematic scan Glauber dynamics as $\psi^{\-{GD}}_{\infty}$ to emphasize that we are dealing with the projected measure.

\begin{lemma}[\text{~\cite[Lemma 7]{guo2019counting}} and \text{~\cite[Lemma 6]{feng2022improved}}] Suppose $q_0 \le |Q_v| \le q_1$ for any $v \in V$. For any $r \ge k \ge 2$, if $q_0^k \ge e q_1 r \Delta$, 
    
\end{lemma}
    
\end{comment}
